Open-system modeling of quantum annealing: theory and applications

In this dissertation, we explore how quantum annealing (QA) and its applications behave in an open system setting. We give derivations and numerical recipes for effective parallel simulation methods for time-dependent open dynamics of quantum annealing devices. We consider the weak-coupling limit to an environment and also the case of $1/f$ noise. The stochastic time-dependent quantum trajectories technique can be utilized in studying weak measurements and feedback error correction in quantum annealing. Then we focus on opensystem descriptions of reverse annealing (RA), which is a promising variant and application of quantum annealing. We show that, with various simulation tools, reverse annealing can benefit from the interaction between the annealer and its environment.

==> ResearchTopic1.tex <==
\chapter{Quantum trajectories}
\label{cha:research_topic_1}
We describe a quantum trajectories technique for the unraveling of the quantum adiabatic master equation in Lindblad form.  By evolving a complex state vector of dimension $N$ instead of a complex density matrix of dimension $N^2$, simulations of larger system sizes become feasible.  The cost of running many trajectories, which is required to recover the master equation evolution, can be minimized by running the trajectories in parallel, making this method suitable for high performance computing clusters. In general, the trajectories method can provide up to a factor $N$ advantage over directly solving the master equation. In special cases where only the expectation values of certain observables are desired, an advantage of up to a factor $N^2$ is possible. We test the method by demonstrating agreement with direct solution of the quantum adiabatic master equation for $8$-qubit quantum annealing examples. We also apply the quantum trajectories method to a $16$-qubit example originally introduced to demonstrate the role of tunneling in quantum annealing, which is significantly more time consuming to solve directly using the master equation. The quantum trajectories method provides insight into individual quantum jump trajectories and their statistics, thus shedding light on open system quantum adiabatic evolution beyond the master equation.

With the growing ability to control and measure ever-larger quantum systems, understanding how to model the interactions between open quantum systems and their environment has become exceedingly important \cite{Wiseman:book}. 
The open system dynamics is often described in terms of a master equation in Lindblad form, describing the effective dynamics of the quantum system after the environmental degrees of freedom have been traced out \cite{Breuer:2002}.  An equivalent approach is that of quantum trajectories (also known as the Monte Carlo wavefunction method)~\cite{carmichael2009statistical,dum1992monte,molmer1993monte}, which can be understood as an unraveling of the master equation in Lindblad form, and which generates a stochastic process whose average is fully equivalent to the master equation (for a review, see Ref.~\cite{daley2014quantum}).  Each trajectory in this approach can also be viewed as the result of continuous indirect measurements of the environment in a certain basis \cite{brun:719}. A quantum trajectories approach exists also for non-Markovian master equations \cite{Imamoglu:94,Breuer:2004wq}. 

While a vast literature exists on the topic of quantum trajectories for time-independent master equations, much less is known for the case of time-dependent master equations (see, e.g., Ref.~\cite{Caiaffa:2017aa}), which is our focus here. Specifically, we focus on the case of open systems evolving adiabatically according to a time-dependent Hamiltonian, weakly coupled to the environment \cite{springerlink:10.1007/BF01011696,ABLZ:12-SI}. This is particularly relevant in the context of quantum annealing and more generally adiabatic quantum computing, whereby the computation proceeds via a time-dependent Hamiltonian and the result of the computation is encoded in the ground state of the final Hamiltonian (for reviews see Refs.~\cite{RevModPhys.80.1061,Albash-Lidar:RMP}). A large body of literature exists on the use of quantum Monte Carlo methods in the context of quantum annealing (see, e.g., Refs.~\cite{Santoro,Heim:2014jf,Albash:2017aa}), but these methods focus on equilibrium properties, while here we are interested in dynamics. The interplay between the key quantities that determine adiabaticity and non-unitary dynamics has not been previously explored in the setting of Monte Carlo wavefunction methods, and here we resolve this question by finding an upper bound on the size of the Monte Carlo time-step. Nor has the question of reducing the computational cost of simulations of the adiabatic master equation via quantum trajectories been discussed so far, and we address this here.

Thus, here we develop the first treatment of a quantum trajectories unravelling of a time-dependent adiabatic master equation (AME).
We make a formal comparison between the quantum trajectory unraveling of the Lindblad master equation with time-independent and time-dependent operators, and discuss the validity of applying it to the unraveling of the AME.   While our analysis closely follows the standard time-independent approach, the time-dependent case results in new additional validity conditions that must be satisfied.

The individual trajectories of the AME shed new light on how the average case captured by the AME emerges.  When the quantum state is a pure energy eigenstate and the unitary evolution is adiabatic, the drift term in the quantum trajectories approach vanishes, and the quantum state follows the instantaneous eigenstates until a jump occurs.  We can associate these jumps with an excitation or relaxation process, depending on the direction of the jump.  This provides an intuitive (yet rigorous) picture for how the averaged dynamics of the AME arises.

An important advantage of the quantum trajectories approach is that for an $N$-dimensional system, one quantum trajectory requires storing and updating $2N-1$ real numbers, while solving the master equation for a density matrix requires storing and updating $N^2-1$ real numbers. This quadratic saving allows simulations of systems with sizes that are infeasible by directly solving the master equation. The tradeoff is that many trajectories must be run in order to accurately approximate the solution of the master equation, but this tradeoff can be reduced by using many parallel processes to represent each trajectory.

Our presentation is organized as follows. In Sec.~\ref{sec:II} we briefly review the AME. We unravel the AME in Sec.~\ref{sec:III} into quantum trajectories taking the form of quantum jumps, allowing for an arbitrary time-dependence of the Hamiltonian and Lindblad operators. In Sec.~\ref{sec:IV} we provide an algorithmic implementation for our adiabatic quantum trajectories and in Sec.~\ref{sec:V} we present three case studies. We perform a cost comparison between the direct simulation of the AME and the quantum trajectories method in Sec.~\ref{sec:timequantitative}. Additional technical details and proofs are provided in the Appendices.

\section{Adiabatic master equation in Lindblad form}
\label{sec:II}
We focus on the AME in Lindblad form, which can be derived with suitable approximations (in the weak coupling limit after performing the Born-Markov, rotating wave, and adiabatic  approximation) from first principles starting
from the system Hamiltonian $H_{\textrm{S}}$, 
the environment Hamiltonian $H_B$, and the interaction Hamiltonian $H_I = g \sum_\alpha A_{\alpha} \otimes B_{\alpha}$, with system operators $A_\alpha$, environment operators $B_{\alpha}$, and system-bath coupling strength $g$~\cite{ABLZ:12-SI}.  
The adiabatic (Lindblad) master equation describes the evolution of the system density matrix $\rho(t)$ and has
%the following form (setting $\hbar = 1$ from now on):

\beq
\label{eqt:ME2-H}
\frac{d}{dt} \rho(t) = -i \left[H_{\textrm{S}}(t) + H_{\textrm{LS}}(t), \rho(t) \right] + \mathcal{L}_{\textrm{WCL}} [\rho(t)] \ , \\
\eeq
%
where $H_{\textrm{LS}}(t)$, which commutes with $H_{\textrm{S}}(t)$, is a Lamb shift Hamiltonian arising from the interaction with the environment.  The dissipative term  $\mathcal{L}_{\mathrm{WCL}}$ takes the form:

\begin{eqnarray}
\mathcal{L}_{\textrm{WCL}}  [\rho(t)]   &\equiv& \sum_{\alpha, \beta} \sum_{\omega} \gamma_{\alpha \beta}(\omega) \left(L_{\beta,\omega}(t) \rho(t) L_{\alpha, \omega}^{\dagger}(t)\phantom{\frac{1}{2}} \right. \notag \\
&& \hspace{-0.5cm} \left. \qquad\qquad - \frac{1}{2} \left\{ L_{\alpha,\omega}^{\dagger}(t) L_{\beta,\omega}(t) , \rho(t) \right\} \right) \ , \label{eqt:ME2-L}
\end{eqnarray}
%
where the sum over $\omega$ is over the Bohr frequencies (eigenenergy differences) of $H_{S}$, $\gamma_{\alpha \beta}(\omega)$ is an element of the positive matrix $\gamma$, and satisfies the Kubo-Martin-Schwinger (KMS) condition if the bath is in a thermal state with inverse temperature $\beta = 1/T$:
\beq
\gamma_{\alpha \beta}(- \omega) = e^{-\beta\omega} \gamma_{\beta\alpha }(\omega)\ .
\label{eq:KMS}
\eeq
The time-dependent Lindblad operators are given by:
%
\begin{align}
L_{\alpha, \omega}(t) &= \sum_{a,b} \delta_{\omega, \eps_b(t) - \eps_a(t)} \bra{\eps_a(t)} A_\alpha \ket{\eps_b(t)} | \eps_a(t) \rangle  \langle \eps_b(t)| \ ,
\label{eq:Lindblad2}
\end{align}
%
where $\ket{\varepsilon_a(t)}$ is the $a$-th instantaneous energy eigenstate of $H_{\textrm{S}}(t)$ with eigenvalue $\varepsilon_a(t)$. 
With this form for the Lindblad operators, decoherence can be understood as occurring in the instantaneous energy eigenbasis~\cite{Albash:2015nx}. 

For the purpose of unravelling the above master equation into quantum trajectories, it is convenient to diagonalize the matrix $\gamma$ 
by an appropriate unitary transformation $u(\omega)$:
%
\begin{equation}
\sum_{\alpha, \beta} u_{i, \alpha}(\omega) \gamma_{\alpha \beta}(\omega) u_{j, \beta}(\omega)^{\dagger} = \left(\begin{matrix} \gamma'_1(\omega) & 0 &\hdots \\0 & \gamma'_2(\omega) & \hdots \\ \vdots & \vdots & \ddots &
\end{matrix}\right)_{i, j} \ ,
\label{eq:unitarytransform}
\end{equation}
%
and to define new operators $A_{i,\omega}(t)$ given by
%
\begin{equation}
L_{\alpha, \omega}(t) = \sum_{i}u_{i,\alpha}(\omega) A_{i,\omega}(t) \ .
\label{eq:L}
\end{equation}
%
In this basis, we can write the dissipative part in diagonal form as:
%
\begin{eqnarray}
\label{eqt:dissdiag}
{\mathcal{L}}_{\textrm{WCL}}  [\rho(t)]  & = &\sum_{i}\sum_{\omega}\gamma'_i(\omega)\left(
A_{i,\omega}(t) \rho(t) A^\dagger_{i,\omega}(t)\phantom{\frac{1}{2}} \right. \notag \\
&& \hspace{-0.5cm} \left. \qquad\qquad - \frac{1}{2} \left\{ A_{i,\omega}^{\dagger}(t) A_{i,\omega}(t) , \rho(t) \right\} \right) \ .
\end{eqnarray}

\section{III: Stochastic Schr\"odinger Equation}
\label{sec:III}
With Eq.~\eqref{eqt:dissdiag}, the master equation Eq.~\eqref{eqt:ME2-H} is in diagonal form and can be unravelled into quantum trajectories. The trajectory is described by a stochastic differential equation (SDE) in the form of jumps or diffusion. Let us consider the case where the coefficients $\gamma'_i(\omega)$ in Eq.~\eqref{eqt:dissdiag} also depend on time. If all $\gamma'_i(\omega, t) \geq 0$, then the dynamics is completely positive (CP)-divisible~\cite{laine2010measure}, and the master equation can be unravelled by using the known unravelling of the the time-independent SDE case~\cite{Breuer:2002,gardiner2004quantum,brun:719}, simply by replacing the time-independent operators and coefficients by the time-dependent ones.

Such an unravelling is also possible, but with modifications, when the dynamics is positive (P)-divisible, i.e., where $\gamma'_i(\omega, t)$ need not be all positive.\footnote{The condition on $\gamma'_i(\omega, t)$ such that the map is P-divisible can be found in the proof given in~\cite{breuer2009stochastic} or Eq.~(25) in~\cite{Caiaffa:2017aa}.} This can be in the form of:
\begin{itemize}
\item {Jump} trajectories: the master equation is unravelled via the non-Markovian quantum jump method (NMQJ)~\cite{piilo2008non, breuer2009stochastic,piilo2009open,harkonen2010jump}, where terms with negative coefficients $\gamma'_i(\omega, t)$ describe the negative channel.
\item {Diffusive} trajectories: recent work on diffusive trajectories~\cite{Caiaffa:2017aa} replaces $\gamma'_i(\omega, t)$ and the operators by the eigenvalues and eigenvectors of a positive transition rate operator $W$ (Eq.~(11) in~\cite{Caiaffa:2017aa}). P-divisible dynamics can be unravelled into a SDE in terms of such eigenvalues and eigenvectors.
\end{itemize}

In the following, we focus on the case of CP maps [with all $\gamma'_i(\omega)\geq 0$] and unravel the master equation in the quantum jumps picture.

\subsection{Unravelling the master equation}
First we absorb the $\gamma'$ coefficients into the definition of $A_i$:
%
\beq 
\sqrt{\gamma'_i(\omega)}A_{i,\omega}(t)\rightarrow A_i(t) \ .
\label{eqt:Aired}
\eeq
%
In this redefinition, the index $i$ now includes the Bohr frequencies.
We write Eq.~\eqref{eqt:ME2-H} in terms of an effective non-Hermitian Hamiltonian $H_{\eff}$:
%
\begin{align}
\label{eqt:effdiagonalform}
\frac{d}{dt}{\rho}(t) &= - i\left(H_{\text{eff}}(t)\rho_S(t) - \rho_S(t)H^{\dagger}_{\text{eff}}(t)\right) \nonumber\\
&\phantom{{}=}+ \sum_{i}A_{i}(t) \rho_S(t) A^\dagger_{i}(t)   \,, 
\end{align}
%
where 
\begin{equation}
\label{eq:Heff}
H_{\text{eff}}(t) = H_{\textrm{S}}(t) + H_{\text{\textrm{LS}}}(t) - \frac{i}{2} \sum\limits_{i}{A}_{i}^{\dagger}(t) {A}_{i}(t)\,.
\end{equation}%
%
Equation~\eqref{eqt:effdiagonalform} can be unravelled into quantum trajectories in the quantum jumps picture, where each trajectory describes the stochastic evolution of a pure state (if the initial state $\rho$ is mixed, $\rho = \sum_i p_i \ketbra{\psi_i}$, then the evolution can be performed on each initial pure state).  The stochastic evolution of the pure state can be written in terms of a stochastic Schr\"{o}dinger equation (in It$\hat{\text{o}}$ form), the ensemble average of which is equivalent to the master equation:
%
\begin{align}
\label{eqt:sse}
d\ket{\psi(t)} &= \left(- i{H}_{\text{eff}}(t) + \frac{1}{2}\sum_{i}\braket{{A}_{i}^{\dagger}(t){A}_{i}(t)}\right) dt \ket{\psi(t)} \nonumber \\
&\phantom{{}=}+ \sum_{i} dN_{i}(t)\left(  \frac{{A}_{i}(t)}{\sqrt{\braket{{A}^{\dagger}_{i}(t){A}_{i}(t)}}} - \mathds{1}        \right)\ket{\psi(t)}
\end{align}
%
where 
\beq
\braket{{A}_{i}^{\dagger}(t){A}_{i}(t)} \equiv \braket{\psi(t)|{A}_{i}^{\dagger}(t){A}_{i}(t)|\psi(t)} = \lVert{A}_{i}(t)\ket{\psi(t)}\rVert^2\ .
\label{eq:12}
\eeq 
We give a derivation of Eq.~\eqref{eqt:sse} below.
The first term on the r.h.s. of Eq.~\eqref{eqt:sse} gives a deterministic evolution composed of a Hermitian component [$-i(H_{\text{S}}(t) + H_{\text{\textrm{LS}}}(t))$] and a ``drift'' component 
\beq
D(t) \equiv  \frac{1}{2}\sum_{i} A_{i}^{\dagger}(t)A_{i}(t) - \braket{A_{i}^{\dagger}(t)A_{i}(t)} \ ,
\eeq
and the second term describes the stochastic jump process.  The stochastic variable $dN_{i}(t)\equiv N_i(t+dt) - N_i(t)$ is the number of jumps of type $i$ in the interval $dt$, where we have denoted by $N_i(t)$ the number of jumps of type $i$ up to time $t$.  The expectation value of the stochastic variable is given by  \cite{Breuer:2002}:
%
\beq
E[dN_{i}(t)] = \braket{{A}_{i}^{\dagger}(t){A}_{i}(t)}dt \,.
\eeq
%
Since the probability of a jump occurring scales linearly with $dt$, the probability of having more than one jump vanishes faster than $dt$, so as $dt\to 0$ only one jump out of all possible types during $dt$ is permitted. Therefore we can write~\cite{gardiner2004quantum}:

\begin{equation}
\label{eqt:stochastic1}
dN_{i}(t) = \left\{
                \begin{array}{ll}
                  1 &\text{with prob.                } \braket{{A}_{i}^{\dagger}(t){A}_{i}(t)}dt\\
                  0 &\text{with prob.                }  1 - \braket{{A}_{i}^{\dagger}(t){A}_{i}(t)}dt
                \end{array}
\right.
\end{equation}
with the It$\hat{\text{o}}$ table:
%
\bes
\label{eqt:stochastic2}
\begin{align}
dN_{j}(t)dN_{k}(t) &= \delta_{jk}dN_{j}(t)  \\
dN_{j}(t)dt &= 0 \,.
\end{align}
\ees
%
From Eq.~\eqref{eqt:stochastic1}, the probability of any jump occurring, $\sum_{i}\braket{{A}_{i}^{\dagger}(t){A}_{i}(t)}dt$, is small compared to the probability of no jump occurring, so $\sum_{i}dN_{i}(t) = 0$ most of the time. During the infinitesimal time-step $dt$, if $\sum_{i}dN_{i}(t) = 0$, then only the deterministic evolution takes places; if however $\sum_{i}dN_{i}(t) = 1$, then a jump occurs. When a jump occurs, it dominates over the deterministic evolution, which is proportional to $d t$, and the deterministic part can be ignored.

\subsection{Deterministic evolution and jump process}
\label{ssec:A}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We now derive Eq.~\eqref{eqt:sse} by explaining how each probability element appears.  Let us denote by $\ket{\psi(t)}$ and $\ket{\tilde{\psi}(t)}$ the normalized and unnormalized state vectors respectively, and assume they are equal at time $t$, i.e., $\ket{\tilde{\psi}(t)} = \ket{\psi(t)}$.  
%
For the infinitesimal time-step from $t$ to $t+dt$, the state vector evolution from $\ket{\psi(t)}$ to $\ket{\psi(t+dt)}$ involves two possibilities: either no jump occurring (with probability $1- dp$) or a jump occurring (with probability $dp$).  This is depicted in Fig.~\ref{fig:branch}.
%
\begin{figure}[t!]
\centering
\includegraphics[width=3in]{qt/branching.pdf}  
\caption{A depiction of the stochastic evolution of the state $\ket{\psi}$ by an infinitesimal time state at time $t$.}  
\label{fig:branch}
\end{figure}
%

When no jump occurs, the evolution is described by the Schr\"{o}dinger equation associated with $H_\eff$, and since the effective Hamiltonian is non-Hermitian the norm of the state vector is not preserved during the evolution:
%
\begin{equation}
\label{eqt:Schr}
\frac{d\ket{\tilde{\psi}(t)}}{dt} = -iH_{\text{eff}}(t) \ket{\tilde{\psi}(t)} \,.
\end{equation}
%
The resulting state after one infinitesimal time-step $dt$ is:
%
\bes
\label{eqt:detun}
\begin{align}
\ket{\tilde{\psi}(t+dt)} &= \exp\left[-iH_{\text{eff}}(t)dt\right]\ket{\psi(t)} \\   
&= \left[\mathds{I} - i dt H_{\text{eff}}(t)   + O(dt^2)\right] \ket{\psi(t)} \ .
\end{align}
\ees
%
The norm squared $\|\tilde{\psi}(t+dt)\|^2$ is the probability of the conditional evolution under $H_\eff$, 
so that (as we show explicitly in Appendix~\ref{app:A}) the jump probability is given by
%
\beq
1-\|\tilde{\psi}(t+dt)\|^2 = dt  \sum_{i}\braket{{A}_i^{\dagger}(t){A}_i(t)} + O(dt^2) 
\label{eqt:squareofnorm}
\eeq
%
[recall Eq.~\eqref{eq:12} and note that $H_{\text{\textrm{S}}}(t)+H_{\text{\textrm{LS}}}(t)$ cancels out to first order].
Therefore we can identify the infinitesimal jump probability $dp(t)$ with the r.h.s. of Eq.~\eqref{eqt:squareofnorm}, i.e., to first order in $dt$:
%
\bes
\label{eq:jumprate}
\begin{align}
\label{eqt:jumpprob}
dp(t) &= \sum_{i} dp_i (t) = dt \lambda(t) \\
\label{eqt:typeprob}
dp_i(t) &= dt \braket{{A}_i^{\dagger}(t){A}_i(t)} \ ,
\end{align}
\ees
where $\lambda(t) = \dot{p}(t)$ is the jump rate, and $dp_i(t)$ is the probability of the jump of type $i$.  Note that since our definition of the $A_i$ operators includes the rates $\gamma'$ [recall Eq.~\eqref{eqt:Aired}], the jump rate depends on the instantaneous Bohr frequencies and the KMS condition.

When the jump of type $i$ occurs the state is updated as:
%
\begin{equation}
\label{eqt:jumpun}
\ket{\tilde{\psi}(t+dt)} ={A}_i(t)\ket{\psi(t)} \,.
\end{equation}

We can unify the two possibilities in Eq.~\eqref{eqt:detun} and Eq.~\eqref{eqt:jumpun} as a stochastic Schr\"{o}dinger equation for the unnormalized state vector where only terms of order $dt$ are kept:
\bes
\label{eqt:sse2}
\begin{align}
d\ket{\tilde{\psi}(t)} &= \ket{\tilde{\psi}(t + dt)} - \ket{\tilde{\psi}(t)} \\
&= -i dt H_{\text{eff}}(t)\ket{\tilde{\psi}(t)}  + \nonumber\\
&\phantom{=}\sum_{i}dN_{i}(t)\left({A}_i(t)-\mathds{1}\right)\ket{\tilde{\psi}(t)} \,,
\end{align}
\ees
where we used $\ket{\tilde{\psi(t)}} = \ket{\psi(t)}$. The stochastic element $dN_{i}(t)$ has the properties given in Eqs.~\eqref{eqt:stochastic1} and~\eqref{eqt:stochastic2}; $\mathds{1}$ is subtracted since when the jump  occurs $\sum_{i}dN_{i}(t)\ket{\tilde{\psi}(t)} = \ket{\tilde{\psi}(t)}$ and the term involving $H_{\text{eff}}(t)$ is absent, so in this manner we ensure that $\ket{\tilde{\psi}(t)}$ is appropriately subtracted from the r.h.s.

We can write a similar expression for the normalized state vector $\ket{\psi(t)}$ by normalizing Eqs.~\eqref{eqt:detun} and~\eqref{eqt:jumpun}.  If a deterministic evolution occurs, we have
%
\bes
\label{eqt:deterministicequivalence}
\begin{align}
\label{eqt:deterministicequivalence-1}
\ket{\psi(t + dt)} &= \frac{\exp\left[-iH_{\text{eff}}(t)dt\right]\ket{\psi(t)}}{\norm{\exp\left[-iH_{\text{eff}}(t)dt\right]\ket{\psi(t)}}} \\
&\hspace{-1cm}= \frac{\left(\mathds{1} - i dt H_{\text{eff}}(t)+O(dt^2)\right)\ket{\psi(t)}}{\sqrt{1 - dt \sum_{i}\braket{{A}_i^{\dagger}(t){A}_i(t) } + O(dt^2)}}\\
&\hspace{-1cm} = \left(\mathds{1} - i dt H_{\text{eff}}(t) + \frac{1}{2}\sum_{i} \braket{{A}_i^{\dagger}(t){A}_i(t)}dt \right)\ket{\psi(t)}  \notag \\
& + {O}(dt^2)\ .
\end{align}
\ees
%
If a jump of type $i$ occurs, we have
%
\begin{equation}
\ket{\psi(t + dt)} = \frac{{A}_i(t)\ket{\psi(t)}}{\norm{{A}_i(t)\ket{\psi(t)}}} = \frac{{A}_i(t)\ket{\psi(t)}}{\sqrt{\braket{{A}^{\dagger}_{i}(t){A}_{i}(t)}}}\,.
\label{eqt:jump}
\end{equation}
%
Therefore, in analogy to Eq.~\eqref{eqt:sse2} we can write the stochastic Schr\"odinger equation for the normalized state as in Eq.~\eqref{eqt:sse}.




\section{IV: Simulation procedure for adiabatic quantum trajectories}
\label{sec:IV}
In this section we formulate an algorithm for implementing adiabatic quantum trajectories. We start by noticing that the update in Eq.~\eqref{eqt:deterministicequivalence-1} corresponds to the evolution by the first part of the stochastic Schr\"{o}dinger equation. Therefore, the deterministic evolution in the first term of Eq.~\eqref{eqt:sse} is equivalent to propagating the state vector via the Schr\"{o}dinger equation with $H_\eff(t)$ and then renormalizing it. 

When a jump occurs, one of the operators $A_i(t)$ is applied.  The relative weight of each $A_i(t)$ is $dp_i(t)$, given in Eq.~\eqref{eqt:typeprob}. In this case, the state is evolved as in Eq.~\eqref{eqt:jumpun}, and the normalized state is given in Eq.~\eqref{eqt:jump}. 
The update in Eq.~\eqref{eqt:jump} corresponds to the evolution by the second term of Eq.~\eqref{eqt:sse}. 

This provides a direct way to algorithmically implement the quantum trajectories method.   Starting from a known normalized initial state, the state is evolved via a sequence of deterministic evolutions and jumps, as in Eqs.~\eqref{eqt:detun} and~\eqref{eqt:jump}, by drawing a random number at each finite but small time-step $\Delta t$ and determining which of the two choices to take.  Compared to the standard time-independent case, the size of the time-step must satisfy additional conditions in order for the approximations to hold:
%
\beq
\Delta t \ll \min_t \left\{ \frac{2\vertiii{H_{\text{eff}}(t)}}{\| \dot{H}_{\text{eff}}(t)\|},
\frac{1}{\vertiii{H_{\text{eff}}(t)}},
\left|\frac{ \lambda(t) }{ \lambda^2(t)-\dot{\lambda}(t)}\right| \right\} \ ,
\label{eq:newcond}
\eeq
%
where $\|\cdot\|$ is the operator norm (largest singular value).  We give a proof of this new bound in Appendix~\ref{app:B}.  While the second and third terms reduce to the known conditions for the time-independent case, the first term in Eq.~\eqref{eq:newcond} is unique to the time-dependent case and reflects the error associated with time evolution under a time-dependent effective Hamiltonian.  This term highlights the fact that the faster the effective Hamiltonian and its eigenstates vary in time, the smaller is the time-step required to properly follow the trajectory. Eq.~\eqref{eq:newcond} can also be viewed as the physical timestep upper bound in weak measurement.
%%DL: why?
%, but this may also take us beyond the regime of validity of the AME.

However, drawing a random number at each time-step is computationally expensive, 
so it is more efficient to use the waiting time distribution~\cite{Breuer:2002}
to determine the first jump event.  As we mentioned before [Eq.~\eqref{eqt:squareofnorm}] the square norm of the unnormalized wavefunction at $t + dt$ gives the probability of no jump during the infinitesimal interval $[t,t+dt]$. We show in Appendix~\ref{sec:C} that starting from the normalized state $\ket{\psi(t)}$, the probability of no jump occurring in the finite (not necessarily small) time interval $[t,t+\tau]$ is given by
%
\begin{equation}
\|\tilde{\psi}(t+\tau)\|^2 =  \exp\left(-\int_t^{t+\tau}\lambda(s)ds \right) \,,
\end{equation}
%
where the jump rate $\lambda(t)$ is given in Eq.~\eqref{eqt:jumpprob}. 
With this, the simulation procedure for one single trajectory is as follows, starting from $t$:
\begin{itemize}
\label{item:algo}
\item Draw a random number $r$.
%
\item Propagate the unnormalized wavefunction by solving the Schr\"{o}dinger equation with $H_\eff$ [Eq.~\eqref{eqt:Schr}] until the jump condition is reached at $t+\tau$, i.e., for $\tau$ such that $\braket{\tilde{\psi}(t+\tau)|\tilde{\psi}(t+\tau)} \leq  r$. (Recall that the norm of the unnormalized wavefunction will keep decreasing in this process.)
%
\item Determine which jump occurs by drawing another random number and update the wavefunction by applying jump operators, and renormalize.
%
\item Repeat the above steps with the new normalized state.  
%
\item Repeat until the final simulation time is reached.
\end{itemize}
%

We prove that averaging over quantum trajectories recovers the master equation in Appendix~\ref{app:B}. Specifically, we show there that if we denote the state of the $k$-th trajectory at time $t$ by $\ket{\psi_k(t)}$, then we can approximate the master equation solution for the density matrix $\rho(t)$ as $\frac{1}{n}\sum_{k=1}^{n}\ketbra{\psi_k(t)}$ for large $n$. Choosing a basis $\{\ket{z_i}\}$ for the system Hilbert space, we can thus approximate the density matrix element $\bra{z_i} \rho(t) \ket{z_j}$ as $\frac{1}{n}\sum_{k=1}^{n}\langle{z_i} \ketbra{\psi_k(t)} {z_j}\rangle$ for large $n$.
%


\section{V: Case studies}
\label{sec:V}
We consider a system of $N$ qubits with a transverse-field Ising Hamiltonian given by
\begin{subequations}
\label{eqt:H_S}
\begin{eqnarray}
\label{eqt:H_Sa}
{H_{\textrm{S}}(t)} &=& A(t) H_{\textrm{S}}^X + B(t) H_{\textrm{S}}^Z {\ , } \\
H_{\textrm{S}}^X &\equiv& -\sum_{i=1}^N \sigma_i^x { \ ,}\\
H_{\textrm{S}}^Z &\equiv&  - \sum_{i=1}^N h_i
\sigma_i^z + \sum_{i>j=1}^N  J_{i j} \sigma_i^z \sigma_j^z \ .
\end{eqnarray}
\end{subequations}
%

\begin{figure}[t]
\centering
\subfigure[\ ]{\includegraphics[width=0.49\textwidth]{qt/fig4_1}\label{fig:4a}} 
\subfigure[\ ]{\includegraphics[width=0.15\textwidth]{qt/Case0989Crop2}\label{fig:4b}} 
\subfigure[\ ]{\includegraphics[width=0.49\textwidth]{qt/fig4_2}\label{fig:4c}} 
\caption{Graphs of (a) the $8$-qubit chain, (b) the $8$-qubit Hamiltonian exhibiting a small gap, and (c) the $16$-qubit ``tunneling-probe" Hamiltonian of Ref.~\cite{Boixo:2014yu}. (a) Only the first qubit is subjected to an applied field and each qubit is ferromagnetically coupled with $J = -1$. (b)  Solid lines corresponds to ferromagnetic coupling and dashed lines corresponds to  antiferromagnetic coupling.  The thickness denotes the strength of the coupling.  Local fields are shown inside the circles.  Full parameters are given in Eq.~\eqref{eqt:Case0989}.  (c) The left $8$-qubit cell and right $8$-qubit cell are each subjected to applied fields with opposite direction. Each qubit is ferromagnetically coupled to others as shown by the lines, with $J = -1$.}
\end{figure}

%
\begin{figure}[t]
\begin{center}
{\includegraphics[width=0.49\textwidth]{qt/EnergyPop_8Qubit_tf=10us_T=20mK_DW1_v1}} 
\end{center}
\caption{The evolution of the population in the instantaneous ground state for the $8$-qubit problem in Eqs.~\eqref{eqt:H_S} and \eqref{eqt:Ising} for a total time of $t_f = 10 \mu s$ and temperature $2.6$GHz (in $\hbar\equiv 1$ units), as a function of the normalized time $s=t/t_f$.  The quantum trajectories results with $10^4$ trajectories (QT, blue circles) are in excellent agreement with the adiabatic master equation (ME, red solid line).   Inset: the convergence of the ground state population (averaged over quantum trajectories) towards the master equation result as a function of the number of trajectories,  at $s = 1$.  The error bars represent $2 \sigma$ confidence intervals, where $\sigma$ is the standard deviation of the mean generated by taking $10^3$ bootstraps over the number of trajectories. }
  \label{fig:3qubits8qubits}
\end{figure}
%

We assume that the qubit-system is coupled to independent, identical bosonic baths, with the bath and interaction Hamiltonian being 
%
\bes
\begin{align}
\label{eq:SBm}
H_B &= \sum_{i=1}^N \sum_{k=1}^\infty \omega_k b_{k,i}^\dagger b_{k,i} \ ,  \\
 H_{I} &= g \sum_{i=1}^N
\sigma_i^z \otimes \sum_k \left(b_{k,i}^\dagger + b_{k,i} \right) \ ,
\end{align}
\ees
%
where $b_{k,i}^\dagger$ and $b_{k,i}$ are, respectively, raising and lowering operators for the $k$-th
oscillator mode with natural frequency $\omega_k$. 
The bath correlation functions appearing in Eq.~\eqref{eqt:ME2-L} are given by
%
\begin{equation}
\gamma_{ij}(\omega) = 2\pi g^2\frac{\omega e^{-|\omega|/\omega_c}}{1-e^{-\b\omega}} \delta_{ij} \ ,
\end{equation}
%
arising from an Ohmic spectral density~\cite{ABLZ:12-SI}, and satisfy the KMS condition~\eqref{eq:KMS}.


%%%%%%%%%%%
\subsection{$8$-qubit chain} \label{sec:8qubitchain}
%
As a first illustrative example and as a consistency check, we reproduce the master equation evolution of the $8$-qubit ferromagnetic Ising spin chain in a transverse field studied in Ref.~\cite{ABLZ:12-SI}. For this problem, the Ising parameters are given by [also shown in Fig.~\ref{fig:4a}]
%
\begin{equation} \label{eqt:Ising}
 h_1 = \frac{1}{4} \ , \quad h_{i>1}=0  \ , \quad  J_{i, i+1} = -1 \ , \quad i = 1, \dots, 8 \ .
\end{equation}
%
The functional form of the functions $A(t)$ and $B(t)$ is given in Appendix \ref{app:Chain} (they are the annealing schedule of the D-Wave One ``Rainier" processor, described in detail, e.g., in Ref.~\cite{q108}, and were also used in the original AME study of the $8$-qubit chain~\cite{ABLZ:12-SI}). 
The effect of changing the schedule is small; for comparison we provide in Appendix~\ref{app:Chain} results for a linear annealing schedule with the same bath parameters. As shown in Fig.~\ref{fig:3qubits8qubits}, we recover the master equation solution within the error bars.  The initial state is the ground state of $H_{S}(0)$, which is the uniform superposition state.  

It is illustrative to see how a single trajectory differs from the averaged case, and we show this in Fig.~\ref{fig:8qubitssingle}.  Instead of the smooth change in the population as observed in the averaged case, the single trajectory behaves like a step-function. This is explained by the fact that the drift term vanishes if $\ket{\psi(t)}$ is a nondegenerate eigenstate, as shown in Appendix~\ref{app:eigenstate-proof}. Therefore changes in the state's overlap with the instantaneous ground state occur only due to the jump operators.  In this picture, the ground state population revival observed after the minimum gap is crossed is associated with jumps from the first excited state (or higher states for large $T$) to the ground state. After the minimum gap, there are more transitions back to the ground state than out of the ground state (see the inset of Fig.~\ref{fig:8qubitssingle}). Such a difference (divided by the number of trajectories) leads to the rise of the ground state population. 

Using Eq.~\eqref{eq:jumprate}, we can give an explicit expression for the jump rate from the first excited state back to ground state. As shown in  Appendix~\ref{app:lindbladfermi}, this is given by:
\begin{equation}
\label{eq:inctunnrate}
\lambda_{1\rightarrow0}(t) = 
\sum_{\alpha = 1}^{8} \gamma_\alpha(\omega_{10})|\langle\psi_0(t)|\sigma^{z}_{\alpha} |\psi_1(t)\rangle|^2\ .
\end{equation}

%
\begin{figure}[t] %  figure placement: here, top, bottom, or page
\centering
\includegraphics[width=0.49\textwidth]{qt/Trajectory_r55_8Qubit_tf=10us_T=20mK_DW1_v1}
\caption{The overlap squared of the (normalized) state with the instantaneous ground state of $H_{S}(t)$ for a typical single trajectory of the 8 qubit chain in Sec.~\ref{sec:8qubitchain}, with $t_f  = 10\mu s$ and temperature $2.62$GHz, as a function of the normalized time $s=t/t_f$. The sudden changes in the overlap are due to the action of the jump operators $\left\{A_i(t) \right\}$, taking the state from one eigenstate to another. This is to be contrasted with the smooth behavior of Fig.~\ref{fig:3qubits8qubits} when we average over different trajectories.  Inset: a histogram of the net number of jumps to the instantaneous ground state (GS).  A negative number indicates a jump out of the ground state, and a positive number indicates a jump towards the ground state. The change from negative to positive net jumps occurs at the minimum gap point.}
\label{fig:8qubitssingle}
\end{figure}
%

\begin{figure}[t]
\begin{center}
{\includegraphics[width=0.49\textwidth]{qt/EnergyPop_Case0989_tf=10us_T=12mK_DW2X_v1}} 
\end{center}
\caption{The evolution of the population in the instantaneous ground state for the $8$-qubit problem in Eqs.~\eqref{eqt:H_S} and \eqref{eqt:Case0989} for a total time of $t_f = 10 \mu s$ and temperature $1.57$GHz, as a function of the normalized time $s=t/t_f$.  The quantum trajectories results with $5\times 10^3$ trajectories (blue circles) are in excellent agreement with the master equation (red solid line). We also show the closed-system evolution (yellow dashed line) to highlight that the evolution is not adiabatic.   Inset: the instantaneous energy gap between the first excited state and the ground state during the anneal. The minimum occurs at $s^*=0.46$, coinciding with the sharp discontinuity observed in the instantaneous ground state population.}
   \label{fig:case0989}
\end{figure}
%%%%%%%%%%%
\subsection{$8$-qubit non-adiabatic example} 
\label{sec:case0989}

We now consider an $8$-qubit problem with a sufficiently small minimum gap such that the closed-system evolution is not adiabatic even with $t_f = 10 \mu s$ and using the DW2X annealing schedule (described in detail, e.g., in Ref.~\cite{Albash:2017aa}).  While this strictly violates the assumptions under which the AME is derived,%
\footnote{Equation~(27) in Ref.~\cite{ABLZ:12-SI} is a necessary condition for the validity of the AME. It states that $\frac{h}{\Delta^2 t_f}\ll 1$, where $\Delta$ is the ground state gap and $h = \max_{s\in [0,1];a,b} |\bra{\epsilon_a(s)}|\partial_sH_S(s)\ket{\epsilon_b(s)}|$, with $s=t/t_f$ and $\ket{\epsilon_a(s)}$ being the instantaneous $a$-th eigenstate of the system Hamiltonian $H_S(s)$. We find that for $t_f = 10 \mu s$, the l.h.s.$\approx 5$.}
we can ask about the dynamics associated with the master equation irrespective of its origins. We are interested in this example since it illustrates some aspects of the quantum trajectories picture which are not visible in the adiabatic limit, as explained below.

The Ising Hamiltonian $H_S^Z$ is defined with parameters:
%
\bes \label{eqt:Case0989}
\begin{align}
3 \vec{h} &= (-2, -2, 2, -3, 1, 3, -3, 3) \ , \\
 3J_{0,4} &= \phantom{-}1, 3J_{0,5} = -3,  3J_{0,6} = -1,  3J_{0,7} = -1,  \\
 3J_{1,4} &= -1, 3J_{1,5} = -2,  3J_{1,6} = \phantom{-}2,  3J_{1,7} = -3,  \\
 3J_{2,4} &= -2, 3J_{2,5} = -1,  3J_{2,6} = -3,  3J_{2,7} = -2, \\
 3J_{3,4} &= -3, 3J_{3,5} = -3,  3J_{3,6} = -1,  3J_{3,7} = -3, 
\end{align}
\ees
%
Figure~\ref{fig:case0989} shows our simulation results, obtained by solving the AME directly and by using the trajectories approach. Reassuringly, the agreement between the two is excellent. Also plotted are the closed system results for this problem, which exhibit a sharp diabatic transition out of the ground state at the minimum gap point (the small gap is shown in the inset). The AME and trajectories results show that the ground state population loss starts before the diabatic transition, due to thermal excitations, but that the ground state population loss is partially mitigated by the presence of the thermal bath, with the open system ending up with a higher ground state population than the closed system. 

The diabatic transition results in different trajectories than those observed for the adiabatic case in Sec.~\ref{sec:8qubitchain}.  We show such a case in Fig.~\ref{fig:Case0989single}.  Instead of the pulse-like structure seen in Fig.~\ref{fig:8qubitssingle}, we observe a combination of both drifts and jumps.  Because the diabatic transition generates a non-eigenstate that is a coherent superposition of the ground state and first excited state, drifts caused by the environment show up in the subsequent evolution.  Furthermore, this superposition also means that the Lindblad operator associated with $\omega = 0$, if having different component weights in Eq.~\eqref{eq:Lindblad2}, can also induce jumps (e.g., the jumps around $s = 0.6$ in Fig.~\ref{fig:Case0989single}), an effect that is completely absent in the adiabatic case.  These jumps need not project the state completely onto an instantaneous energy eigenbasis state, but they can change the relative weights on the different occupied eigenstates, which manifest themselves as `incomplete' jumps in the trajectories.

We reemphasize that due to the violation of the conditions under which the AME is derived, the observations we have reported for this example are strictly valid only when the AME is taken at face value, and do not necessarily reflect actual physical dynamics.


\begin{figure}[h] %  figure placement: here, top, bottom, or page
\centering
\includegraphics[width=0.49\textwidth]{qt/Trajectory_r200_Case0989_Gauge0_tf=10us_v1}
\caption{The overlap squared of the (normalized) state with the instantaneous ground state of $H_{S}(t)$ (blue solid curve) and the sum of the first three instantaneous excited states (red dashed curve) for a typical single trajectory of the $8$-qubit problem in Sec.~\ref{sec:case0989}, with $t_f  = 10\mu s$ and temperature $1.57$GHz, as a function of the normalized time $s=t/t_f$. A diabatic transition occurs at $s^* = 0.46$. The continuous decay immediately afterward and between the `incomplete' jumps is to be contrasted with the step-function like single trajectories of the adiabatic case seen in Fig.~\ref{fig:8qubitssingle}. 
}
\label{fig:Case0989single}
\end{figure}

\begin{figure}[h!] %  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=0.49\textwidth]{qt/EnergyPop_Google_Gadget_tf=10us_v2} 
   \caption{Quantum trajectory results for a temperature of $12m$K and $20m$K using the DW2X annealing schedule. Results are averaged over $5000$ trajectories. A revival of instantaneous ground state population occurs after the minimum gap (shown by the dashed vertical line).}
   \label{fig:GoogleGadget}
\end{figure}
%

%%%%%%%%%%%
\subsection{$16$-qubit ``tunneling-probe" Hamiltonian}
\label{sec:16qubit}
%
In order to demonstrate the computational utility of the trajectories approach over the master equation approach, we now give results for a $16$-qubit system first studied in Ref.~\cite{Boixo:2014yu} for the purpose of probing tunneling in quantum annealing. 

For this problem, the parameters of Eq.~\eqref{eqt:H_S} are [also shown in Fig.~\ref{fig:4b}]:
\begin{equation} 
\label{eqt:H_S16}
 h_{\text{L}} = 0.44\ , \quad h_{\text{R}} = -1  \ , \quad  J_{i, i+1} = -1 \ , \quad i = 1, \dots, 16 \ .
\end{equation}
where the sets $L$ and $R$ range over $i = 1,\dots, 8$ and $i = 9,\dots, 16$, respectively. Ref.~\cite{Boixo:2014yu} chose the value of $h_{\text{L}}$ to ensure that the minimum ground state gap is lower than the temperature $T=15.5$mK, in order to study a non-trivial interplay between tunneling and thermal activation.\footnote{The problem features one global minimum and one local (false) minimum, which are separated by a tall energy barrier at around the minimum gap point (see Fig.~2 in Ref.~\cite{Boixo:2014yu}); to reach the global minimum from the false minimum, the system state has to transverse the barrier. Such transitions can be modeled as quantum jumps in the quantum jump picture.} This parameter choice means that incoherent effects play a relatively strong role in this problem, which are not well captured by the AME. Thus, similarly to the previous example, the AME is being used here outside of its strict validity domain. We are interested in testing whether it can nevertheless qualitatively capture the correct physical effects. Moreover, direct master equation simulations for such a large system take longer than 24 hours (which is a standard time-window on high-performance clusters), while each quantum trajectory takes less than 24 hours.  We can then exploit many CPU cores to perform many trajectories in parallel. To this end we used $320$ CPU cores and repeated the simulation $16$ times for a total of over $5000$ trajectories.
 
Our simulations (see Fig.~\ref{fig:GoogleGadget}) show how population is lost from the instantaneous ground state to the first excited state near the minimum gap point $s \approx 0.308$.
It also shows a small population revival after the minimum gap is crossed.  As in Sec.~\ref{sec:8qubitchain}, this revival is associated with jumps from the first excited state (or higher states for large $T$) back to the ground state. Encouragingly, despite the perturbative nature of the AME, this revival is qualitatively in agreement with the results of Ref.~\cite{Boixo:2014yu} (see their Fig.~4). The latter work found a stronger revival on the basis of the non-perturbative, non-interacting blip approximation (NIBA), which more accurately captures additional transitions that occur when the energy level broadening is larger than the energy gap between energy levels.  


\section{Simulation cost comparison}
\label{sec:timequantitative}

We now provide a cost comparison between the simulations cost of directly solving the AME and the quantum trajectories method. The first two subsections in this section follow Ref.~\cite{Breuer:2002} closely (while adding some details), and we borrow the notation used in that reference. In subsection~\ref{sec:parallel} we provide a new analysis that reveals that the quantum trajectories method can exhibit a scaling advantage ranging between $O(N)$ and $O(N^2)$ over the direct solution of the AME.

 \subsection{Number of trajectories}
The number of trajectories needed can be found from the standard error of the sample mean. As an example, let us consider the standard error $\hat{\sigma}_{t}$ associated with the instantaneous ground state population  $\langle\psi_{0}(t)|\rho(t)|\psi_{0}(t)\rangle$:
\begin{align}
\hat{\sigma}_{t}^2 &= \frac{1}{R(R-1)}\sum_{r=1}^{R}\left(|\langle\psi_{0}(t)|\psi^{r}(t)\rangle|^2  - \hat{M}_t  \right)^2  \label{eq:stderror}\, ,
\end{align}
where $\ket{\psi^r(t)}$ denotes the state associated with trajectory $r$ at time $t$, $\hat{M}_t = \frac{1}{R}\sum_{r=1}^{R}|\langle\psi_{0}(t)|\psi^{r}(t)\rangle|^2$, and $R$ is the total number of trajectories.  By fixing the value of the standard error $\hat{\sigma}_{t}$, the number of necessary trajectories $R$ can then be determined. 


%
\subsection{Cost comparison}
Since we expect $\hat{\sigma}_{t} \sim \frac{1}{\sqrt{R}}$, let us write
\begin{equation}
\label{eq:factor}
\hat{\sigma}_{t}^2 =  \frac{\lambda_{B}(N)}{R} \sim \frac{1}{R}\,,
\end{equation}
where $\lambda_{B}(N) = \frac{1}{R-1}\sum_{r=1}^{R}(\langle\psi^r(t)| B|\psi^r(t)\rangle  - \hat{M}_t)^2$ for an observable $B$ and mean value $\hat{M}_t = \frac{1}{R}\sum_{r=1}^{R}\langle\psi^{r}(t)|B|\psi^{r}(t)\rangle$. The factor $\lambda_{B}(N)$ is a non-increasing function of the system dimension $N$ \cite{Breuer:2002}: 
\begin{equation}
\label{eq:lambdaB}
\lambda_{B}(N) \sim N^{-x} \,,
\end{equation}
where the scaling $x$ depends on the observable: 
\begin{equation}
0 \left(\text{not self-averaging}\right) \leq x \leq 1 \left(\text{strongly self-averaging}\right) \,.
\end{equation}
Thus, to obtain the same standard error for increasing dimension, the number of trajectories need not be increased in general.  This is another advantage of the trajectories method for growing system dimension. Such a phenomenon has also been observed in time-dependent stochastic density functional theory~\cite{gao2015sublinear}.
%
From Ref.~\cite{Breuer:2002}, the total serial CPU time required for the simulation of the master equation, denoted $T_{\text{AME}}$, versus the stochastic method with $R$ trajectories, denoted $T_{\text{StS}}$, is:
\bes
\label{eq:timecost}
\begin{align}
T_{\text{AME}} &= k_{1} s_{1}(N) N^{\beta} \,, \label{eq:T-AME}\\
T_{\text{StS}} &= k_{2} R(N) s_{2}(N) N^{\alpha} \,,
\label{eq:T-StS}
\end{align}
\ees
%
where $k_1$ and $k_2$ are constants depending on the specific implementation of each method, $s_{1}(N)$ is the total number of evaluations of $\mathcal{L}_{\textrm{WCL}}[\rho(t)]$ [Eq.~\eqref{eqt:ME2-L}] using the master equation method, and $s_{2}(N)$ is the total number of evaluations of $H_{\text{eff}}(t)\ket{\psi(t)}$ [Eq.~\eqref{eq:Heff}] in a single trajectory.

$R(N)$ in Eq.~\eqref{eq:T-StS} is the minimum number of trajectories needed to obtain a standard error lower than a particular chosen value. To account for the constraint that $R(N)\geq 1$, we rewrite Eq.~\eqref{eq:lambdaB} as $\lambda_B(N) = \Lambda_{B} N^{-x}$, and Eq.~\eqref{eq:factor} as:
\begin{equation}
R(N) =
\begin{dcases} 
      \Bigl\lceil \frac{\Lambda_{B} N^{-x}}{\hat{\sigma}_{t}^2} \Bigr\rceil& \text{\space  for } N < N^{*} \\
      1 & \text{\space  for } N\geq N^{*} 
   \end{dcases}
\end{equation}
where $N^{*} =  \lceil\left({\Lambda_{B}}/{\hat{\sigma}_{t}^2}\right)^\frac{1}{x}\rceil$.   
For $x > 0$, the required number of trajectories decreases with $N$ until $N^{*}$, after which one trajectory gives the expectation value within the desired accuracy.

In general, the number of operations needed to evaluate $\mathcal{L}_{\textrm{WCL}}[\rho(t)]$ relative to the number needed to evaluate $H_{\text{eff}}(t)\ket{\psi(t)}$ differs by a factor of $N$, so that $\beta \approx \alpha + 1$, and Eq.~\eqref{eq:timecost} becomes
\bes
\begin{align}
T_{\text{AME}} &= k_1 s_{1}(N) N^{\alpha + 1} \,,\\
T_{\text{StS}} &=
\begin{dcases} 
      k_2' s_{2}(N) N^{\alpha - x} &\text{\space  for } N < N^{*}  \\
      k_{2} s_{2}(N) N^{\alpha} &\text{\space  for }  N\geq N^{*} 
   \end{dcases}
\end{align}
\ees
where 
\begin{equation}\label{eqt:k2prime}
k_2' = k_2\left(\frac{\Lambda_{B}}{\hat{\sigma}_{t}^2}\right) \,,
\end{equation}
and $k_2'$ hence depends on the required accuracy as well. In many situation $s_{1}(N)$ and $s_{2}(N)$ grow with $N$, but they are roughly equal or grow in same manner with $N$. By dividing these two expressions, we can obtain the ratio of $T_{\text{AME}}/T_{\text{StS}}$, 
\begin{equation}
\frac{T_{\text{AME}}} {T_{\text{StS}}} =
\begin{dcases} 
      \frac{k_1  }{k_2' }N^{1 + x} & \text{\space  for }N < N^{*} \\
      \frac{k_1  }{k_2 }N & \text{\space  for } N\geq N^{*} 
   \end{dcases}  \ . 
\end{equation}
%
Since $0\leq x \leq 1$, we can write
\begin{equation} 
\label{eqt:timeComparison}
\begin{aligned}
       \frac{k_1}{k_2'}N &\leq \frac{T_{\text{AME}}}{T_{\text{StS}}} \leq  \frac{k_1}{k_2'}N^2 & \text{\space  for } N < N^{*} \,,\\
     &  \frac{T_{\text{AME}}}{T_{\text{StS}}} = \frac{k_1}{k_2}N & \text{\space for } N\geq N^{*} \,. 
\end{aligned} 
\end{equation}
%

We say that the trajectories method has an advantage over the direct master equation solution if $\frac{T_{\text{AME}}}{T_{\text{StS}}}> 1$. The constant factor $\frac{k_1}{k_2'}$ is typically a small number because it is proportional to the required standard error squared [Eq.~\eqref{eqt:k2prime}]. 
Therefore there is an advantage for the trajectories method when either $N$ is sufficiently large or when a sufficient number of CPU cores $C$ is available (see the next subsection). 
Equation~\eqref{eqt:timeComparison} shows that an advantage
beyond linear in $N$ is attainable for $N<N^\ast$ on a single CPU. The reason is that the number of trajectories needed to achieve a fixed accuracy decreases with increasing system dimension.  For $N>N^\ast$, only one trajectory is required, and the advantage scales as $O(N)$.   

We note that the larger-than-linear advantage only holds if we are interested in estimating operators with the same self-averaging property. This is in contrast to evolving the entire density matrix, as in the AME, which allows the expectation value of any observable to be calculated.  If we demand this same capability from the trajectories approach, then only the linear advantage holds.
 
\subsection{Parallel implementation}
\label{sec:parallel}

The stochastic wave function method is very well-suited for parallel computing implementations. The communication needed between each core is minimal since each trajectory is simulated independently. Assuming $C$ CPU cores are used, where $C \leq R(N)$, we can adjust the time cost [Eq.~\eqref{eq:T-StS}] for the stochastic method to
\begin{equation}
T_{\text{StS}} = k_{2} \frac{R(N)}{C} s_{2}(N) N^{\alpha} \,.
\end{equation}
Note that the number of cores $C$ is held constant, i.e., is independent of the system dimension $N$. Therefore, we can update Eq.~\eqref{eqt:timeComparison} to:
\begin{equation}
\begin{aligned}
       \frac{k_1}{k_2'}C N &\leq \frac{T_{\text{AME}}}{T_{\text{StS}}} \leq  \frac{k_1}{k_2'}C N^2 & \text{\space  for } N < N^{\star} \,,\\
     &  \frac{T_{\text{AME}}}{T_{\text{StS}}} = \frac{k_1}{k_2}  N & \text{\space for } N\geq N^{\star} \,.
      \end{aligned} 
\end{equation}
%
where $N^{\star} =  \lceil\left({\Lambda_{B}}/\left({C \hat{\sigma}_{t}^2} \right) \right)^\frac{1}{x}\rceil$.  Here $N^{\star}$ is the system dimension where $R(N^{\star}) = C$, and one execution of the $C$ parallel CPU cores is enough to obtain the desired standard error.  

Again, the larger-than-linear advantage in $N$ only holds if we are interested in estimating operators with the same self-averaging property, and otherwise we can only expect a linear advantage in $N$.

\section{Conclusion}
In this work, we have shown how quantum trajectories (in the form of quantum jumps) can be unravelled from the adiabatic master equation. We have described and demonstrated a simulation procedure in terms of the waiting time distribution that reproduces the results of the master equation for examples involving $8$ and $16$-qubit systems. 
Direct master equation simulations for the $16$-qubit example would take a long time, but the simulation of the quantum trajectories remains computationally feasible for larger system dimensions by allowing us to simulate many trajectories in parallel. 
A scaling cost comparison of the two methods shows that, generically, the quantum trajectories method yields an improvement by a factor linear in the system dimension $N$ over directly solving the adiabatic master equation. However, the trajectories method can be expected to be up to a factor $c N^2$ faster than a direct simulation of the master equation if only the expectation value of specific self-averaging observables is desired. Here $c$ is a constant proportional to the number of parallel processes and the target standard error.
 
We therefore believe this approach will be particularly useful in enabling the study of larger systems than has been possible using a direct simulation of the AME. 

In addition, the quantum trajectories method offers fresh physical insight into the nature of individual trajectories and their statistics, which may become a helpful tool in interpreting computational bottlenecks in quantum annealing and adiabatic quantum computing.

Finally, while we did not address this in the present work, the quantum trajectories approach is well known to be a convenient path towards continuous measurement and the inclusion of quantum feedback control~\cite{Wiseman:book}. This approach might in the future provide a path towards error correction of adiabatic quantum computing, e.g., by formulating control targets that push the system back to the ground state after diabatic or thermal transitions.

\section{Error estimates}
\label{app:A}
Let us assume that the system is in a pure state at time $t$, i.e., $\rho_S(t) = \ketbra{\psi(t)}$, and let us consider a single time-step. In a single trajectory, the evolution of $\ket{\psi(t)}$ involves two possibilities: no jump or a jump. The ensemble average of trajectories after one finite time-step mainly involves two kinds of errors: the error associated with the norm of the state vector (Sec.~\ref{sssec:en}), and the error associated with the probability elements in a finite time-step (Sec.~\ref{sssec:ep}).

\subsection{Error associated with the norm squared of a no-jump trajectory}
\label{sssec:en}
The Schr\"{o}dinger equation of the effective Hamiltonian in the case of a no-jump trajectory is given by
%
\begin{equation}
\label{eqt:Schrapp2}
\frac{d\ket{\psi(t)}}{dt} = -i H_{\text{eff}}(t) \ket{\psi(t)} \ .
\end{equation}
%
The resulting state after one time-step $\Delta t$ is:
%
\begin{equation}
\label{eqt:euler} 
\ket{\tilde{\psi}(t+\Delta t)} =V_{\text{eff}}(t+\Delta t, t)\ket{\psi(t)}  \ ,
\end{equation}
%
where 
\beq 
V_{\text{eff}}(t+\Delta t, t) = {\cal T}\exp\left[-i\int_t^{t+\Delta t}H_{\text{eff}}(t')dt'\right]
\eeq 
is a non-unitary contractive evolution operator ($\vertiii{ V_{\text{eff}}(t+\Delta t, t)} \leq 1$ for every induced norm) and $\ket{\tilde{\psi}(t+\Delta t)}$ is unnormalized since $H_{\text{eff}}(t)$ is not hermitian.
%
We can expand the time-ordered exponential for $V_{\text{eff}}(t+\Delta t, t)$ as
%
\begin{align}
\label{Eqt: TDtaylor}
&{}{\cal T}\exp\left[-i\int_t^{t+\Delta t}H_{\text{eff}}(t')dt'\right]    \\
&=\mathds{1} - i \int_{t}^{t+\Delta t} dt' H_{\text{eff}}(t')   + \left(-i\right)^2 \frac{1}{2!} \mathcal{T}\left(\int_{t}^{t+\Delta t} dt' H_{\text{eff}}(t')\right)^2 +
\left(-i\right)^3 \frac{1}{3!}\mathcal{T}\left(\left(\int_{t}^{t+\Delta t} dt' H_{\text{eff}}(t')\right)^3\right) \cdots \nonumber
\end{align}
%
For any $H_{\text{eff}}(t)$ that is $C^{K}$ on an open interval containing $[0, t_f]$ ($H^{(k)}_{\text{eff}}(t)$ is continuous and bounded for $1\leq k \leq K$):
%
\begin{equation}
\int_{t}^{t+\Delta t} dt' H_{\text{eff}}(t') = 
\sum\limits_{k = 0}^{K-1}\frac{H^{(k)}_{\text{eff}}(t)}{(k+1)!}(\Delta t)^{k+1} + O((\Delta t)^{K+1})\, ,
\end{equation}
%
as $\Delta t \rightarrow 0$. Assume $H_{\text{eff}}(t)$ is $C^{K}$ and $K \geq 2$. Let $\dot{H}_{\eff}(t)\equiv H^{(1)}_{\text{eff}}(t)$ denote the time derivative of $H_\eff(t)$.
We have:
%
\bes
\begin{align}
\label{Eqt: integral}
\int_{t}^{t+\Delta t} dt' H_{\text{eff}}(t')&= H_{\text{eff}}(t)\Delta t + \frac{1}{2!}\dot{H}_{\text{eff}}(t) (\Delta t)^2 + O((\Delta t)^3) \,,\\
\mathcal{T}\left(\int_{t}^{t+\Delta t} dt' H_{\text{eff}}(t')\right)^2 &= 2\int_{t}^{t+\Delta t} dt' H_{\text{eff}}(t')  \int_{t}^{t'} dt'' H_{\text{eff}}(t'') \nonumber\\
&= H_{\text{eff}}(t)^2(\Delta t)^2 + \frac{1}{2}H_{\text{eff}}(t)\dot{H}_{\text{eff}}(t)(\Delta t)^3 + \frac{1}{2}\dot{H}_{\text{eff}}(t)H_{\text{eff}}(t)(\Delta t)^3 + O((\Delta t)^4)\ \,, \\
\mathcal{T}\left(\int_{t}^{t+\Delta t} dt' H_{\text{eff}}(t')\right)^3 &= H_{\text{eff}}(t)^3(\Delta t)^3 + O((\Delta t)^4) \,.
\end{align}
\ees
%
Therefore, we have, to second order in $\Delta t$:
%
\beq
\label{eq:A7}
V_{\text{eff}}(t+\Delta t, t) = \mathds{1} -i \left( H_{\text{eff}}(t)\Delta t + \frac{1}{2!}\dot{H}_{\text{eff}}(t) (\Delta t)^2 \right) + \left(-i\right)^2 \frac{1}{2!} H_{\text{eff}}(t)^2(\Delta t)^2  + O((\Delta t)^3)\ ,
\eeq
%
so that:
%
\begin{align}
&{} V^{\dagger}_{\text{eff}}(t+\Delta t, t) V_{\text{eff}}(t+\Delta t, t) \nonumber \\
=&{}  \mathds{1} + i\Delta t \left(H^{\dagger}_{\text{eff}}(t) - H_{\text{eff}}(t)\right) 
+ \frac{1}{2!}(\Delta t)^2\left[ i\dot{H}^{\dagger}_{\text{eff}}(t) - i\dot{H}_{\text{eff}}(t) 
- \left(H^{\dagger 2}_{\text{eff}}(t) + H^2_{\text{eff}}(t)\right)\right] + O((\Delta t)^3) \ . 
\end{align}
%
We approximate $N(t,\Delta t)\equiv \|\ket{\tilde{\psi}(t+\Delta t)} \|^2$ by:
%
\beq
\label{Eqt: Step2}
N(t,\Delta t) = \braket{\tilde{\psi}(t+\Delta t)|\tilde{\psi}(t+\Delta t)} 
\approx \bra{\psi(t)}\left(\mathds{1} + i \Delta t\left(H^{\dagger}_{\text{eff}}(t) - H_{\text{eff}}(t) \right)\right)\ket{\psi(t)} \equiv E(t,\Delta t)\, .
\eeq
%
The approximation error is given by:
%
\bes
\begin{align}
\delta (t,\Delta t) &\equiv N(t,\Delta t)-E(t,\Delta t)\\
 &= \frac{1}{2}(\Delta t)^2\bra{\psi(t)}\left[ i\dot{H}^{\dagger}_{\text{eff}}(t) - i\dot{H}_{\text{eff}}(t) 
- \left(H^{\dagger 2}_{\text{eff}}(t) + H^2_{\text{eff}}(t)\right)\right] \ket{\psi(t)}+ O((\Delta t)^3) \\
&\leq \frac{(\Delta t)^2}{2}\vertiii{i(\dot{H}^{\dagger}_{\text{eff}}(t) - \dot{H}_{\text{eff}}(t)) - ( H^{\dagger 2}_{\text{eff}}(t) + H^2_{\text{eff}}(t))} + \vertiii{O((\Delta t)^3)}\ ,
\label{Eqt: errornorm}
\end{align}
\ees
%
where $\|\cdot\|$ is the operator norm (largest singular value).


Eq.~\eqref{Eqt: errornorm} gives the relation between the error of the norm square approximation and the time-step. It is also helpful to consider the sources of error here as they will be used later. This error mainly arises from two sources during the truncations of Taylor expansion: 
%
\begin{enumerate}
\item The truncation of the Taylor expansion of the integral [Eq.~\eqref{Eqt: integral}] to keep only $H_{\text{eff}}(t)\Delta t$. This turns Eq.~\eqref{Eqt: TDtaylor} into $\exp\left(-iH_{\text{eff}}(t)\Delta t\right)$.  For this to hold, we require 
\begin{align}
\label{Eqt: case1}
\left\lVert \frac{1}{2}\dot{H}_{\text{eff}}(t) (\Delta t)^2 
+ O((\Delta t)^3) \right\rVert \ll  \lVert H_{\text{eff}}(t)\Delta t \rVert \, ,
\end{align}
%
implying:
%
\begin{align}
\Delta t \ll 2\frac{\vertiii{H_{\text{eff}}(t)}}{\vertiii{\dot{H}_{\text{eff}}(t)}}  \, ,
\label{Eqt: 1stcon}
\end{align}
assuming $\dot{H}_{\text{eff}}(t)\neq 0$; if it is then the condition becomes $\Delta t \ll \left(\frac{K!\vertiii{H_{\text{eff}}(t)}}{\vertiii{{H^{(K)}_{\text{eff}}(t)}}}\right)^{1/K}$ for the lowest value of $K$ such that $H^{(K)}_{\text{eff}}(t)\neq 0$, where the superscript denotes the $K$-th derivative.

\item Keeping only the first order term in Eq.~\eqref{eq:A7} afterwards, i.e., $\mathds{1} - iH_{\text{eff}}(t)$.  
This requires, in addition to Eq.~\eqref{Eqt: 1stcon}:
%
\begin{align}
\label{Eqt: case2}
\left\lVert\frac{1}{2}H^2_{\text{eff}}(t)(\Delta t)^2 + O((\Delta t)^3)
\right\rVert \ll  \vertiii{H_{\text{eff}}(t)\Delta t} \, ,
\end{align}
%
\end{enumerate}
implying, for all $t$ such that the denominators do not vanish:
 \beq 
 \label{eqt:Deltat2}
 \Delta t \ll  \min \left\{ \frac{\vertiii{H_{\text{eff}}(t)}}{\vertiii{\dot{H}_{\text{eff}}(t)}}, \frac{1}{\vertiii{H_{\text{eff}}(t)}} \right\} \ ,
 \eeq
where we ignored the factor of $2$.
%
In conclusion, the norm after one time-step is related to the jump probabilities as:
\bes
\begin{align}
N(t,\Delta t) &= 
 \bra{\psi(t)}\left(\mathds{1} + i (\Delta t)\left(H^{\dagger}_{\text{eff}}(t) - H_{\text{eff}} \right)\right)\ket{\psi(t)} \notag \\
 &\qquad + \delta(t,\Delta t) \\
&= 1 - \Delta t \sum\limits_{i}\braket{{A}_{i}^{\dagger}(t) {A}_{i} (t)} + \delta(t,\Delta t) \\
&= 1 - \Delta p(t) + \delta(t,\Delta t) \,,\label{Eqt: squareofnorm}
\end{align}
\ees
where we used Eq.~\eqref{eq:Heff} and defined the (approximate) jump probabilities as:
 \bes
 \label{Eqt: typeofprob}
\begin{align}
&{}\Delta p(t)  = \sum_i \Delta p_i(t) \\
&{}\Delta p_i(t) = \Delta t \braket{ {A}_{i}^{\dagger}(t) {A}_{i} (t)}  \, .
\label{eqt:typeofprob}
\end{align}
\ees
This explains Eqs.~\eqref{eqt:squareofnorm} and~\eqref{eq:jumprate}.

%%%%%%%%%%%%%%%%
\subsection{Error associated with probability elements}
\label{sssec:ep}
We have defined the $\Delta p_i(t)$ and $\Delta p(t)$ in a fixed time-step in Eq.~\eqref{Eqt: typeofprob}.
Note that even in the time-independent case, where both the Hamiltonian and Lindblad operators are time-independent, $1- \Delta p(t)$ is never exactly equal to the norm squared of the state vector after one time-step, and $\Delta p_i(t)$ is not exactly the jump probability inside the time-step. They are only approximations. 
%

For a finite time-step $\Delta t$, with $p_0$ the probability of having no jump inside the interval $[t, t+\Delta t]$ and $p_1$ the probability of having one jump inside the interval $[t, t+\Delta t]$, we have:
\beq
p_{0} = e^{-\int_t^{t+\Delta t} \lambda(t') dt'} = 1-p_{1}  \,.
\label{eq:p_0}
\eeq
%
Note that as $\Delta t \rightarrow 0$, $p_{0} = 1 - \lambda(t)\Delta t + o(\Delta t)$, $p_{1} \simeq \lambda(t)\Delta t$.
We shall focus on the case where the time-step is sufficiently small such that the probability of two or more jumps occurring within a single time-step is negligible.\footnote{E.g., the quantum jump can be described by a Poisson process with a state-dependent inhomogeneous jump rate, with two or more jumps as successive one and no-jump processes, and $\sum_{n\geq 2}p_{n} = o(\Delta t)$ as $\Delta t\rightarrow 0$.} 

First, we can expand the exponential as
%
\begin{align}
p_0 
&=1 - \int_t^{t+\Delta t} 
\lambda(t')dt' + \frac{1}{2}\left(\int_t^{t+\Delta t} \lambda(t') dt'
\right)^2 \cdots \nonumber
\end{align}
%
During the time window from $t$ to $t+\Delta t$, $\lvert\psi(t')\rangle$ [required to calculate $\lambda(t')$] is obtained by solving the Schr\"{o}dinger equation with the effective Hamiltonians [Eq.~\eqref{eqt:Schrapp2}] and renormalizing the solution during the integration. As we show in Sec.~\ref{sec:C}, in any finite interval the norm squared of the unnormalized state vector [Eq.~\eqref{Eqt: Step2}] is equal to $p_0$. This is the reason why we can use the waiting time distribution (or Gillespie algorithm~\cite{gillespie1977exact}) as our simulation method in the main text.

Second, since
%
\begin{align}
\int_{t}^{t+\Delta t} dt' \lambda(t') = \sum\limits_{k = 0}^{\infty}\frac{\lambda^{(k)}(t)}{(k+1)!}(\Delta t)^{k+1} \ ,
\end{align}
we have
%
\begin{align}
\label{eqt:p0allterms}
= 1 - \lambda(t)\Delta t + e_p \ ,
\end{align} 
where the error $e_p$ associated with the probability elements in a fixed time-step is:
%
\begin{equation}
e_p = - \frac{1}{2}\frac{d}{dt}
\lambda(t)(\Delta t)^2 + \frac{1}{2}
\lambda^2(t)(\Delta t)^2 + O((\Delta t)^3) \,.
\end{equation}
%
This should be much smaller than the first order term $\lambda(t) \Delta t$. Therefore, we need 
%
\begin{align}
\Delta t \ll \left|\frac{ \lambda(t) }{  \lambda^2(t)-\frac{d}{dt} \lambda(t)}\right|  \, .
\label{Eqt: Poissoncon}
\end{align}
%
In the time-independent case, this reduces to 
\beq
\Delta t \ll \frac{1}{ \lambda} \ .
\eeq

\section{Proof of equivalence between the master equation and trajectories formulations}
\label{app:B}

Our goal in this section is to show how the master equation, Eq.~\eqref{eqt:effdiagonalform}, can be recovered from the quantum trajectories formulation, and to find a bound on the time-step $\Delta t$. This generalizes the proof for the time-independent case found in~\cite{molmer1993monte}.

%
\subsection{To jump or not to jump}
\label{sssec:2}
The probability elements $\Delta p(t)$ and $\Delta p_i (t)$ are important for determining whether a jump occurs and if a jump does occur, which jump type occurs. 
In order to determine if a jump occurs or not, we draw a random number $\epsilon$, uniformly distributed between 0 and 1. If $\Delta p(t) < \epsilon$, which is almost always the case since $\Delta p(t)$ is very small, no jump occurs. In the case of no jump, $\ket{\psi(t)}$  evolves according to the effective Schr\"{o}dinger equation, Eq.~\eqref{eqt:Schrapp2}. At time $t+\Delta t$ we simply renormalize the solution of Eq.~\eqref{eqt:euler}:
\bes
\begin{align}
\left|\psi(t + \Delta t)\right> &= \frac{1}{\sqrt{\braket{\tilde{\psi}(t+\Delta t)| \tilde{\psi}(t+\Delta t)}}}\ket{\tilde{\psi}(t+\Delta t)}\\&\stackrel{\eqref{Eqt: squareofnorm}}{=} \frac{1}{\sqrt{1 - \Delta p(t) + \delta}}\ket{\tilde{\psi}(t+\Delta t)} \ .
\end{align}
\ees

If $\Delta p(t) > \epsilon$, the state undergoes an abrupt jump and we choose the new wavefunction among the different states $A_{i}\ket{\psi(t)}$ and renormalize:
%
\bes
\begin{align}
\left|\psi(t + \Delta t)\right> &= \frac{{A}_{i}(t)\ket{\psi(t)}}{\sqrt{\bra{\psi(t)} {A}_{i}^{\dagger}(t) {A}_{i} (t)\ket{\psi(t)}}} \\
&\stackrel{\eqref{eqt:typeofprob}}{=} 
\sqrt{\frac{\Delta t}{\Delta p_i(t)}} {A}_{i}(t)\ket{\psi(t)}\ .
\end{align}
\ees
%
Which type of jumps occurs is determined according to the probability 
\bes
\begin{align}
\Pi_i(t) &= \frac{\Delta p_i(t)}{\Delta p(t)} = \frac{\braket{\psi(t)|{A}_{i}^{\dagger}(t){A}_{i}(t)|\psi(t)}\Delta t}{\sum\limits_{i}\braket{\psi(t)|{A}_{i}^{\dagger}(t){A}_{i}(t)|\psi(t)}\Delta t} \\
&= \frac{\braket{{A}_{i}^{\dagger}(t){A}_{i}(t)}}{\lambda(t)}\ ,
\label{eq:Pi(t)}
\end{align}
\ees
where 
\beq
\lambda(t) = \sum_{i}\langle {A}_{i}^{\dagger}(t){A}_{i}(t)\rangle 
\label{eq:lambda}
\eeq
is the time-dependent jump rate.


\subsection{Averaging over trajectories}
\label{sssec:3}

Let $H_{\text{eff}}(t)$ be $C^{K}$ with $K \geq 2$. 
We first express the mean value $\bar{\sigma}_{S}(t)$ as a sum over the non-Hermitian evolution [with probability $1 - \Delta p(t)$] and the jump trajectories [with probability $\Delta p(t)$], so that as $\Delta t \rightarrow 0$ we have: 
%
%
\bes
\begin{align}
\label{Eqt: averaging}
\bar{\sigma}_{S}(t + \Delta t) 
&= \left[1 - \Delta p(t)\right]\frac{\ket{\tilde{\psi}(t + \Delta t)}}{\sqrt{1 - \Delta p(t) + \delta}}\frac{\bra{\tilde{\psi}(t + \Delta t)}}{\sqrt{1 - \Delta p(t) + \delta}}  \nonumber \\
& + \Delta p(t) \sum\limits_{i} \Pi_{i}(t) \sqrt{\frac{\Delta t}{\Delta p_i(t)}}{A}_{i}(t)  \ket{\psi(t)}\sqrt{\frac{\Delta t}{\Delta p_i(t)}}\bra{\psi(t)}{A}_{i}^{\dagger}(t) \\
&\stackrel{\eqref{eq:Pi(t)}}{=}   \frac{1 - \Delta p(t)}{1 - \Delta p(t) + \delta}\ket{\tilde{\psi}(t + \Delta t)}\bra{\tilde{\psi}(t + \Delta t)}
+ \Delta t \sum\limits_{i}{A}_{i}(t)\sigma_{S}(t){A}_{i}^{\dagger}(t) 
\label{Eqt: noninnerproductform}
\end{align}
\ees
%
Combining Eq.~\eqref{eqt:euler} with Eq.~\eqref{eq:A7} we have:
\beq
\ket{\tilde{\psi}(t+\Delta t)} =
\left[ \mathds{1} -i \left( H_{\text{eff}}(t)\Delta t + \frac{1}{2!}\dot{H}_{\text{eff}}(t) (\Delta t)^2 \right) + \left(-i\right)^2 \frac{1}{2!} H_{\text{eff}}(t)^2(\Delta t)^2  + O((\Delta t)^3) \right] \ket{\psi(t)}  \ .
\eeq
Recall that in Eq.~\eqref{eqt:Deltat2} we gave conditions allowing us to neglect the $O((\Delta t)^2)$ terms.
Thus: 
\begin{align}
\label{eq:B3}
\bar{\sigma}_{S}(t + \Delta t) 
&=  \frac{1 - \Delta p(t)}{1 - \Delta p(t) + \delta}\left( \mathds{1} - i H_{\text{eff}}(t) \Delta t 
+ O((\Delta t)^2)\right)\bar{\sigma}_{S}(t) \left(\mathds{1} + i H^{\dagger}_{\text{eff}}(t) \Delta t
+O((\Delta t)^2)\right)\\
&\phantom{==}+ \Delta t \sum\limits_{i}{A}_{i}(t)\bar{\sigma}_{S}(t){A}_{i}^{\dagger}(t)\nonumber  \, .
%%%%%%
\end{align} 
\begingroup
\allowdisplaybreaks
%
where we have replaced $\sigma_{S} (t)$ by $\bar{\sigma}_{S} (t)$ after averaging over many trajectories. 
Rearranging this expression into a form that exposes the terms that will become the master equation,
the expression for the averaged state at $t + \Delta t$ becomes:
\bes
\begin{align}
\bar{\sigma}_{S}(t + \Delta t) &= \bar{\sigma}_{S}(t) + i\Delta t\left(\bar{\sigma}_{S}(t)H_{\text{eff}}^{\dagger}(t) - H_{\text{eff}}(t)\bar{\sigma}_{S}(t) \right)+ \Delta t \sum_{i} {A}_{i}(t) \bar{\sigma}_{S}(t){A}_{i}^{\dagger}(t) \\
&\phantom{==}
- \frac{\delta}{1 - \Delta p(t) + \delta} \left[ \bar{\sigma}_{S}(t) +  i\bar{\sigma}_{S}(t)\left(H_{\text{eff}}^{\dagger}(t) -H_{\text{eff}}(t)\right) \bar{\sigma}_{S}(t) \Delta t \right] + O((\Delta t)^2)\ .
\label{eq:B5b}
\end{align}
\ees
%
%
Note that $\delta$ is $O((\Delta t)^2)$ as $\Delta t \rightarrow 0$ [Eq.~\eqref{Eqt: errornorm}], and $\Delta p(t) = \Delta t \sum_{i}\braket{\psi(t)|{A}_{i}^{\dagger}(t){A}_{i}(t)|\psi(t)}$ is $O(\Delta t)$ as $\Delta t \rightarrow 0$, so that:
%
\bes
\begin{align}
\frac{\delta}{1 - \Delta p(t) + \delta} &= 
\frac{O((\Delta t)^2)}{1 - O(\Delta t) + O((\Delta t)^2)} \\
&=O((\Delta t)^2)\, . 
\end{align} 
\ees
%
Therefore line~\eqref{eq:B5b} can be absorbed into $O((\Delta t)^2)$, and we are left with:
\begin{align}
\frac{\bar{\sigma}_{S}(t + \Delta t) - \bar{\sigma}_{S}(t)}{\Delta t} =&
-i\left(H_{\text{eff}}(t)\bar{\sigma}_{S}(t) - \bar{\sigma}_{S}(t)H_{\text{eff}}^{\dagger}(t) \right)\notag \\
&+  \sum_{i} {A}_{i}(t) \bar{\sigma}_{S}(t){A}_{i}^{\dagger}(t) 
+ O(\Delta t) \ ,
\end{align}
which becomes the master equation, Eq.~\eqref{eqt:effdiagonalform}, in the $\Delta t \to 0$ limit.


\subsection{Upper bound on $\Delta t$}
\label{ssec:upperbound}
The above proof takes $\Delta t \rightarrow 0$. We would like to know how small the time-step $\Delta t$ should be in order for the approximations made to be valid. In Eq.~\eqref{eq:B3}, we expanded the time-ordered exponential, and kept only the first order terms. This is equivalent to the criteria in Eqs.~\eqref{Eqt: case1} and ~\eqref{Eqt: case2}, summarized as a single condition in Eq.~\eqref{eqt:Deltat2}. 
As shown in Sec.~\ref{sssec:en}, this also automatically makes the error in the norm squared approximation $\delta$ small. We also need to satisfy Eq.~\eqref{Eqt: Poissoncon}, in order to accurately approximate the probability elements. Taken together, therefore:
 \beq 
 \Delta t \ll  \min \left\{ \frac{\vertiii{H_{\text{eff}}(t)}}{\vertiii{\dot{H}_{\text{eff}}(t)}}, \frac{1}{\vertiii{H_{\text{eff}}(t)}}, \left|\frac{ \lambda(t) }{  \lambda^2(t)-\dot \lambda(t)}\right| \right\} \ .
 \label{eq:B7}
 \eeq
In practice, choosing a constant time-step that satisfies Eq.~\eqref{eq:B7} in the whole timespan $[0, t_f]$ is sufficient, though one might prefer to implement an adaptive time-step tailored to the instantaneous value of the R.H.S. 
%%%%%%%%%%%%%%%%
\section{On the validity of waiting times (quantum time-dependent operators)}
\label{sec:C}
Here we show the validity of using the waiting time distribution in the case of time-dependent operators. The argument presented here is based on Ref.~\cite{Breuer:2002} and we extend it to the time-dependent case.

Let us denote by $\ket{\psi(t)}$ and $\ket{\tilde{\psi}(t)}$ the normalized and unnormalized state vectors respectively, and let us assume they are equal at time $t$. This can happen when $t = 0$ or any time immediately after each jump. Let $t^+ \equiv t+\tau$, where $\tau$ can be as large as is possible until the next jump occurs,  and
\begin{equation}
V_{\text{eff}}(t^+, t) = {\cal T}\exp\left[-i\int_t^{t^+}H_{\text{eff}}(t')dt'\right] \ ,
\end{equation}
Then:
%
\bes
\begin{align}
\ket{\tilde{\psi}(t + \tau)} &=  
 V_{\text{eff}}(t^+, t)\ket{\psi(t)}  \ ,\\
\ket{\psi(t^+)} &=  
 \frac{V_{\text{eff}}(t^+, t)\ket{\psi(t)}}{\left\lVert V_{\text{eff}}(t^+, t)\ket{\psi(t)} \right\rVert} \,.
 \label{eq:C2b}
\end{align}
\ees
%
Then, starting from $t$, for any future $t^{+} > t$, we have
%
\bes
\begin{align}
\frac{d\phantom{,}}{dt^{+}}\left\lVert \ket{\tilde{\psi}(t^{+})} \right\rVert^2 &= \phantom{}\frac{d\phantom{,}}{dt^{+}}\left\lVert{\cal T}\exp\left[-i\int_t^{t^+}H_{\text{eff}}(t')dt'\right]\ket{\psi(t)}\right\rVert^2 \\
&= \frac{d\phantom{,}}{dt^{+}}\bra{\psi(t)}V_\eff^{\dagger}(t^+,t) V_\eff(t^+,t)\ket{\psi(t)} \\
&=\bra{\psi(t)}V_\eff^{\dagger}(t^+,t)(+i)H^{\dagger}_{\text{eff}}(t^{+})V_\eff^{}(t^+,t)\ket{\psi(t)} +
\bra{\psi(t)}V_\eff^{\dagger}(t^+,t)(-i)H_{\text{eff}}(t^{+})V_\eff^{}(t^+,t)\ket{\psi(t)} \\
&=-\bra{\psi(t)}V_\eff^{\dagger}(t^+,t)\left(\sum\limits_{i}{A}^{\dagger}_{i}(t^{+}){A}_{i}(t^{+})\right)V_\eff^{}(t^+,t)\ket{\psi(t)} \\
&=  -\left\lVert V_{\text{eff}}(t^{+}, t)\ket{\psi(t)} \right\rVert^2 \sum\limits_{i} \bra{\psi(t^{+})} {A}^{\dagger}_{i}(t^{+}){A}_{i}(t^{+}) \ket{\psi(t^{+})}  \, ,
\end{align}
\ees
%
%
where in the last equality we used Eq.~\eqref{eq:C2b}.

%
Let $N(t^{+}) \equiv \| \ket{\tilde{\psi}(t^{+})} \|^2$, as in Eq.~\eqref{Eqt: Step2}.  We have
% 
\begin{equation}
\frac{d\phantom{,}}{dt^{+}} N(t^{+}) = -N(t^{+})  \lambda(t^+)   \, ,
\end{equation}
%
where $\lambda$ is the time-dependent jump rate [Eq.~\eqref{eq:lambda}].
The solution to this differential equation with the initial condition $N(t) = 1$ is
%
\begin{equation}
N(t^{+}) = \exp\left(-\int_t^{t^{+}} \lambda(t') dt'\right) = p_0(t^{+})  \, ,
\end{equation}
where $p_0$ is the probability of not having any jump inside the interval [Eq.~\eqref{eq:p_0}], which we have now shown to be equal to the the norm squared of the unnormalized state vector for any finite interval $[t, t+\tau]$. 

No commutators of operators at different times appears in the derivation. The use of the waiting time distribution is therefore valid for time-dependent operators as long as the correlation matrix is positive.

\section{Effect of the annealing schedule on the $8$-qubit chain example} 
\label{app:Chain}

We provide the functional form for the (D-Wave 1) annealing schedule functions $A(t)$ and $B(t)$ used in Sec.~\ref{sec:8qubitchain} in Fig.~\ref{fig:5a}.  We compare this non-linear schedule to a linear annealing schedule with an overall energy scale chosen to closely match the energy scale at which the first annealing schedule curves cross.  The dynamics associated with the linear annealing schedule [shown in Fig.~\ref{fig:5b}] is somewhat different than the non-linear one. This can be attributed to the differences between the two schedules. In order to ensure that the two sets of schedules intersect at the same energy scale, this requires the linear schedule to start from a significantly smaller energy scale.  This results in some important effects on the dynamics.  First, this energy scale is not large enough to ensure that the thermal state at $s = 0$ has negligible weight on excited states.  Since we use the ground state as the initial state of the simulation, which is now sufficiently different from the thermal state at $s=0$, the dissipative dynamics causes visible changes in the state immediately, which can be see as both the dip in Fig~\ref{fig:5a} near $s=0$ and the large number of excitations at the beginning of the anneal in Fig.~\ref{fig:5c}.  Second, even after this initial dip, the lower energy scale associated with the linear schedule means that thermal depopulation of the ground state occurs generally sooner relative to the non-linear schedule studied in the main text, although at a lower rate because of the linear form of the schedule.  Furthermore, because the transverse field remains significant compared to the Ising term for longer in the anneal than in the linear case, repopulation of the ground state due to thermal relaxation occurs for a longer period of time.  However, ultimately, the ground state probability at the end of the anneal is not significantly different than that shown in Fig.~\ref{fig:3qubits8qubits}. The jump statistics are shown in Fig.~\ref{fig:5c}, and closely resemble the non-linear case shown in the inset of Fig.~\ref{fig:8qubitssingle}.

\begin{figure*}[htb!] %  figure placement: here, top, bottom, or page
\centering
\subfigure[\ ]{\includegraphics[width=0.32\textwidth]{qt/AnnealingSchedules}\label{fig:5a}} 
\subfigure[\ ]{\includegraphics[width=0.32\textwidth]{qt/EnergyPop_8Qubit_tf=10us_T=20mK_LinearSchedule_8GHz_v1}\label{fig:5b}} 
\subfigure[\ ]{\includegraphics[width=0.32\textwidth]{qt/BarPlot_8Qubit_tf=10us_T=20mK_LinearSchedule_8GHz}\label{fig:5c}} 
\caption{(a): Dotted lines: Linear schedule; Solid lines: D-Wave schedule used in Fig.~\ref{fig:3qubits8qubits}; (b): Same as in Fig.~\ref{fig:3qubits8qubits} (the evolution of the population in the instantaneous ground state for the $8$-qubit problem), but with a linear schedule. Inset: the convergence of the ground state population towards the AME results. (c): A histogram of the net number of jumps to the instantaneous ground state (GS). It shares the same pattern as in the non-linear schedule case (the inset of Fig.~\ref{fig:8qubitssingle}), but the net number of jumps out of the ground state is smaller due to the smaller energy scale in the linear schedule.}
\label{fig:8qubitslinear}
\end{figure*}
%


\section{Proof that eigenstates of $H_S$ are modified only under jumps}
\label{app:eigenstate-proof}

Recall that the Lindblad operators are defined in Eq.~\eqref{eq:Lindblad2} of the main text as:
\begin{align}
L_{\alpha, \omega}(t) &= \sum_{a,b} \delta_{\omega, \eps_b(t) - \eps_a(t)} \bra{\eps_a(t)} A_\alpha \ket{\eps_b(t)} 
| \eps_a(t) \rangle  \langle \eps_b(t)| \,.
\end{align}
After inverting Eq.~\eqref{eq:L} we have 
\begin{equation}
A_{i,\omega}(t) = \sum_{\alpha}u^{*}_{i,\alpha}(\omega)L_{\alpha, \omega}(t) 
\end{equation}
for the new Lindblad operators corresponding to a diagonalized $\gamma$ matrix of decay rates.

Assume for simplicity that the $\gamma$ matrix is already diagonal, so that $u$ is just an identity transformation and $i$ is a relabeling of $\alpha$; then
\begin{align}
A_{i,\omega}(t) &= \sum_{a,b} \delta_{\omega, \eps_b(t) - \eps_a(t)} \bra{\eps_a(t)} A_\alpha \ket{\eps_b(t)} 
| \eps_a(t) \rangle  \langle \eps_b(t)| \nonumber \\
A^{\dagger}_{i,\omega}(t) &= \sum_{a,b} \delta_{\omega, \eps_b(t) - \eps_a(t)} \bra{\eps_b(t)} A_\alpha \ket{\eps_a(t)} 
| \eps_b(t) \rangle  \langle \eps_a(t)| \,.
\end{align}

Consider the drift term 
\[
-\frac{1}{2}\sum_{i} \left[ A_{i}^{\dagger}(t)A_{i}(t) - \braket{A_{i}^{\dagger}(t)A_{i}(t)}\right]\ket{\psi(t)}dt\ .
\] 
Since $A_i(t)$ comes from the redefinition where the index $i$ includes the Bohr frequencies [Eq.~\eqref{eqt:Aired}]: $\sqrt{\gamma'_i(\omega)}A_{i,\omega}(t)\rightarrow A_i(t)$, the drift term becomes the following after we reintroduce the Bohr frequencies:
%
\begin{equation}
- \frac{1}{2}\sum_{i}\sum_{\omega} \gamma'_i(\omega)\left[ A_{i,\omega}^{\dagger}(t)A_{i,\omega}(t) - \bra{\psi(t)} A_{i,\omega}^{\dagger}(t)A_{i,\omega}(t) \ket{\psi(t)} \right]\ket{\psi(t)}dt \,. 
\label{eq:explicit}
\end{equation}

\subsection{When $\ket{\psi(t)}$ is an eigenstate of $H_{S}(t)$}
If the $\ket{\psi(t)}$ is an eigenstate of $H_{S}(t)$ (denoted as $\ket{\eps_b(t)}$ here),
\begin{align}
A_{i,\omega}(t)\ket{\psi(t)} = A_{i,\omega}(t)\ket{\eps_b(t)} &=  \sum_{a} \delta_{\omega, \eps_b(t) - \eps_a(t)} \bra{\eps_a(t)} A_\alpha \ket{\eps_b(t)} 
| \eps_a(t) \rangle \nonumber \\
\bra{\psi(t)}A^{\dagger}_{i,\omega}(t) = \bra{\eps_b(t)}A^{\dagger}_{i,\omega}(t) &= \sum_{a} \delta_{\omega, \eps_b(t) - \eps_a(t)} \bra{\eps_b(t)} A_\alpha \ket{\eps_a(t)} \langle \eps_a(t)| \,.
\end{align}

Concentrate on the term of the parenthesis inside each summation of Eq.~\eqref{eq:explicit}, i.e.
\begin{equation}
\left[ A_{i,\omega}^{\dagger}(t)A_{i,\omega}(t) - \bra{\eps_b(t)} A_{i,\omega}^{\dagger}(t)A_{i,\omega}(t) \ket{\eps_b(t)}  \right]\ket{\eps_b(t)} \,.
\label{eq:paraterm}
\end{equation}
The first term is:
\begin{align}
&\phantom{{}={}} A_{i,\omega}^{\dagger}(t) A_{i,\omega}(t)\ket{\eps_b(t)}  \nonumber\\
&= \left(\sum_{a^{\prime},b^{\prime}} \delta_{\omega, \eps_{b^{\prime}}(t) - \eps_{a^{\prime}}(t)} \bra{\eps_{b^{\prime}}(t)} A_\alpha \ket{\eps_{a^{\prime}}(t)} 
| \eps_{b^{\prime}}(t) \rangle  \langle \eps_{a^{\prime}}(t)| \right) \sum_{a} \delta_{\omega, \eps_b(t) - \eps_a(t)} \bra{\eps_a(t)} A_\alpha \ket{\eps_b(t)} 
| \eps_a(t) \rangle \nonumber\\
&= \sum_{a,b^{\prime}} \delta_{\omega, \eps_{b^{\prime}}(t) - \eps_{a}(t)} \delta_{\omega, \eps_b(t) - \eps_a(t)}\bra{\eps_{b^{\prime}}(t)} A_\alpha \ket{\eps_{a}(t)}  \bra{\eps_a(t)} A_\alpha \ket{\eps_b(t)}
| \eps_{b^{\prime}}(t) \rangle  \nonumber\\
&= \sum_{a,b^{\prime}} \delta_{0, \eps_{b^{\prime}}(t) - \eps_{b}(t)} \delta_{\omega, \eps_b(t) - \eps_a(t)}\bra{\eps_{b^{\prime}}(t)} A_\alpha \ket{\eps_{a}(t)}  \bra{\eps_a(t)} A_\alpha \ket{\eps_b(t)}
| \eps_{b^{\prime}}(t) \rangle   \, ,
\label{eq:firstterm}
\end{align}
where the sum over $b^{\prime}$ denotes the sum over $\ket{\eps_{b^{\prime}}}$ sharing the same energy as $\ket{\eps_{b}}$.
The second term is:
\begin{align}
&\phantom{{}={}} \bra{\eps_b(t)} A_{i,\omega}^{\dagger}(t)A_{i,\omega}(t) \ket{\eps_b(t)} \ket{\eps_b(t)}  \nonumber\\
&= \left(\sum_{a^{\prime}} \delta_{\omega, \eps_b(t) - \eps_{a^{\prime}}(t)} \bra{\eps_b(t)} A_\alpha \ket{\eps_{a^{\prime}}(t)} \langle \eps_{a^{\prime}}(t)| \right) \left(\sum_{a} \delta_{\omega, \eps_b(t) - \eps_a(t)} \bra{\eps_a(t)} A_\alpha \ket{\eps_b(t)} 
| \eps_a(t) \rangle \right)\ket{\eps_b(t)} \nonumber\\
&= \left(\sum_{a} \delta_{\omega, \eps_b(t) - \eps_{a}(t)} \bra{\eps_b(t)} A_\alpha \ket{\eps_{a}(t)} \bra{\eps_a(t)} A_\alpha \ket{\eps_b(t)} \right)\ket{\eps_b(t)} \,.\nonumber\\
\label{eq:secondterm}
\end{align}

Subtracting Eq.~\eqref{eq:secondterm} from Eq.~\eqref{eq:firstterm} yields the drift term [Eq.~\eqref{eq:paraterm}], which is not zero, but a linear combination of degenerate eigenstates with the same energy $\eps_b(t)$. Before the jump happens the environment leads to the redistribution of $\ket{\eps_b(t)}$ to other states in the same energy manifold. (The Lamb shift $H_{\text{\text{LS}}}(t) = \sum_{i,\omega}S_{i}(\omega) A^\dagger_{i,\omega}(t) A_{i,\omega}(t) $ also yields the same effect.) Since they all share the same energy, this does not affect the overlap with the ground state. If the evolution by $H_{\text{S}}(t)$ is adiabatic, such a linear combination will stay in the same energy manifold and this explains the square-pulse like behavior in the overlapping with the ground state in Fig.~\ref{fig:8qubitssingle} of the main text.

\subsection{No degeneracy in $\eps_b(t)$}
If there are no degenerate states with energy $\eps_b(t)$, 
\begin{align}
&\phantom{{}={}} A_{i,\omega}^{\dagger}(t) A_{i,\omega}(t)\ket{\eps_b(t)}  = \sum_{a} \delta_{\omega, \eps_b(t) - \eps_a(t)}\bra{\eps_{b}(t)} A_\alpha \ket{\eps_{a}(t)}  \bra{\eps_a(t)} A_\alpha \ket{\eps_b(t)}
| \eps_{b}(t) \rangle 
\end{align}
This cancels with $\bra{\eps_b(t)} A_{i,\omega}^{\dagger}(t)A_{i,\omega}(t) \ket{\eps_b(t)} \ket{\eps_b(t)}$ [Eq.~\eqref{eq:secondterm}] and the drift term [Eq.~\eqref{eq:paraterm}] becomes zero.
\newline
%
%

\section{Derivation of Eq.~\eqref{eq:inctunnrate}}
\label{app:lindbladfermi}

When the state is $\ket{\psi_1(t)}$, its jump rate $\lambda_{1 \rightarrow 0}(t) $ to $\ket{\psi_0(t)}$ comprises the summation of Lindblad terms responsible for the $1 \rightarrow 0$ transition:
\begin{equation}
\lambda_{1 \rightarrow 0}(t) = \sum_{\alpha \in \{1\rightarrow 0\}}\braket{{A}_\alpha^{\dagger}(t){A}_{\alpha}(t)} \,.
\end{equation}
The summation is over the number of qubits $n$. Since each qubit is coupled to its own environment with an independent noise source, the $\gamma$ matrix in Eq.~\eqref{eq:unitarytransform} is already diagonal. From Eq.~\eqref{eq:Lindblad2}
we know that
\begin{equation}
L_{\alpha, \omega_{10}}(t) = \sum_{a,b} \delta_{\omega_{10}, \eps_b(t) - \eps_a(t)} \bra{\eps_a(t)} \sigma^{z}_{\alpha} \ket{\eps_b(t)} | \eps_a(t) \rangle  \langle \eps_b(t)|    \,.
\end{equation}

Assume that Bohr frequency $\omega_{10}(t)$ is due only to the $1\rightarrow 0$ transition (even if it is not, the other terms would be annihilated by the matrix element $\langle \psi_1(t) |\dots |\psi_1(t) \rangle$). The Lindblad operators ${A}_{\alpha}(t)$ have the form:
\begin{equation}
{A}_{\alpha}(t) = \sqrt{\gamma_{\alpha}(\omega_{10})}\langle\psi_0(t)|\sigma^{z}_{\alpha} |\psi_1(t)\rangle| \psi_0(t) \rangle  \langle \psi_1(t)|  \,.
\end{equation}
%
Therefore:
\begin{align}
\lambda_{1 \rightarrow 0}(t) &= \sum_{\alpha}  \langle \psi_1(t) | {A}^{\dagger}_{\alpha}(t)  {A}_{\alpha}(t)   |\psi_1(t) \rangle    \\
&=  \sum_{\alpha=1}^{n} \gamma_\alpha(\omega_{10})|\langle\psi_0(t)|\sigma^{z}_{\alpha} |\psi_1(t)\rangle|^2 \nonumber  \,.
\end{align}
Here $\gamma_\alpha(\omega_{10})$ is evaluated with respect to the Ohmic spectral density.
% \paragraph{}
% \Blindtext[2]


\chapter{1/f noise}
\label{cha:research_topic_2}
The trajectories method in the previous section can be applied to the non-markovian noise particularly of $1/f$ noise.

\section*{One qubit and one fluctuator}
\subsection*{Qubit}
The only qubit is subjected to time-independent magnetic field pointing in the $z$-direction. The initial state of the qubit is $(\ket{0}+\ket{1})/\sqrt{2}$, with initial Bloch vector pointing in the $x$-direction: $M(0) = (1, 0, 0)$.

The dynamics of the qubit is described by the precession equation (Schrodinger equation)
\begin{equation} \label{bv1}
\dot{\mathbf{M}} = \mathbf{B} \times \mathbf{M} \, .
\end{equation}

However, a stochastic magnetic field is $b(t)$ exists and is pointing parallel to $B$ such that the total magnetic field is $B+b(t)$.
\subsection*{Fluctuator}
The stochastic magnetic field is $b(t)$ originates from the fluctuator, which can find itself in one of two (meta)stable states, 1 and 2, and once a while makes a switch between them. We consider the symmetric RT process: $\gamma_{1\to 2}=\gamma_{2\to 1}=\gamma/2$. When the fluctuator is in state 1, the stochastic magnetic field is $b(t) = +b$; similarly when it is in state 2, the stochastic magnetic field is $b(t) = -b$. 

Define $m_{+}(t) = M_{x}(t) + iM_{y}(t)$, the decay of the ensemble average $\braket{m_{+}(t)}$ gives the $T2^{*}$. The differential equation of $\braket{m_{+}(t)}$ and its analytical solution is given in~\cite{1f}~(P.26) as:
\begin{equation} \label{FID01}
\braket{\ddot{m}_+} + \gamma \braket{\dot{m_+}} = -b^2  \braket{m_+} 
\end{equation}
with initial conditions $  \braket{ m_+ (0)}=1$, $\braket{\dot{m}_+(0)}=0$.  The solution of Eq.~(\ref{FID01}) with these 
initial conditions is
\begin{eqnarray} \label{FID02}
\braket{m_+}&=&(2\mu)^{-1}e^{-\gamma t/2}\left[(\mu +1)e^{\gamma \mu t/2}+ (\mu -1)e^{-\gamma \mu t/2}\right]\, , \nonumber \\
\mu &\equiv& \sqrt{1-(2b/\gamma)^2}\, .
\end{eqnarray}

\subsection*{Plots}
Define the ratio of the strength of fluctuator over the rate of fluctuator as $g =b/(\gamma/2) =  \frac{2b}{\gamma}$. By using Gillispie algorithm to determine the flipping times of fluctuator (thus the sign of the stochastic magnetic field), and averaging over many realizations, we plot the time evolution of ensemble average $\braket{m_{+}(t)}$ with $g = 0.8$ and $g = 5$. Although in each realization the initial state of the qubit is fixed, the initial state of the fluctuator is not. If the fluctuator starts at either state with equal probability, the initial condition $\braket{\dot{m}_+(0)}=0$ above is fuifilled.
\begin{figure}[htb!]
\centering
\includegraphics[width=1\textwidth]{1f/fig22repro.png}
\caption{Reproduction of FIG.~21 of~\cite{1f} (P.26). Blue lines: results reproduced from averaging 8000 realizations. The initial state of the fluctuator is either state 1 or 2 with equal probability. Green lines: analytical solutions.} Note that $b = 5$ for both curves.
\end{figure}


\paragraph{}
The stronger the fluctuator is or the slower the fluctuator switches, the resulting ensemble average $\braket{m_{+}}$ of the qubit decays faster. However, its decay rate saturates as the ratio $g$ reaches 1, where the behavior of $\braket{m_{+}(t)}$ enters from strictly decay to damped oscillation. To demonstrate FIG.~23 and Eq.~52 of~\cite{1f} numerically, $\braket{m_{+}(t)}$s with different $g$ are plotted in Fig.~\ref{fig:decayfactorlook}. Note that $\gamma$ is 1 switch/(time unit)~\cite{Bergli2009}. 
\begin{figure}[htb!]
\centering
\includegraphics[width=1\textwidth]{1f/decayfactorlook.png}
\caption{Saturation of decay as $b$ further increases. Note that $\gamma$ = 1 switch/(time unit) for all curves. The decay rate is saturated (cannot decay faster) after $g = 2b/\gamma$ reaches 1. Each curves are produced from averaging 10000 realizations with a random initial fluctuator state for each realization. }
\label{fig:decayfactorlook}
\end{figure}

\section*{One qubit and an ensemble of fluctuators}
\subsection*{Notations for ensemble of fluctuators to come up with an overall $1/\omega$ power spectrum: $S(\omega) = \mathcal A /\omega$.}
\subsubsection*{E Paladino, YM Galperin, G Falci, and BL Altshuler~\cite{1f}}
%In the simplest case, when the kinetics of fluctuations is characterized by a single relaxation rate,
% $\gamma$, the correlation function of a fluctuating quantity $x(t)$ is proportional to $e^{-\gamma |t|}$. 
% Then the spectral density is a Lorentzian function of frequency, 
%\begin{equation} \label{Lorentzian}
%S_x (\omega)  \propto \mathcal{L}_\gamma (\omega) \equiv \frac{1}{\pi} \frac{\gamma}{\omega^2 +\gamma^2}.
%\end{equation}
%In more general cases, the kinetics of $x(t)$ is a superposition of several, or even many, relaxation 
%processes with different rates. In general, a continuous distribution of the relaxation rates, 
%$\mathcal{P}_x(\gamma)$ may exist. Then the noise spectral density can be expressed as 
%\begin{equation} \label{total-spectrum}
%S_x (\omega)  \propto\int_0^\infty d\gamma \, \mathcal{P}_x(\gamma)  \mathcal{L}_\gamma (\omega) .
%\end{equation}

A single two-state fluctuator is described by a stochastic variable $\chi (t)= \pm 1$ with rates $\gamma_{1\to 2}=\gamma_{2\to 1}=\gamma/2$. The power spectrum of the noise generated by the $i$-th fluctuator is:
\begin{equation} \label{ns2}
S_i(\omega)=b_i^2 \cL_{\gamma_i} (\omega)\, ,
\end{equation}
where 
%Consider a classical stochastic variable $\chi (t)$, which at any time takes the values $\chi (t) = \pm 1$.  It is thus suitable for describing 
%a two-state fluctuator that can find itself in one of two (meta)stable states, 1 and 2, and once a while it 
%makes a switch between them.  
%rates $\gamma_{1\to 2}$ and $\gamma_{2\to 1}$, which can be different.  For simplicity, we will limit ourselves to 
%symmetric RT process: $\gamma_{1\to 2}=\gamma_{2\to 1}=\gamma/2$.   
$\cL_{\gamma_i} (\omega)$ is a Lorentzian function of frequency, 
\begin{equation} \label{Lorentzian}
\mathcal{L}_{\gamma_i} (\omega) \equiv \frac{1}{\pi} \frac{\gamma_i}{\omega^2 +\gamma_i^2}.
\end{equation}
The couplings $b_i$ are distributed with a  small dispersion around an average value $\overline b $.
Under these conditions the total power spectrum reads
\begin{equation} \label{ns_narrow_b}
S(\omega) = \overline{b^2} \int_{\gamma_m}^{\gamma_M} d\gamma \, \frac{P_0}{2 \gamma} \,  \cL_{\gamma} (\omega) 
\approx    \frac{{\mathcal A}}{\omega}\, ,
\end{equation}
where the amplitude  $\mathcal A$ can be expressed in terms of the number of \fs per noise
decade, $n_d= {\mathcal N}_T \ln{(10)}/\ln{(\gamma_M/\gamma_m)}$, as follows 
${\mathcal A} = \overline{b^2} P_0/4 = \overline{b^2}  n_d/(2 \ln(10))$.
%The spectrum exhibits a crossover to $\omega^{-2}$ behavior at $\omega \sim \gamma_M$. 

\subsection*{Distribution function of the fluctuators}
%P.416 Chap.22 of~\cite{Weiss2002}, log-uniform distribution of the level splitting.
%From under Eq.~(19) of~\cite{Bergli2009}, it turns out that distribution (18), which 
The ($1/\gamma$) distribution (Eq.~\eqref{eq:avnps1}) of the frequencies of the fluctuators corresponds to a uniform distribution of $\ln \, \gamma$.
Plot below shows there are $12$ decades of noise and the number of \fs per decade is $n_d = 100$. 
\begin{figure}[htb!]
\centering
\includegraphics[width=0.8\textwidth]{1f/frequencydist.pdf}
\caption{Distribution of frequencies of 1200 fluctuators.}
\end{figure}

\begin{figure}[htb!]
\centering
\includegraphics[width=0.7\textwidth]{1f/combinedfig2mxmp.pdf}
\caption{
\scriptsize Top: $\gamma_{\text{min}}=10^{-6}$, $\gamma_{\text{max}}=100$, $n_d=100$, $\langle b\rangle = 10^{-4}/4$;
Bottom: $\gamma_{\text{min}}=10^{-4}$, $\gamma_{\text{max}}=100$, $n_d=100$, $\langle b\rangle = 0.01/4$
Results are averages over $8k$ realizations.  Each BC is initially in a pure 
state randomly sampled according to 
$\langle \delta p_0 \rangle= \delta p_{eq}=0.08$. $\Delta b /\langle b \rangle \sim 0.2$.} %KY: 0.2 standard d seems not there in fig.2 at first. make any difference if no standard d?
\label{fig:decayfactorlook}
\end{figure}

\subsection*{Comparison with~\cite{torrontegui2016activated} and~\cite{baer1997quantum}}
\begin{align}
H_{S} &= -\left[\omega \sigma_{z} + \delta \sigma_{x}\right] /2 \\
H_{B} &= \sum_{k=1}^\infty \omega_k b_k^\dagger b_k + \sum_k \left(\epsilon_k b_k^\dagger b_k + T_k \sum_l [c^\dagger_{kl} b_k +\text{h.c.}] + \sum_l \varepsilon_{kl} c^\dagger_{kl} c_{kl} \right)\\
H_{SB} &= \sum_{i=1}^N  \sigma_i^z \otimes B^{\text{flu}}_i =  \sigma^z \otimes \sum_k \mu_{k} b_k^\dagger b_k
\end{align}
where $b_k (b^\dagger_k)$, $ c_{kl} (c_{kl}^\dagger)$ operators for fluctutator and fermionic band respectively. $T_k$ is the coupling to fermonic band. $\mu_{k}$ is the coupling strength of system qubit to fluctuator. $\gamma_{k}$ is the fluctuation rate, and $\mu_{k}/\gamma_{k}$ corresponds to $g_k$. 

System inherent adiabatic timescale is $\tau_{S}$. Fluctuator timescale is $\tau_{B} = \frac{1}{\gamma_{\text{slow}}}$. One important condition to have Lindblad form $\tau_{S} >> \tau_{B}$.


While for spin swap dephasing
\begin{align}
H_{S} &= -\left[\omega \sigma_{z} + \delta \sigma_{x}\right] /2 = A(t) H_{S}^{x} + B(t)H_{S}^{z} \\
H_{B} &= \sum_{k=1}^\infty \omega_k b_k^\dagger b_k \\
H_{SB} &= \sum_{i=1}^{N}\sigma_{i}^{z} \otimes \sum_{k}^{K} d_{k}(\hat{\sigma}_{k}^{\dagger} + \hat{\sigma}_{k}) 
\end{align}
Limitation: swapping the spins randomly at a rate faster than the recurrence time.


\section{Hamiltonian formulation}
\begin{equation}\label {qb1}
\hat{H}_{\text{sys}}=\frac{1}{2}\left(A(t) \,  \sigma_x + B(t) \, \sigma_z \right) \, .
\end{equation}

is cast into the spin-(time dependent) magnetic field description:

\begin{equation} \label{qb2}
\hat{H}_{\text{sys}}=(1/2)\mathbf{B}\cdot \sigma\, , \ B_z\equiv  B(t), \ B_x \equiv A(t)\, .
\end{equation}

The Schr{\"o}dinger equation turns out to be equivalent to the precession equation for the
Bloch vector:
\begin{equation} \label{bv1}
\dot{\mathbf{M}} = \mathbf{B} \times \mathbf{M} \, .
\end{equation}

\begin{figure}[h!]
\centerline{\includegraphics[width=4.5cm]{1f/paladino_fig01}}
\caption{Bloch vector representing the state of a qubit in the rotating 
(with angular frequency $B_0$) frame of reference.  
In the laboratory frame of reference it precesses around the $z$-axis
 with (time-dependent) angular velocity $B$. Fluctuations of 
 this velocity is $b(t)$ \label{figAGB1}}
\end{figure}

\section{Spin-fluctuator model}
A single two-state fluctuator is described by a stochastic variable $\chi (t)= \pm 1$ with rates $\gamma_{1\to 2}=\gamma_{2\to 1}=\gamma/2$. The power spectrum of the noise generated by the $i$-th fluctuator is:
\begin{equation} \label{ns2}
S_i(\omega)=b_i^2 \cL_{\gamma_i} (\omega)\, ,
\end{equation}
where 
%Consider a classical stochastic variable $\chi (t)$, which at any time takes the values $\chi (t) = \pm 1$.  It is thus suitable for describing 
%a two-state fluctuator that can find itself in one of two (meta)stable states, 1 and 2, and once a while it 
%makes a switch between them.  
%rates $\gamma_{1\to 2}$ and $\gamma_{2\to 1}$, which can be different.  For simplicity, we will limit ourselves to 
%symmetric RT process: $\gamma_{1\to 2}=\gamma_{2\to 1}=\gamma/2$.   
$\cL_{\gamma_i} (\omega)$ is a Lorentzian function of frequency, 
\begin{equation} \label{Lorentzian}
\mathcal{L}_{\gamma_i} (\omega) \equiv \frac{1}{\pi} \frac{\gamma_i}{\omega^2 +\gamma_i^2}.
\end{equation}

The couplings $b_i$ are distributed with a  small dispersion around an average value $\overline b $.
Under these conditions the total power spectrum reads
\begin{equation} \label{ns_narrow_b}
S(\omega) = \overline{b^2} \int_{\gamma_m}^{\gamma_M} d\gamma \, \frac{P_0}{2 \gamma} \,  \cL_{\gamma} (\omega) 
\approx    \frac{{\mathcal A}}{\omega}\, ,
\end{equation}
where the amplitude  $\mathcal A$ can be expressed in terms of the number of \fs per noise
decade, $n_d= {\mathcal N}_T \ln{(10)}/\ln{(\gamma_M/\gamma_m)}$, as follows 
${\mathcal A} = \overline{b^2} P_0/4 = \overline{b^2}  n_d/(2 \ln(10))$.

\subsection{Single fluctuator}
A single fluctuator induces an extra stochastic magnetic field $b_1(t)$ along the $B_z$.




Its effect can be included in the $\hat{H}_{\text{sys}}$, as:
\begin{equation}
\hat H_{\text{sys}} = \frac{1}{2}\left(A(t) \,  \sigma_x + B(t) \, \sigma_z \right)
+ \frac{1}{2} \,  b_1 \chi_1(t) \sigma_z \, .
\label{H_SF_general}
\end{equation}

where $\chi_1(t)$ switches with $\gamma_1/2$.




\subsection{Many fluctuators}
For many fluctuators,
\begin{equation}
\hat H_{\text{sys}} = \frac{1}{2}\left(A(t) \,  \sigma_x + B(t) \, \sigma_z \right)
+ \frac{1}{2} \,  \sum_{i}b_i \chi_i(t) \sigma_z \, .
\label{H_SF_general}
\end{equation}

where $\chi_i(t)$ switches with $\gamma_i/2$. 

The sum of fluctuator-$i$ is such that the $\chi_i(t)$ is distributed in $1/\gamma_i$.

\subsection{Case studies}
We study the decay of ensemble average $\braket{m_{+}(t)}$ of the qubit. Its decay rate saturates as the ratio $g$ reaches 1, where the behavior of $\braket{m_{+}(t)}$. Note that $\gamma$ is 1 switch/(time unit). 

\subsubsection{Single fluctuator: $A(t) = 0$ and $B(t) = 0$ for all $t$}
Consider the following Hamiltonian
\begin{equation}
\hat H_{\text{sys}} =  b_1 \chi_1(t) \sigma_z \,,
\label{H_SF_general1}
\end{equation}
is the case where there is no system driving. (where $\chi_1(t)$ switches with $\gamma_1/2$. )

The qubit's initial state is $\ket{+} = \frac{\ket{0}+\ket{1}}{\sqrt{2}}$. Denote $\ket{\psi(t)} = a\ket{0} + b\ket{1}$ the qubit state at time $t$, obtained by the stochastic Schr\"{o}dinger equation.

\begin{align}
M_{x}(t) &= ab^{*} + a^{*}b,\\
M_{y}(t) &= iab^{*} - ia^{*}b,.
\end{align}

After averaging many trajectories, we recover the density matrix evolution
\begin{equation}
\rho(t) = \frac {1}{2}{\begin{pmatrix}1+\braket{M_{z}(t)} & \braket{M_{x}(t)}-i\braket{M_{y}(t)}\\\braket{M_{x}(t)}+i\braket{M_{y}(t)} & 1-\braket{M_{z}(t)}\end{pmatrix}}  = \frac {1}{2}{\begin{pmatrix}1+\braket{M_{z}(t)} & \braket{M_{x}(t)}-i\braket{M_{y}(t)}\\\mathbf{\braket{M_{+}(t)}} & 1-\braket{M_{z}(t)}\end{pmatrix}}
\label{eq:fiddm}
\end{equation}

\begin{figure}[h!]
\centerline{\includegraphics[width=18.5cm]{1f/decayfactorlook_testing1126}}
\caption{$g = 2b/\gamma$. $10000$ trajectories.}
\end{figure}


\subsubsection{Multiple fluctuators with a time-dependent system Hamiltonian}
The simulation is illustrated with the following example.
\begin{equation}
\hat H_{\text{sys}} = -\frac{A}{2}\left(\left(1-\frac{t}{t_f}\right) \,  \sigma_x  + \frac{t}{t_f} \, \sigma_z \right)
+ \frac{1}{2} \,  \sum_{i = 1}^{10}b_i \chi_i(t) \sigma_z \, .
\label{H_SF_general}
\end{equation}
where: 
\\ $A = 1$ GHz;
\\The sum over fluctuator-$i$ with the fluctuator $\chi_i(t)$ distributed in $1/\gamma_i$ with  $\gamma_i \in [\gamma_{\text{min}}, \gamma_{\text{max}}]$; \\
$\gamma_{\text{min}} = 0.1$ GHz, $\gamma_{\text{max}} = 10$ GHz. \\
$\chi_i(t)$ switches with $\gamma_i/2$ and takes value of $\{-1, 1\}$;\\
There are 10 fluctuators; \\ 
The strengths of the fluctuators has mean $\langle b\rangle = 0.2$ GHz \footnote{Because in this illustration only $10$ fluctuators are included, their strengths are selected to be relatively large.} and standard deviation $\Delta b /\langle b \rangle = 0.2$.


For the ground state population (where the ground state is defined w.r.t the system Hamiltonian without the stochastic noise), its evolution with an annealing time $t_f = 1 \mu s$ is plotted in Fig.~\ref{fig:GS}.

\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/gspplot_reprod}}
\caption{Pure dephasing noise: $\gamma_{\text{min}}$=$0.1$ GHz, $\gamma_{\text{max}}=10$ GHz. 
Number of \fs is $10$. $\langle b\rangle = 0.2$ GHz,
$\Delta b /\langle b \rangle = 0.2$. Results are averaged over $1k$ trajectories.  The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$ (i.e. each fluctuator is $0.08$ more likely to be initialized in state $1$ than state $-1$).}
\label{fig:GS}
\end{figure}

For the coherence, because of the time-dependent system Hamiltonian, the off-diagonal part of the density matrix (in computational basis) now has a nonzero imaginary component. Therefore, the absolute value $|\braket{\sigma_{+}(t)}| = |\braket{M_{+}(t)}|$\footnote{Rigoriously,  from Eq.~\ref{eq:fiddm} the off diagonal element $|\braket{\sigma_{+}(t)}| = \frac{1}{2} |\braket{M_{+}(t)}|$, but here in the plot the $\frac{1}{2}$ is omitted due to different conventions in other papers.} is plotted. Its evolution with an annealing time $t_f = 1 \mu s$ is plotted in Fig.~\ref{fig:coherence}.



\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/offdiagonal_reprod}}
\caption{Pure dephasing noise: $\gamma_{\text{min}}=0.1$ GHz, $\gamma_{\text{max}}=10$ GHz. 
Number of \fs is $10$. $\langle b\rangle = 0.2$ GHz,
$\Delta b /\langle b \rangle = 0.2$. Results are averaged over $100$ trajectories.  The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$ (i.e. each fluctuator is $0.08$ more likely to be initialized in state $1$ than state $-1$).}
\label{fig:coherence}
\end{figure}



\section{Week of 12/8-1/20: Multiple fluctuators with a time-dependent system Hamiltonian: steady state, temperature, and $T_1$, $T_2$ decay simulation}
In the week of 12/8, I worked on the steady state and  temperature dependence of telegraph noise simulation on an annealing Hamiltonian; and I worked on $T_1$, $T_2$ decay simulation using the telegraph noise model.
\subsection{Relating initial distribution of fluctuators with temperature}
The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}$, which is defined by: 
\begin{equation}
\label{eq:fluctuatorequilibrium}
    \delta p_{eq} = 1 - (e^{-\epsilon/2 k_B T} )\simeq  \epsilon/2 k_B T \,.
\end{equation}
\subsection{Two temperature limits}
\label{sec:2Tl}
Here we study the steady state of the system evolved with the following annealing Hamiltonian (initial state is also its ground state):
\begin{equation}
\hat H_{\text{sys}} = -\frac{A}{2}\left(\left(1-\frac{t}{t_f}\right) \,  \sigma_x  + \frac{t}{t_f} \, \sigma_z \right)
+ \frac{1}{2} \,  \sum_{i}b_i \chi_i(t) \sigma_z \, .
\label{H_SF_general2}
\end{equation}
where: 
\\ $A = 1$ GHz;
\\The sum over fluctuator-$i$ with the fluctuator $\chi_i(t)$ distributed in $1/\gamma_i$ with  $\gamma_i \in [\gamma_{\text{min}}, \gamma_{\text{max}}]$; \\
$\gamma_{\text{min}} = 0.01$ GHz, $\gamma_{\text{max}} = 1$ GHz. \\
$\chi_i(t)$ switches with $\gamma_i/2$ and takes value of $\{-1, 1\}$;\\
The strengths of the fluctuators has mean $\langle b\rangle = 0.2$ GHz and standard deviation $\Delta b /\langle b \rangle = 0.2$.



\subsubsection{Infinite temperature $T \rightarrow \infty$} 
Take $T \rightarrow \infty$, the thermal equilibrium distribution of $\delta p_{eq} \rightarrow 0$. In this case, the initial distribution of fluctuators has equal probability of being in spin up or spin down, i.e. $P(\chi_i(0) = 1) = P(\chi_i(0) = -1) = \frac{1}{2}$.
Fig.~\ref{fig:highTlimit} shows that the steady state is a maximally mixed state, with (instantaneous) ground state approaching $1/2$, and off-diagonal elements in computational basis decaying to $0$.

\begin{figure}[h!]
\includegraphics[width=8.0cm]{1f/gspplot_highT.pdf}
\includegraphics[width=8.0cm]{1f/offdiagplot_highT.pdf}
\caption{High temperature limit, pure dephasing noise: $\gamma_{\text{min}}=0.01$ GHz, $\gamma_{\text{max}}=1$ GHz. 
Number of \fs is $20$. $\langle b\rangle = 0.2$ GHz,
$\Delta b /\langle b \rangle = 0.2$. Results are averaged over $1k$ trajectories.  The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0$ (i.e. each fluctuator is equally likely to be initialized in state $1$ than state $-1$).}
\label{fig:highTlimit}
\end{figure}


\subsubsection{Zero temperature $T \rightarrow 0$} 
Take $T \rightarrow 0$, the thermal equilibrium distribution of $\delta p_{eq} \rightarrow 1$. In this case, the initial distribution of fluctuators are all collectively spin up, i.e. $P(\chi_i(0) = 1) = 1$. 
Fig.~\ref{fig:zeroTlimit} shows that the steady state is also a maximally mixed state, with (instantaneous) ground state approaching $1/2$, and off-diagonal elements in computational basis decaying decaying to $0$.
Assuming the strengths and frequencies of the fluctuators do not depend on temperature, with temperature $T \rightarrow 0$, we can see that the fluctuators destroy the coherence faster and cause larger oscillations to the (instantaneous) GS population at early anneal. 



\begin{figure}[h!]
\includegraphics[width=8.0cm]{1f/gspplot_zeroT.pdf}
\includegraphics[width=8.0cm]{1f/offdiagplot_zeroT.pdf}
\caption{Zero temperature limit, pure dephasing noise: $\gamma_{\text{min}}=0.01$ GHz, $\gamma_{\text{max}}=1$ GHz. 
Number of \fs is $20$. $\langle b\rangle = 0.2$ GHz,
$\Delta b /\langle b \rangle = 0.2$. Results are averaged over $1k$ trajectories.  The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 1$.}
\label{fig:zeroTlimit}
\end{figure}

\subsection{$T_{1}$ and $T_{2}$ time}
\subsubsection{$T_1$ time}
To measure $T_1$ time, we initialize the state in the $\ket{1}$ state and evolve it with the following Stochastic Hamiltonian with fluctuator in the longitudinal direction:
\begin{equation}
    H(t) = \frac{E}{2}\sigma_z + \frac{1}{2} \,  \sum_{i}b_i \chi_i(t) \sigma_x \,,
\end{equation}
where $\chi_i(t)$ switches with $\gamma_i/2$. The sum of fluctuator-$i$ is such that the $\chi_i(t)$ is distributed in $1/\gamma_i$. At large time $t \gg T_1$, the resulting density matrix under this initial condition and Hamiltonian can be expressed as:
% \begin{equation}
% \rho(t)  = {\begin{pmatrix}(\rho_{00}(0)-1)e^{-\frac{t}{T_1}} + 1 & \rho_{10}(0)e^{-i\omega t} e^{-\frac{t}{T_2}}\\
% \rho_{01}(0)e^{i\omega t} e^{-\frac{t}{T_2}} & (1-\rho_{00}(0))e^{-\frac{t}{T_1}}\end{pmatrix}}
% \label{eq:fiddm}
% \end{equation}
\begin{equation}
\rho(t)  = {\begin{pmatrix}-\frac{1}{2}e^{-\frac{t}{T_1}} + \frac{1}{2} & 0\\
0 & \frac{1}{2}e^{-\frac{t}{T_1}} + \frac{1}{2}\end{pmatrix}}
\label{eq:fiddm}
\end{equation}

The $T_1$ time can then be found by finding the decay profile of the diagonal elements of Eq.~\ref{eq:fiddm}. For the example of qubit having energy of $E/2 = 1$ GHz and fluctuator strength being $\langle b\rangle = 0.046$ GHz, the $T_1$ time and decay profile is plotted in Fig.~\ref{fig:T1}.


\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/espplot_new.pdf}}
\caption{Longitudinal noise: $\gamma_{\text{min}}=0.01$ GHz, $\gamma_{\text{max}}=1$ GHz. 
Number of \fs is $\mathbf{200}$. $\langle b\rangle = 0.046$ GHz,
$\Delta b /\langle b \rangle = 0.2$. Results are averaged over $1k$ trajectories.  The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$ (i.e. each fluctuator is $0.08$ more likely to be initialized in state $1$ than state $-1$).}
\label{fig:T1}
\end{figure}



\subsubsection{$T_2$ time}
To measure $T_2$ time (without presence of Longitudinal noise), we initialize the state in the $\ket{+}$ state and evolve it with the following Stochastic Hamiltonian with fluctuator in the transverse direction:
\begin{equation}
    H(t) = \frac{E}{2}\sigma_z + \frac{1}{2} \,  \sum_{i}b_i \chi_i(t) \sigma_z \,,
\end{equation}
where $\chi_i(t)$ switches with $\gamma_i/2$. The resulting density matrix under this initial condition and Hamiltonian can be expressed as:
% \begin{equation}
% \rho(t)  = {\begin{pmatrix}-\frac{1}{2}e^{-\frac{t}{T_1}} + 1 & \frac{1}{2}e^{-i\omega t} e^{-\frac{t}{T_2}}\\
% \frac{1}{2}e^{i\omega t} e^{-\frac{t}{T_2}} & \frac{1}{2}e^{-\frac{t}{T_1}}\end{pmatrix}}
% \label{eq:fiddm2}
% \end{equation}

\begin{equation}
\rho(t)  = {\begin{pmatrix}\frac{1}{2} & \frac{1}{2}e^{-i\omega t} e^{-\frac{t}{T_2}}\\
\frac{1}{2}e^{i\omega t} e^{-\frac{t}{T_2}} & \frac{1}{2}\end{pmatrix}}
\, \text{       with       }
\rho(0)  = \begin{pmatrix}\frac{1}{2}\,\,\, & \frac{1}{2}\\
\frac{1}{2}\,\,\, & \frac{1}{2}\end{pmatrix} \,.
\label{eq:fiddm2}
\end{equation}



The $T_2$ time can then be found by finding the decay profile of expectation value of the $\ket{+}$ state. Its time evolution according to Eq.~\ref{eq:fiddm2} is:
\begin{equation}
    \left<+|\rho(t)|+\right> = \frac{1}{2} + \frac{1}{2}e^{-\frac{t}{T_2}} \cos{\omega t} \,.
\end{equation}

As $\left<+|\rho(t)|+\right> = \frac{1}{2}$, the off-diagonal elements of the density matrix vanish. For the example of qubit having energy of $E/2 = 1$ GHz and fluctuator strength being $\langle b\rangle = 0.046$ GHz, the expectation value and decay profile is plotted in Fig.~\ref{fig:T2}.


\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/t2plot_new.pdf}}
\caption{Transverse noise: $\gamma_{\text{min}}=0.01$ GHz, $\gamma_{\text{max}}=1$ GHz. 
Number of \fs is $\mathbf{100}$. $\langle b\rangle = 0.046$ GHz,
$\Delta b /\langle b \rangle = 0.2$. Results are averaged over $1k$ trajectories.  The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$ (i.e. each fluctuator is $0.08$ more likely to be initialized in state $1$ than state $-1$). Here we donote the decay profile as $e^{-t/T_2^{*}}$ since there is no longitudinal noise (i.e. $T_1 = \infty$).}
\label{fig:T2}
\end{figure}

\section{Circuit Hamiltonian}
% The exact form of $H_{S}(s)$ depends on many parameters. To see its dependence on $\phi_x(s)$ and $\phi_z(s)$, 
% \begin{align}
%     H_{S}(s) &\propto \cos(\phi_x(s)/ 2) \,,\notag\\
%     H_{S}(s) &\propto \sqrt{1 + \tan(\phi_x(s)/2)^2)} \,,\notag\\
%     H_{S}(s) &\propto e^{i\phi_z(s)}\,,\notag\\
%     H_{S}(s) &\propto e^{-i\phi_z(s)}\,.
% \end{align}

The CFSQ circuit Hamiltonian $H_{S}(s)$ takes the form of:
\begin{equation*}
H_S(s)= \frac{E_C}{2}{\hat{n}}^2-2E_J\cos{(\hat{\varphi})+2\alpha E_J\sqrt{1+d^2\tan^2{\left(\frac{\varphi_x(s)}{2}\right)}}\cos{\left(\frac{\varphi_x(s)}{2}\right)}}\cos\left(2\hat{\varphi}+\varphi_z(s)-\varphi_0(s)\right) \,,
\end{equation*}
which can be rewritten as:
\begin{eqnarray*}
\label{Eq:CH}
    H_{S}(s) &=& E_{J}\left(\frac{E_C}{2E_J} \hat{n}^2 - (\hat{d}_{1} + \hat{d}_{1}^{\dagger}) + \right. \notag \\
&& \hspace{-0.5cm} \left. \qquad\qquad \alpha
    \cos{\left(\frac{\phi_x(s)}{2}\right)}\sqrt{1 + d^2 \tan^2{\frac{\phi_x(s)}{2}}}\left(e^{i(\phi_z(s)-\phi_0(s))}\hat{d}_2 + e^{-i(\phi_z(s)-\phi_0(s))}\hat{d}_2^{\dagger}\right) \right)\,,
\end{eqnarray*}
where: \\$E_J$ is the Josephson junction energy; \\
$E_C$ is the mean Capacitive energy $= 2\alpha (E_{J1} + E_{J2})$; \\ $\hat{n}$ is the charge operator (with the same dimension as $H_{S}$); \\ $\hat{d}_{1}$ is the charge displacement operator by 1 cooper pair (with the same dimension as $H_{S}$); \\
$\alpha < 1$ is ratio of the current in one of the small $x$-loop junctions to the current in the large $z$-loop junction. \\
$d = \frac{E_{J1} - E_{J2}}{E_{J1} + E_{J2}}$ is the $x$-loop junction asymmetry; \\ $\phi_x(s)$ is the time-dependent $x$ (barrier) bias phase; \\
$\phi_z(s)$ is the time-dependent $z$ (tilt) bias phase; \\
$\phi_0 = \tan^{-1}{\left(d\tan{\left(\frac{\phi_x(s)}{2}\right)}\right)}$; \\
$\hat{d}_{2}$ is the charge displacement operator by 2 cooper pairs (with the same dimension as $H_{S}$).

As suggested by Huo, the total Stochastic Hamiltonian $H(s)$ can be formulated as fluctuation in persistent current operator:
\begin{equation}
\label{eq:stocH}
    H(s) =  H_{S}(\phi_x(s), \phi_z(s)) + \frac{1}{2} \,  \sum_{i}b_i \chi_i(s) I_p(s) \,,
\end{equation}

where $H_S(s)$ is the time-dependent, adiabatic circuit Hamiltonian for the $s$-curve problem; $I_p(s) = I_p((\phi_x(s), \phi_z(s)))$ is the persistent current operator.

\begin{center}
\begin{tabular}{ |c|c|c| } 
 \hline
 & Qubit & CFSQ  \\ 
 \hline
 fluctuation & $\sigma_z$ &$I_{p}(s)$   \\ 
 \hline
\end{tabular}
\end{center}

\subsection{Case studies}
I studied the time evolution under the circuit Hamiltonian, with the following parameters (4 decimal figures) and flux schedules:
\begin{figure}[h!]
  \begin{minipage}{.5\textwidth}
\begin{align}
    E_J &= 592.9434/2\pi \text{ GHz} \,,\notag\\
    E_c &= 5.4092 \text{GHz} \,,\notag\\
    \alpha &= 0.46 \,,\notag\\
    d &= 0.1 \,,\notag\\
    \phi_x(s) &= 0.96s+1.04\pi \,,\notag\\
    \phi_z(s) &= (0.326s + \phi_z(0))\pi \,.
\end{align}
  \end{minipage}%
  \begin{minipage}{.5\textwidth}
  \vspace{2cm}
    \centering
    \includegraphics[width=8cm]{1f/scurvezgridspectrum_z-121}
    \caption{Spectrum with  $\phi_z(0)/\pi = -1.21$.}
    \label{fig:spectrum}
  \end{minipage}
\end{figure}

The initial tilt bias $\phi_z(0)$ is an external parameter the value of which we can set. Here I focus on $\phi_z(0)/\pi = -1.21$ (the spectrum of the first $5$ levels is plotted in Fig.~\ref{fig:spectrum}. I look into the cases of close-system evolution, open-system evolution from adiabatic master equation, and open-system evolution from the fluctuator 1/f simulation. For close system evolution and adiabatic master equation, I truncate the energy levels of the system to $10$, and plot the populations of the first $5$ levels. For fluctuator 1/f simulation, I do not perform any truncation and simulate the populations of all the $121$ levels , defined by the CFSQ circuit Hamiltonian.

\subsection{Close system annealing evolution}
I ran the close system annealing evolution for $t_f = 6$ ns with value of $\phi_z(0)/\pi = -1.21$, and plotted the results in Fig.~\ref{fig:closed}.
\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/scurvezgridmefidelity_z-121_closed_6ns}}
\caption{The eigenstate populations for  $\phi_z(0)/\pi = -1.21$. Closed-system evolution.}
\label{fig:closed}
\end{figure}

\subsection{Adiabatic master equation simulation}
I ran the adiabatic master equation simulations for $t_f = 6$ ns with value of $\phi_z(0)/\pi = -1.21$. Set the temperature to be 20mK, $g^2$ to be $1e^{-4}$ and $\omega_c$ cutoff frequency to be $4$GHz (I will try higher cutoff frequency later). Since the Lindblad operator is defined based on energy difference, I also additionally set the absolute tolerance of energy difference ($\omega$) to be $\frac{0.1}{2\pi}$Hz for the grouping of Lindblad operator. For example, if $|\omega_{ab} - \omega_{cd}| < \frac{0.1}{2\pi}$Hz, then $L_{ab}$ and $L_{cd}$ are combined into one Lindblad operator $L(\omega)$. The results are plotted in Fig.~\ref{fig:ame}.
\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/scurvezgridmefidelity_z-121_ame_6ns}}
\caption{The eigenstate populations for (a) $\phi_z(0)/\pi = -1.21$. Evolution under adiabatic master equation.}
\label{fig:ame}
\end{figure}

\subsection{1/f noise simulation}
I ran the 1/f noise simulation with the stochastic Hamiltonian Eq.~\ref{eq:stocH}. I use $10$ fluctuators in the form of $I_{p}(s)$. The flipping frquency is sampled from $1/\gamma$ distribution with $\gamma \in \left[\gamma_{\text{min}}, \gamma_{\text{max}}\right]$, $\langle b\rangle = 0.46$ GHz and
$\Delta b /\langle b \rangle = 0.2$. $\phi_z(0)/\pi = -1.21$.
\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/scurvezgridqtfidelity_z-121_1f}}
\caption{The eigenstate populations for (a) $\phi_z(0)/\pi = -1.21$. $\gamma_{\text{min}}=0.01$ GHz, $\gamma_{\text{max}}=1$ GHz. 
Number of \fs is $\mathbf{10}$. $\langle b\rangle = 0.46$ GHz,
$\Delta b /\langle b \rangle = 0.2$. Results are averaged over $10$ trajectories.  The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$. Black line shows the sum of the populations of the first $5$ energy levels. It shows that some of the populations are lost to higher excited states. }
\label{fig:1f}
\end{figure}

\section{Temperature dependence of 1/f noise}
We want to understand how the temperature $T$ affects the coupling strength $b$, switching rate $\gamma$, number of fluctuators, and the steady state behavior of the system qubit evolution.


In~\cite{shnirman20071} (1/f noise and two-level systems in Josephson qubits), it is stated that:
\begin{itemize}
    \item Coupling strength $b$ does not depend much on temperature $T$.
    \item Switching rate cutoff has to be smaller than $T$, $\gamma_{\text{max}} \ll T$.
    \item Each fluctuator has its own energy $E_i$, only those with $E_i \ll T$ are involved.
    \item For the spectra $S(\omega)$, extrapolations of the low-frequency $1/ f$ and high-frequency Ohmic spectra cross at $\omega \sim T$. 
\end{itemize}

In~\cite{burnett2014evidence} (Evidence for interacting two-level systems from the 1/f noise of a superconducting resonator), it is stated that:
\begin{itemize}
    \item The number of activated TLSs (fluctuators) is proportional to temperature. The effect of each fluctuator is small as $T/b_i$.
    \item The noise of superconducting
qubit (at a fixed frequency, e.g. $0.1\text{Hz}$) increases as the temperature is decreased. $S(0.1\text{Hz}) \propto 1/T^{1.22}$. Moreover, $1/f$ dependence is observed only at the low temperature, but not high temperature.
    \item This is because of the fact that as the dephasing rate of the fluctuator ($\gamma \propto T^{1.22}$) decreases with temperature the energy drift becomes more visible. As a result, with decreasing temperature the noise sensitivity increases, even if the number of thermally excited fluctuators decreases. 
\end{itemize}

\subsection{2/8: Multiple toy examples of studying the steady state: (A) Annealing.}
I continue the examples in Sec.~\ref{sec:2Tl}, but with different effects from fluctuators.

% One can produce a nontrivial steady state if the environment does not just have fluctuators in a single orientation (e.g. $\sigma_z$ or $\sigma_x$), but have fluctuators of both orientations. 

I include fluctuators of both longitudinal and transverse orientations ($\sigma_z$ and $\sigma_x$) in the environment. This leads to the tilting of the noise axis in the bloch sphere.

\subsubsection{(Example.A1)}
Consider the following configuration. A driven qubit, coupled to $20$ fluctuators pointing to both longitudinal direction and transverse direction.

% \sout{\scriptsize $\hat H_{\text{sys}} = -\frac{A}{2}\left(\left(1-\frac{t}{t_f}\right) \,  \sigma_x  + \frac{t}{t_f} \, \sigma_z \right)
% + \frac{1}{2} \,  \sum_{i = 1}^{10}b_i \chi_i(t) \sigma_z - 0.2b_i \chi_i(t) \sigma_x $}

\begin{equation}
\hat H_{\text{sys}} = -\frac{A(t/t_f)}{2}\sigma_x  + \frac{B(t/t_f)}{2}\sigma_z 
+ \frac{1}{2} \,  \sum_{i = 1}^{20}b_i \chi_i(t) (\sigma_z - 0.2 \sigma_x)\, .
\label{H_SF_general}
\end{equation}
where: 
%\\ $A = 1$ GHz;
\\ $A$ and $B$ are the DWave 2000 schedules. Magnitude around $6$ Hz;
\\The sum over fluctuator-$i$ with the fluctuator $\chi_i(t)$ distributed in $1/\gamma_i$ with  $\gamma_i \in [\gamma_{\text{min}}, \gamma_{\text{max}}]$; \\
$\gamma_{\text{min}} = 0.1$ GHz, $\gamma_{\text{max}} = 10$ GHz. \\
$\chi_i(t)$ switches with $\gamma_i/2$ and takes value of $\{-1, 1\}$;\\
There are $20$ fluctuators; \\ 
The strengths of the fluctuators has mean $\langle b\rangle = 0.2$ GHz and standard deviation $\Delta b /\langle b \rangle = 0.2$. Strong compared to the system Hamiltonian; \\
A mixture of longitudinal and transverse noise; \\
The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$ (i.e. each fluctuator is $0.08$ more likely to be initialized in state $1$ than state $-1$).


% \begin{figure}[h!]
% %\vspace{50pt}
% \hspace{-1cm}
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=3.1in]{1f/gsplot_ss_new.png}
% \caption{}
% \label{fig:sub1}
% \end{subfigure}
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=3.1in]{1f/gspplot_tdss100ns}
% \caption{}
% \label{fig:sub2}
% \end{subfigure}\\
% \hspace{-1cm}
% \begin{subfigure}[b]{0.49\textwidth}

% \includegraphics[width=3.1in]{1f/gspplot_ss_300ns}
% \caption{}
% \label{fig:sub3}
% \end{subfigure}
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=3.1in]{1f/gspplot_ss_500ns}
% \caption{}
% \label{fig:sub4}
% \end{subfigure}
% \label{fig: spectrums}
% \end{figure}



\begin{figure}[h!]
\includegraphics[width=3.1in]{1f/gsplot_ss_new.png}
\includegraphics[width=3.1in]{1f/gspplot_tdss100ns}
\includegraphics[width=3.1in]{1f/gspplot_ss_300ns}
\includegraphics[width=3.1in]{1f/gspplot_ss_500ns}
\caption{}
\end{figure}

\subsubsection{(Example.A2)}
Consider the following configuration. A driven qubit, coupled to $20$ fluctuators pointing to both longitudinal direction and transverse direction.

\begin{equation}
\hat H_{\text{sys}} = -\frac{A(t/t_f)}{2}\sigma_x  - \frac{B(t/t_f)}{2}\sigma_z 
+ \frac{1}{2} \,  \sum_{i = 1}^{20}b_i \chi_i(t) (\sigma_z - 0.4 \sigma_x)\, .
\label{H_SF_general}
\end{equation}
where: 
%\\ $A = 1$ GHz;
\\ $A$ and $B$ are the DWave 2000 schedules. Magnitude around $6$ Hz;
\\The sum over fluctuator-$i$ with the fluctuator $\chi_i(t)$ distributed in $1/\gamma_i$ with  $\gamma_i \in [\gamma_{\text{min}}, \gamma_{\text{max}}]$; \\
$\gamma_{\text{min}} = 0.1$ GHz, $\gamma_{\text{max}} = 10$ GHz. \\
$\chi_i(t)$ switches with $\gamma_i/2$ and takes value of $\{-1, 1\}$;\\
There are $20$ fluctuators; \\ 
The strengths of the fluctuators has mean $\langle b\rangle = 2\pi\,0.2$ GHz and standard deviation $\Delta b /\langle b \rangle = 0.2$. Strong compared to the system Hamiltonian; \\
A mixture of longitudinal and transverse noise; \\
The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$ (i.e. each fluctuator is $0.08$ more likely to be initialized in state $1$ than state $-1$).

\begin{figure}[h!]
\centerline{\includegraphics[width=10.5cm]{1f/gspplot_ss_A2}}
\caption{}
\label{fig:exampleA2}
\end{figure}


\subsubsection{(Example.A3)}
Consider the following configuration. A driven qubit, coupled to $20$ fluctuators pointing to both longitudinal direction and transverse direction.

\begin{equation}
\hat H_{\text{sys}} = -\frac{A(t/t_f)}{2}\sigma_x  - \frac{B(t/t_f)}{2}\sigma_z 
+ \frac{1}{2} \,  \sum_{i = 1}^{20}b_i \chi_i(t) (\sigma_z - 0.2 \sigma_x)\, .
\label{H_SF_general}
\end{equation}
where: 
%\\ $A = 1$ GHz;
\\ $A$ and $B$ are the DWave 2000 schedules. Magnitude around $6$ MHz;
\\The sum over fluctuator-$i$ with the fluctuator $\chi_i(t)$ distributed in $1/\gamma_i$ with  $\gamma_i \in [\gamma_{\text{min}}, \gamma_{\text{max}}]$; \\
$\gamma_{\text{min}} = 0.1$ GHz, $\gamma_{\text{max}} = 10$ GHz. \\
$\chi_i(t)$ switches with $\gamma_i/2$ and takes value of $\{-1, 1\}$;\\
There are $20$ fluctuators; \\ 
The strengths of the fluctuators has mean $\langle b\rangle = 2\pi\,0.2$ GHz and standard deviation $\Delta b /\langle b \rangle = 0.2$. Strong compared to the system Hamiltonian; \\
A mixture of longitudinal and transverse noise; \\
The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$ (i.e. each fluctuator is $0.08$ more likely to be initialized in state $1$ than state $-1$).


% \begin{figure}[h!]
% \centerline{\includegraphics[width=10.5cm]{gspplot_ss_A4}}
% \caption{}
% \label{fig:exampleA2}
% \end{figure}
\begin{figure}[h!]
\centerline{\includegraphics[width=10.5cm]{1f/gspplot_ss_A5}}
\caption{}
\label{fig:exampleA2}
\end{figure}

The paper~\cite{vestgaarden2008nonlinearly} studies how the Landau-Zener like dynamics of a qubit and the end state are influenced by the coupling strength and switching rate of the fluctuators.

\subsection{ Time-independent system Hamiltonian: Different fluctuator orientations.}
\begin{equation}
    H(t) = \frac{E}{2}\sigma_z + \frac{1}{2} \,  \sum_{i}b_i \chi_i(t) [\sigma_x - \sigma_z]\,,
\end{equation}

where: 
\\ $A = 1$ GHz;
\\The sum over fluctuator-$i$ with the fluctuator $\chi_i(t)$ distributed in $1/\gamma_i$ with  $\gamma_i \in [\gamma_{\text{min}}, \gamma_{\text{max}}]$; \\
$\gamma_{\text{min}} = 0.01$ GHz, $\gamma_{\text{max}} = 1$ GHz. \\
$\chi_i(t)$ switches with $\gamma_i/2$ and takes value of $\{-1, 1\}$;\\
The strengths of the fluctuators has mean $\langle b\rangle = 0.2$ GHz and standard deviation $\Delta b /\langle b \rangle = 0.2$.

\begin{figure}[h!]
\centerline{\includegraphics[width=10.5cm]{1f/gspplot_ss1.pdf}}
\caption{Longitudinal noise: $\gamma_{\text{min}}=0.01$ GHz, $\gamma_{\text{max}}=1$ GHz. 
Number of \fs is $20$. $\langle b\rangle = 0.2$ GHz,
$\Delta b /\langle b \rangle = 0.2$. Results are averaged over $3k$ trajectories.  The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$ (i.e. each fluctuator is $0.08$ more likely to be initialized in state $1$ than state $-1$).}
\label{fig:gspplot_ss1}
\end{figure}

\newpage
\begin{equation}
    H(t) = \frac{E}{2}\sigma_z + \frac{1}{2} \,  \sum_{i}b_i \chi_i(t) [\sigma_x]\,,
\end{equation}

where: 
\\ $A = 1$ GHz;
\\The sum over fluctuator-$i$ with the fluctuator $\chi_i(t)$ distributed in $1/\gamma_i$ with  $\gamma_i \in [\gamma_{\text{min}}, \gamma_{\text{max}}]$; \\
$\gamma_{\text{min}} = 0.01$ GHz, $\gamma_{\text{max}} = 1$ GHz. \\
$\chi_i(t)$ switches with $\gamma_i/2$ and takes value of $\{-1, 1\}$;\\
The strengths of the fluctuators has mean $\langle b\rangle = 0.2$ GHz and standard deviation $\Delta b /\langle b \rangle = 0.2$.

\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/gspplot_ss2.pdf}}
\caption{Longitudinal noise: $\gamma_{\text{min}}=0.01$ GHz, $\gamma_{\text{max}}=1$ GHz. 
Number of \fs is $20$. $\langle b\rangle = 0.2$ GHz,
$\Delta b /\langle b \rangle = 0.2$. Results are averaged over $3k$ trajectories.  The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$ (i.e. each fluctuator is $0.08$ more likely to be initialized in state $1$ than state $-1$).}
\label{fig:gspplot_ss2}
\end{figure}

\begin{equation}
    H(t) = \frac{E}{2}\sigma_z + \frac{1}{2} \,  \sum_{i}b_i \chi_i(t) [\sigma_x + \sigma_z]\,,
\end{equation}

where: 
\\ $A = 1$ GHz;
\\The sum over fluctuator-$i$ with the fluctuator $\chi_i(t)$ distributed in $1/\gamma_i$ with  $\gamma_i \in [\gamma_{\text{min}}, \gamma_{\text{max}}]$; \\
$\gamma_{\text{min}} = 0.01$ GHz, $\gamma_{\text{max}} = 1$ GHz. \\
$\chi_i(t)$ switches with $\gamma_i/2$ and takes value of $\{-1, 1\}$;\\
The strengths of the fluctuators has mean $\langle b\rangle = 0.2$ GHz and standard deviation $\Delta b /\langle b \rangle = 0.2$.

\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/gspplot_ss3.pdf}}
\caption{Longitudinal noise: $\gamma_{\text{min}}=0.01$ GHz, $\gamma_{\text{max}}=1$ GHz. 
Number of \fs is $20$. $\langle b\rangle = 0.2$ GHz,
$\Delta b /\langle b \rangle = 0.2$. Results are averaged over $3k$ trajectories.  The initial value of each fluctuator is randomly sampled according to thermal equilibrium distribution $\delta p_{eq}= 0.08$ (i.e. each fluctuator is $0.08$ more likely to be initialized in state $1$ than state $-1$).}
\label{fig:gspplot_ss3}
\end{figure}

\subsection{ Time-independent system Hamiltonian: Different fluctuator strengths.}
\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/compare_b.pdf}}
\caption{Same settings as before but green line has $\langle b\rangle = 2$ GHz.}
\label{fig:gspplot_ssb}
\end{figure}

A higher coupling strength to the fluctuators speeds up the evolution to maximally mixed state.

\subsection{Time-independent system Hamiltonian: Different rates in switching up and down}
\begin{figure}[h!]
\centerline{\includegraphics[width=12.5cm]{1f/compare_v.pdf}}
\caption{Same settings as before but flipping up is more likely than flipping down. Blue: Symmetric. Green: Non-symmetric.}
\label{fig:gspplot_ssv}
\end{figure}

% Having non-symmetric rates slightly increases the time to reach equilibrium.
Having non-symmetric rates only slightly increases the time to reach the steady state of maximally mixed state. 


\chapter{Quantum feedback control}
\label{cha:research_topic_4}
\paragraph{}
Quantum feedback or quantum feedback control is a class of methods to prepare and manipulate a quantum system in which that system's quantum state or trajectory is used to evolve the system towards some desired outcome. Just as in the classical case, feedback occurs when outputs from the system are used as inputs that control the dynamics (e.g. by controlling the Hamiltonian of the system). The feedback signal is typically filtered or processed in a classical way, which is often described as measurement based feedback. However, quantum feedback also allows the possibility of maintaining the quantum coherence of the output as the signal is processed (via unitary evolution), which has no classical analogue.

\section{}
Adiabatic quantum computing (AQC)~\cite{albash2018adiabatic} is a quantum approach to solve combinatorial optimization problems. It is related to several variants such as quantum annealing (analog/continuous), trotterized digital annealing~\cite{barends2016digitized}, and a hybrid approach called the quantum approximate optimization algorithm (QAOA)~\cite{farhi2014quantum} that is realized in gate-model quantum computing. 

In AQC, the solution of the computational problem is encoded as the ground state of the final Hamiltonian. In an ideal situation, a quantum state is initiated as the ground state of an initial Hamiltonian, and is evolved to the ground state of the final Hamiltonian. A projective measurement is then performed on the quantum state to read out the solution. However, due to quantum errors, this is not always successful, i.e. at the end of the process the quantum state is not the ground of final Hamiltonian. 

Quantum error correction (QEC) aims to correct such quantum errors. There were previous extensive studies on quantum error correction in AQC~\cite{young2013error, lidar2008towards, mishra2016performance}, mostly centered on passive error correction techniques such as error correcting codes. This proposal is about a particular active quantum error correction approach: feedback-based error correction, for AQC.


\section{Outline of topics}
The following topics about feedback-based error correction will be discussed.
\subsection{Feedback and control}
In active quantum error correction, one may want to know when and what types of corrections to apply to the system qubit(s) during the quantum operation/process. One way to achieve this goal is to perform some kinds of measurement on the quantum system at a current time-step and use the measurement result as a feedback to determine/improve the error correction for future time-steps.

For the particular case of quantum annealing, the system qubits evolve according to a time-dependent system Hamiltonian $H_{S}$. Mathematically, $H_{S} = A(t) H_{i} + B(t)H_{f}$, where $H_{i}$ is the initial system Hamiltonian and $H_{f}$ is the final system Hamiltonian, and $A(t) = 0$ at the end of anneal $t = t_{f}$, and $B(t) = 0$ at $t = 0$. Decoherence arises due to the coupling to a quantized bath (environment). The coupling is described by another system-bath Hamiltonian $H_{SB}$.
Certain decoherence models can be assumed in order to derive a continuous equation describing evolution of system qubits. As the qubit(s) is evolving, measurement and feedback correction can be performed on the qubit(s). One would need to modify the continuous equation to describe the combined effect.


% The definition of feedback is quite broad. The feedback is one such that one observe some information and recycle it into the operation such that the operation becomes better. One example of this is machine learning. The idea of quantum feedback error correction is as follows 
\subsection{Feedback from weak measurement results}
One way to obtain information about quantum system is by weak measurement. Weak measurement is a type of quantum measurement that results in an observer obtaining very little information about the system on average, but also disturbs the state very little~\cite{brun2002simple}. Weak measurement is also often referred to as continuous measurement, where (weak) measurement is performed continuously in successive tiny time-steps. Weak measurement arises from the system qubit successively interacting with environmental (probe) qubits which are subsequently measured (See Fig.~\ref{fig:1}). Depending on the basis in which the environmental qubits is measured, one can obtain different types (jumpy/diffusive) of measurement trajectories for the system qubit being measured.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{feed/continuousmeasurementcenter.png}
    \caption{By successively interacting the system with environmental (probe) qubits which are subsequently measured, we can obtain the weak measurement trajectories.}
    \label{fig:1}    
\end{figure}


When little information is gathered during the measurement, the quantum state is almost entirely preserved. Nevertheless, taking a sufficiently large sample of data still permits the same average information to be extracted as a textbook projective measurement that fully collapses the state. By continuously monitoring partial information about a quantum system, one can control experimental parameters in real time for a variety of purposes, such as error correction, coherence stabilization, state purification. 

\subsubsection{Thermal excitation as error}
In AQC, thermal excitation is considered as an error since we want to preserve the system state as the ground state of the system Hamiltonian. To do that in feedback-based error correction , the system evolution is continuously monitored and feedback is applied conditioned on each weak measurement result. A photo-detection current $I(t)$ of thermal excitation is obtained, $0<t<t_f$. $I(t) = 1$ when a excitation is detected, $0$ otherwise. 

With the assumption of weak-coupling limit, one can derive a master equation describing the evolution of system qubit as:
\begin{align}
\frac{d}{dt} \rho(t) =  -i \left[H_{\textrm{S}}(t) + H_{\textrm{LS}}(t), \rho(t) \right] &+ D[A_{-\omega}(t)]\rho(t) + D[A_{0}(t)]\rho(t) + D[A_{\omega}(t)]\rho(t) \,,
\end{align}
where $A_{-\omega}(t) \propto |\eps_1(t) \rangle  \langle \eps_0(t)| $ is the Lindblad operator of thermal excitation in the instantaneous energy eigenbasis. 
$D[\,\cdot\,]$ refers to the decoherence channel (excitation/dephasing/damping). This master equation can be unraveled into a stochastic Schr\"{o}dinger equation describing the weak measurement. 


\subsubsection{Delay}
After the detection of a thermal excitation ($I(t) = 1$) from ground to excited state, we then want to apply a feedback to correct such errors. However, there usually is a delay between detection and feedback. The most general expression for the effect of the feedback is~\cite{Wiseman-Milburn-book}:
\begin{equation}
[\dot{\rho}_{\text{I}}(t)]_{\text{fb}} = \mathcal{F}[t, \mathbf{I}_{[0, t)}]\rho_{\text{I}}(t)   \,,
\end{equation}
where $ \mathbf{I}_{[0, t)}$ is the complete photocurrent record from time $0$ to $t$, and $\mathcal{F}[t, \mathbf{I}_{[0, t)}]$ is a superoperator.
Assuming that the feedback is of linear functional form, the feedback evolution can be expressed as:
\begin{equation}
[\dot{\rho}_{\text{I}}(t)]_{\text{fb}} = \int_{0}^{\infty} h(s) I(t-s) \mathcal{L}_f \rho_{\text{I}}(t) ds\,,
\end{equation}
where $\mathcal{L}_f$ is the Liouville superoperator representing the feedback control.
If the delay is fixed as $\tau$, an equation incorporating the effect of the feedback is:
\begin{equation}
\label{Eq:implicitfeedbackevolution}
[\dot{\rho}_{I}(t)]_{\text{fb}} = I(t-\tau)\mathcal{L}_f\rho_{I}(t) \,.
\end{equation}
Note that Eq.~\ref{Eq:implicitfeedbackevolution} is non-Markovian for finite $\tau$. Analytical solution of Eq.~\ref{Eq:implicitfeedbackevolution} is hard to obtain and numerical simulation is needed. 

\subsubsection{Types and basis of feedback}
The feedback superoperator $\mathcal{L}_f$ can take the form of Lindbladian or Hamiltonian. In the form of Lindbladian:
\begin{equation*}
\mathcal{L}_f[\,\cdot\,] = F(t)\,\cdot\,F^{\dagger}(t) - \frac{1}{2}\left\{F^{\dagger}(t)F(t), \,\cdot\, \right\} \,.
\end{equation*}

Physically, for the purpose of AQC, this Lindbladian represents a cooling/damping channel in which the qubit is relaxed from excited state to ground state.

In the form of Hamiltonian:
\begin{equation*}
\mathcal{L}_f[\,\cdot\,] = -i\left[H_{\text{fb}}(t), \,\cdot\,\right] \,,
\end{equation*}
where $H_{\text{fb}}(t)$ is called the feedback Hamiltonian. Some examples are
\begin{itemize}
\item $\sigma^x$ in energy eigenbasis
\begin{equation}
H_{\text{fb}}(t) =  \frac{\pi}{2}\left(| \eps_{0}(t-\tau)   \rangle\langle \eps_{1}(t-\tau)  | + | \eps_{1}(t-\tau)   \rangle\langle \eps_{0}(t-\tau)  |\right) \,,
\label{eq:feedbackHenergy}
\end{equation}
\item $\sigma^x$ in computational basis
\begin{equation}
H_{\text{fb}}(t) = H_{\text{fb}} = \frac{\pi}{2} \sigma^x \,,
\label{eq:feedbackHsigmax}
\end{equation}
\item $\sigma^z$ in computational basis
 \begin{equation}
H_{\text{fb}}(t) = H_{\text{fb}} =  \frac{\pi}{2} \sigma^z \,.
\end{equation}
\end{itemize}

Note that in the decoherence model of weak coupling limit, any excitation/relaxation takes place in the energy eigen-basis~\cite{albash2015decoherence}, thus one would expect that the feedback Hamiltonian $\sigma^x$ in energy eigenbasis performs better than $\sigma^x$ in computational eigenbasis (See Fig.~\ref{Fig:2}). Note also that the significance of the $\frac{\pi}{2}$ implies that the feedback Hamiltonian acts instantly (pulse/gate-like). 

Another advantage of such feedback Hamiltonian formalism is that for delay $\tau \rightarrow 0$, one can obtain the feedback master equation that explains the ensemble average of the effect of feedback. 
\begin{align}
\frac{d}{dt} \rho(t) &= -i \left[H_{\textrm{S}}(t) + H_{\textrm{LS}}(t), \rho(t) \right] \notag\\
&+ \left(
e^{-iH_{\text{fb}}(t)}A_{-\omega}(t)\rho(t) A^\dagger_{-\omega}(t)e^{iH_{\text{fb}}(t)}  - \frac{1}{2} \left\{ A_{-\omega}^{\dagger}(t) A_{-\omega}(t) , \rho(t) \right\} \right) \notag\\
&+ D[A_{0}(t)]\rho(t) + D[A_{\omega}(t)]\rho(t)
\label{Eq:feedbackME_H}
\end{align}
This also allows direct simulation, which can be faster than trajectories for a small number of qubits. Fig.~\ref{Fig:2} below compares the two approaches.


\begin{figure}[!h]  
    \centering
    \hspace*{\fill}
    % \begin{subfigure}[t]{0.4\linewidth}
    % \centering
    \includegraphics[width=\linewidth]{feed/energysigmaxinstant_crop.pdf}
    %\includegraphics[width=\linewidth]{energysigmaxinstant_crop_2.pdf} 
    % \caption{} 
    % \label{Fig:2a}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[t]{0.4\linewidth}
    % \centering
    \includegraphics[width=\linewidth]{feed/sigmaxinstant_crop.pdf}
    %\includegraphics[width=\linewidth]{sigmaxinstant_crop_2.pdf} 
    % \caption{}
    % \label{Fig:2b}
    % \end{subfigure}
    % \hspace*{\fill}
    \caption{Linear Schedule. Total annealing time $t_f = 10\mu s$. Instant feedback using (a) $\sigma^{x}$ operator in the instantaneous energy eigenbasis, (b) $\sigma^{x}$ operator in the computational basis. Average over 5000 trajectories. It can also be explained in feedback ME Eq.~\ref{Eq:feedbackME_H} with feedback Hamiltonian (a) Eq.~\ref{eq:feedbackHenergy} ($\tau = 0$), (b) Eq.~\ref{eq:feedbackHsigmax}. QT: quantum trajectories approach. ME: feedback master equation approach.}
    \label{Fig:2}
\end{figure}







\subsection{A need for feedback algorithm}
Note that Eq.~\ref{Eq:implicitfeedbackevolution} only describes the effect of feedback. One will need to include the original system evolution into account.  One difference between AQC and traditional gate-based quantum computing is that AQC relies on a time-dependent annealing Hamiltonian. The system Hamiltonian being time-dependent implies there is an additional freedom, i.e. annealing schedule. One measure of the effectiveness of the quantum error correction is the ground state population at the end of the annealing. Thus one may want to maximize the ground state population at the end of the annealing, i.e.
\begin{align*}
&{\phantom{sssss}}\max_{\boldsymbol{\gamma}}\bra{\epsilon_{0}(t_{f})}\rho_{I}(t_{f})\ket{\epsilon_{0}(t_{f})} \\
&\text{subject to: } \text{experimental constraints}
\end{align*}
\(\boldsymbol{\gamma}\) represents a list of hyperparameters, for example, delay $\tau$, the type of feedback, basis of feedback operator, annealing schedule, etc.~(see Table.\ref{Tab:hyper}). In Fig.~\ref{Fig.3}, only delay $\tau$ varies and other parameters are held constant. There is a non-small (thus experimentally allowed) $\tau$ where the Final GS population is maximized. However, in general since there are many hyperparameters, the optimization problem would be difficult. Other techniques such as machine learning and deep learning would be useful. 

\begin{table}[h!]
\centering
\begin{tabular}{ |c| } 
 \hline
 Hyperparameters \\
 \hline
 Delay $\tau$  \\ 
 Annealing schedule  \\ 
 Type of feedback  \\ 
 Basis of feedback operators  \\ 
 \hline
\end{tabular}
\caption{A table of some examples of hyperparameters for optimization problem.}
\label{Tab:hyper}
\end{table}

\begin{figure}[ht]
\centering
%\includegraphics[width=0.75\textwidth]{feedbackdeltalinear_new_copy}
\includegraphics[width=0.45\textwidth]{feed/feedbackdeltalinear_new_crop.pdf}
\caption{Linear Schedule. Final ground state population. Single qubit. Total annealing time $t_f = 100\mu s$. Dashed purple line is the final ground state population without feedback. Average over 5000 trajectories with Lindbladian feedback.  There is a non-small (thus experimentally allowed) $\tau \approx 60us$ where the Final GS population is maximized.}
\label{Fig.3}
\end{figure}


\chapter{Reverse Annealing: Iterative reverse annealing}
Reverse annealing is a good testbed for open-system simulations. Relaxation is important~\cite{Passarelli2019}.

Reverse annealing has been predicted to have better performance than forward annealing in several systems~\cite{Perdomo-Ortiz2011,Chancellor2017,King2018,Ottaviani2018,Ohkuwa2018, Yamashiro2019,Venturelli2019,Marshall2019}. Passareli et al. \cite{Passarelli2019} tested the effectiveness of reverse annealing on the $p$-spin models with $p=3$. Numerical calculations using the time-dependent Lindblad equation~\cite{Albash2012, Yip2018} showed that the presence of coupling with the boson field significantly changes the performance of reverse annealing. This result shows that the interaction with the environment can lead to an improvement in performance. Since qubits and the environment should always interact with each other on the hardware, it is likely that this result reflects real physical processes in the D-Wave device. However, it is non-trivial if the coupling model  to the environment of Ref.~\cite{Passarelli2019} is good enough to explain experimental data. 

In reverse quantum annealing, the initial state is an eigenstate of the final problem Hamiltonian and the transverse field is cycled rather than strictly decreased as in standard (forward) quantum annealing. We present a numerical study of the reverse quantum annealing protocol applied to the $p$-spin model ($p=3$), including pausing, in an open system setting accounting for dephasing in the energy eigenbasis, which results in thermal relaxation. We consider both independent and collective dephasing and demonstrate that in both cases the open system dynamics substantially enhances the performance of reverse annealing. Namely, including dephasing overcomes the failure of purely closed system reverse annealing to converge to the ground state of the $p$-spin model. We demonstrate that pausing further improves the success probability. The collective dephasing model leads to somewhat better performance than independent dephasing. The protocol we consider corresponds closely to the one implemented in the current generation of commercial quantum annealers, and our results help to explain why recent experiments demonstrated enhanced success probabilities under reverse annealing and pausing.

Iterated reverse annealing (IRA) is a formalism of reverse annealing implemented in current quantum annealers. The system is prepared in a trial solution state, annealed reversely to an inversion point, and then annealed forwardly. It may also be iterated with the last output state as new input. 
We perform IRA experiments on the D-Wave 2000Q device, with a focus on the p-spin problem where p=2. The encoding of problem Hamiltonian is made possible by minor embedding. We examine the dependence of IRA performance on parameters such as problem size, anneal time, inversion points; and also on D-Wave’s functionalities like state reinitialization, number of iterations, pausing. The performance is evaluated in total and partial success probabilities. We can find correct solutions with near certainty. Comparison with standard forward annealing is also made.
We also perform open-system simulations with dephasing in the instantaneous energy eigen-basis. The experimental total success probabilities are well matched. A difference between independent and collective SB coupling model is reported due to spin-symmetry breaking of the classical input. Simulations also show IRA fails in a closed system, suggesting the importance of thermal relaxation in the convergence to the correct solution. 















\section{Iterative reverse annealing}



\label{sec:reverse}
\begin{figure*}[t]
	\subfigure[]{\includegraphics[width = 0.5\columnwidth]{ra1/schedules}\label{fig:schedules}}
	\subfigure[]{\includegraphics[width = 0.5\columnwidth]{ra1/s-of-t}\label{fig:s-of-t}}
	\caption{(a) Annealing schedules (in units such that $\hbar=1$) as a function of the annealing fraction $s(t)$, chosen to be similar to the schedules of the D-Wave processors.
	(b) Annealing fraction $ s(t) $. The blue solid curve represents standard forward quantum annealing of total annealing time $\tau = 500$ns. 
% 	The red dashed curve represents reverse annealing of the same total duration with an inversion point $ (\tinv = 200{\nano\second}, \sinv = 0.6) $.
	}
\end{figure*}	
	
Standard quantum annealing aims at solving optimization problems by employing quantum fluctuations that are slowly decreased to zero, to efficiently explore the solution space~\cite{kadowaki:qa, santoro-martonak, albash:review-aqc}. A system of $ \nspin $ qubits is prepared at $ t = 0 $ in the ground state of a transverse field Hamiltonian, \ie, the uniform superposition over the $ \n = 2^\nspin $ computational basis states $ \{\ket{0}, \ket{1}, \dots, \ket{\n - 1}\} $. 
%The parameter $ \Gamma $ represents the strength of the transverse field. 
The magnitude of transverse field
%$ \hamtf $ 
is then slowly decreased, while the magnitude of the Hamiltonian $ \hamtarget $, encoding the optimization problem, is simultaneously increased. The adiabatic theorem guarantees that if the evolution is long on the timescale set by the inverse of the minimal gap $ \mingap = \min_t [E_1(t) - E_0(t)] $ between the ground state and the first excited state (we set $ \hslash = 1 $ henceforth), then at the end of the anneal $ t = \tf $ the system populates the target ground state of $ \hamtarget $ with a probability $ \pgs $ that approaches unity~\cite{Jansen:07,lidar:102106}. However, any finite sweep rate leads to diabatic Landau-Zener transitions at the avoided crossings~\cite{Joye:LZ}, thus reducing the success probability $ \pgs $ of the adiabatic algorithm. Therefore, the output state of quantum annealing is in general a trial solution of the optimization problem, ideally having a large overlap with the target ground state.
	
Reverse annealing instead aims at refining an already available trial solution~\cite{perdomo:sombrero}. For instance, NP-hard optimization tasks are solved using heuristics, whose output is often an approximation of the true global minimum. The algorithm of reverse annealing is the following.
\begin{enumerate}
	\item At $ t = 0 $, the system is prepared in the trial solution state.
	\item Quantum fluctuations are increased, until a turning point $ \tinv $ is reached during the dynamics. This ends the reversed part of the dynamics.
	\item After the turning point, the dynamics follows the standard quantum annealing schedule; quantum fluctuations are decreased until $ t = \tf $, when the state is eventually measured.
\end{enumerate}
Careful choices of the turning point, and of the initial state, can lead to an improvement in the solution. Moreover, this scheme can also be repeated multiple times, each time starting from the output of the previous stage; hence the terminology of iterated reverse annealing. Assuming that each iteration improves the success probability $ \pgs $, this procedure can systematically improve the quality of the solution. 

We consider the following time-dependent Hamiltonian, suitable for IRA but not ARA (which includes another term):
\begin{equation}
\label{eq:time-dependent-hamiltonian}
	\ham(t) = A\bigl(s(t)\bigr) \hamtf + B\bigl(s(t)\bigr) \hamtarget, \quad  \hamtf = -\sum_{i=1}^{\nspin} \sigma_i^x .
\end{equation}
Since we only consider the IRA protocol, henceforth we simply refer to it as reverse annealing. The function of time $ s(t) $ in Eq.~\eqref{eq:time-dependent-hamiltonian} is the annealing fraction (or dimensionless time) and satisfies $ 0 \le s(t) \le 1 $ for all $ t $. The two functions $ A(s) $ and $ B(s) $ determine the annealing schedule, which we choose to match the annealing schedule of the D-Wave processors [see Fig.~\ref{fig:schedules}]. They satisfy $ A(0) \gg B(0) $ and $ B(1) \gg A(1) $.
	
The functional form of $ s(t) $ distinguishes between standard (forward) and reverse annealing. In standard quantum annealing the dimensionless time is defined as $ s(t) = t / \tf $, $ \tf $ being the annealing time. Thus, $ s(t) $ is a monotonic function of $ t $, and is represented in the plane $ (t, s) $ by a straight line going from $ (0, s_0) $ to $ (\tau, s_1) $, where $ s_0 = s(0) = 0 $ and $ s_1 = s(\tau) = 1 $. This is shown in Fig.~\ref{fig:s-of-t} using a blue solid line, for $ \tau = 500$ ns. During standard quantum annealing, quantum fluctuations are very large at $ t = 0 $, and decrease monotonically until $ t = \tau $.
	
In contrast, in reverse annealing $ s_0 = s_1 = 1 $. Starting from $ s = s_0 $, where quantum fluctuations are zero, the annealing fraction is first decreased until it reaches the inversion point, $ s = \sinv $, at a time $ t = \tinv $. In this first branch, quantum fluctuations are increased. At $ s = \sinv $, the annealing fraction is then increased towards $ s = s_1 $, and quantum fluctuations are decreased again to zero. In Fig.~\ref{fig:s-of-t}, we show a typical function $ s(t) $ for a reverse annealing of annealing time $ \tf = \SI{500}{\nano\second} $ with an inversion point $ (\tinv = \SI{200}{\nano\second}, \sinv = 0.6) $, using a red dashed line.
		
In general, $ \sinv $ and $ \tinv $ can be chosen independently of each other. However, in this work we choose the following linear relation, in order to have only one free parameter:
\begin{equation}
\label{eq:inversion-time}
	\tinv = \tf (1 - \sinv)\ , \ \ \sinv \ne 0, 1.
\end{equation}
In this way, we have that
\begin{equation}\label{eq:schedule}
	s(t) =
	\begin{cases}
		1-t / \tf & \text{for $ t \le \tinv $},\\
		\frac{1 - \sinv}{\tf \sinv} t + \frac{2 \sinv - 1}{\sinv} & \text{for $ t > \tinv $}.
	\end{cases}
\end{equation}
%To avoid ill-defined cases, in the following we will only consider $ \sinv \ne 0, 1 $.
	
Another possible choice would be to fix $ \tinv $ so that the two slopes are the same, \ie, $ \tinv = \tf / 2 $ for all choices of $ \sinv $. This is similar in spirit to what is discussed in Ref.~\cite{nishimori:reverse-pspin-2}. 
	
%	Simulating quantum systems on classical hardware requires an exponentially large amount of computational resources, due to the dimension of the Hilbert space growing exponentially as a function of the number of qubits. Symmetries can often be exploited to restrict to interesting subspaces of the Hilbert space, having smaller dimensions. In this regards, having access to toy models with workable exact solutions and useful symmetries is paramount. 
In what follows, we will focus on the fully-connected ferromagnetic $ p $-spin model, a model with a permutationally invariant Hamiltonian and a nontrivial phase diagram, often used as a benchmark for the performance of quantum annealing~\cite{gross:p-spin, derrida:p-spin}. 
%We will introduce it in the next Section.
	
\section{Ferromagnetic $ p $-spin model}\label{sec:pspin}

The Hamiltonian of the ferromagnetic $ p $-spin model, in dimensionless units, reads
\begin{equation}\label{eq:pspin}
	\hamtarget = -\frac{\nspin}{2}{\left(\frac{1}{\nspin} \sum_{i = 1}^{\nspin} \sigma^z_i\right)}^p,
\end{equation}
with $ p \ge 2 $. For even $ p $, there are two degenerate ferromagnetic ground states, whereas for odd $ p $ the ferromagnetic ground state is nondegenerate. For $ p = 2 $, the Hamiltonian of Eq.~\eqref{eq:time-dependent-hamiltonian} is subject to a second-order QPT in the thermodynamic limit at the critical point $ \scrit $ (or, equivalently, $ \tcrit = \tf \scrit $), separating a para- and a ferromagnetic phase. For $ p > 2 $, the QPT is first-order~\cite{bapst:p-spin}. The presence of QPTs affects also the finite-size behavior of the system, as the minimal spectral gap $ \mingap $, found at $ \sgap $ ($ \tgap = \tf \sgap $), closes as $ \nspin^{-1/3} $ for $ p = 2 $ or exponentially in $ \nspin $ for $ p > 2 $. $ \sgap $ (\ie, $ \tgap $) approaches $ \scrit $ (\ie, $ \tcrit $) as $ \nspin \to \infty $. First-order QPTs are especially detrimental for quantum annealing, as the annealing time has to grow exponentially with the system size to compensate the closure of the gap at $ s = \sgap $. In the following, we will focus on the case $ p = 3 $.
	
We can define the total spin operator $\mathbf{S} = (S_x,S_y,S_z)$ and the dimensionless magnetization operators
\begin{equation}
	m_{\alpha} = \frac{1}{\nspin} S_{\alpha} ,\quad S_{\alpha} = \sum_{i = 1}^{\nspin} \sigma_i^{\alpha}, \quad \alpha\in\{x,y,z\}
\end{equation}
that allow the rewriting of the time-dependent Hamiltonian of Eq.~\eqref{eq:time-dependent-hamiltonian} as
\begin{equation}
	 \ham(t) = -\frac{A(t)}{2} S_x - \frac{B(t)n}{2} m_z^p .
\end{equation}
%\begin{equation}
%	 \ham(t) = -\frac{A(t)}{2} S_x - \frac{B(t)}{2 \nspin^{p - 1}} S_z^p .
%\end{equation}
%with $ \Gamma = 1 $.
Since $[\mathbf{S}^2,S_z]=0$ and both are Hermitian, they share an orthonormal basis $\{\ket{S,\mu_S}\}$ such that the eigenvalues of $\mathbf{S}^2$ are $S(S+1)$ with $S\in\{0,1/2,1,\dots,\nspin/2\}$ for even $ \nspin $ and $S\in\{1/2,1,\dots,\nspin/2\}$ for odd $ \nspin $, and the eigenvalues of $S_z$ are $\mu_S \in \{-S,-S+1,\dots,S\}$.
In the subspace with maximum spin $S=\nspin/2$, we instead label the basis states as $ \ket{w} \equiv \ket{\nspin/2 - w} $, with $ w \in \{0, 1, \dots, \nspin\} $. These are the eigenstates of $ m_z $ with eigenvalues $ m = 1 - 2 w / \nspin $. The target state is the ferromagnetic ground state $ \ket{0} $, \ie, the eigenstate of $ m_z $ with eigenvalue $ m = 1 $. 

The Hamiltonian of the $ p $-spin model commutes with $\mathbf{S}^2$. Hence sectors differing by $S$ do not become coupled under the dynamics generated by the $ p $-spin model Hamiltonian. Since the ferromagnetic ground state and the initial one belong to the subspace with maximum spin $ S = \nspin / 2 $, the interesting dynamics occurs in this subspace, whose dimension scales \emph{linearly} with the number of qubits: $ \n = \nspin + 1 $. This fact enables us to perform numerical calculations with relative large numbers of qubits $\nspin$.

In the following, we will start reverse annealing in each of the $ \nspin $ excited states $ \{\ket{1}, \dots, \ket{\nspin} \}$ of $ \hamtarget $ in the symmetric sector with $ S = \nspin/2 $. The similarity to the ferromagnetic ground state is quantified by the corresponding starting eigenvalue of $ m_z $, denoted $ m_0 $. Note that the $ w $th excited state differs from the ferromagnetic ground state by $ w $ spin flips. Therefore, the initial state and the target solution differ by a fraction $ c = \nspin_\uparrow / \nspin = 1 - w /\nspin $ of up-aligned qubits. These parameters are also related to the Hamming distance $ d\ped{H} $, 
%\ie, the number of $ -1 $ of the state in the single qubit basis. In fact, 
via $ d\ped{H} = \nspin - \nspin_\uparrow = \nspin (1 - c) $.
	
	

\section{Unitary dynamics}
\label{sec:unitary}

\begin{figure*}[tb]
	\subfigure[]{\includegraphics[width = \columnwidth]{ra1/unitary-tf-100}\label{fig:unitary-tf-100}}
	\subfigure[]{\includegraphics[width = \columnwidth]{ra1/unitary-scaling}\label{fig:unitary-scaling}}
	\caption{(a) Success probability in unitary reverse annealing as a function of the inversion point $ \sinv $, for several values of the magnetization of the initial state. The dashed vertical line indicates $ \sinv = \sgap \approx 0.309 $. The annealing time is $ \tf = \SI{100}{\nano\second} $. We sampled the interval $ \sinv \in \rngopen{0}{1} $ using a step size of $ \Delta s = 0.002 $, and repeated the dynamics for each choice of $ \sinv $. (b) Maximum success probability achievable with unitary reverse annealing, as a function of the magnetization of the initial state, for two annealing times: $ \tf = \SI{100}{\nano\second} $ and $ \tf = \SI{1000}{\nano\second} $. The inset zooms in on the region $ m\in\rng{-1.0}{0.0} $. Note the logarithmic scale on the vertical axis.}
\end{figure*}

In this section we study the closed system case of a system of $ \nspin = 20 $ qubits, with $ p = 3 $. For our choice of parameters and in terms of the annealing schedules shown in Fig.~\ref{fig:schedules}, the $ p $-spin system has a minimal gap $ \mingap \approx \SI{2.45}{\giga\hertz} $ at $ \sgap \approx 0.309 $. The annealing time is $ \tf = \SI{100}{\nano\second} $. 
%We start without including system-environment interactions.
	
In Fig.~\ref{fig:unitary-tf-100}, we report the ground state population $ \pgs $  at $ t = \tf $, as a function of the inversion point $ \sinv $, for several initial states: $ m_0 = \text{\numlist{0.9;0.8;0;-1}} $. Recall that the target ground state $ \ket{0} $ has $m=1$. We focus on the region $ \sinv \in \rnglopen{0.0}{0.5}$.
	
The rightmost part of Fig.~\ref{fig:unitary-tf-100} corresponds to cases in which the anneal is reversed too early, \ie, for $ \tinv < \tgap $ and $ \sinv > \sgap $. The system does not cross its quantum critical point, and the success probability is zero. Therefore, no effects on the outcome of the procedure are visible, as the dynamics is slow compared with the minimal inverse level spacing and diabatic transitions are exponentially suppressed. Thus, the system is forced to stay in its initial state, or transition to other excited states. In fact, avoided crossings between pairs of excited eigenstates occur at $ s > \sgap $ for this model, and Landau-Zener processes can further excite the $ p $-spin system.
	
On the other hand, if $ \sinv < \sgap $ the system crosses the minimal gap twice. Here, the success probability benefits from Landau-Zener processes, inducing transitions towards the ground state. In this region, we also note some non-adiabatic oscillations of the success probability, due to the finite annealing time. These oscillations are more evident for large $ m_0 $. As expected from the adiabatic theorem, they are suppressed for longer annealing times. For instance, we verified that they are no longer visible for $ \tf = \SI{1000}{\nano\second} $ (not shown). The sharp rise of the success probability for $ m_0 = 0.9 $ occurs exactly at $ \sinv = \sgap $. For smaller values of $ m_0 $, the success probability rises more smoothly, as the ground state is reached after a preliminary sequence of Landau-Zener transitions between pairs of excited states, whose corresponding avoided crossings occur at $ s > \sgap $. For $ m_0 = 0.8 $, a very small rise of the success probability can still be observed around $ \sinv = \sgap $. This is due to the fact that during the reverse annealing, the system prepared in the second excited state first encounters an avoided crossing with the first excited state, where part of the population is transferred to the latter, and then the avoided crossing with the ground state, where the system populates its ground state. After reversing the dynamics, the two avoided crossings are encountered again (in the reverse order) and part of the population gets excited, thus reducing the success probability $ \pgs $.

As expected, reverse annealing is more effective when the initial state is close to the correct ground state. Moreover, as is also clear from Fig.~\ref{fig:unitary-tf-100}, the inversion time $ \sinv $ must be increasingly close to $0$ for decreasing $ m_0 $, in order to obtain a nonzero success probability at $ t = \tf $. This means that almost the entire dynamics is spent in the reverse part of the annealing, and the system is eventually quenched towards $ s = s_1 $ for $ t \approx \tf $. Even so, if the initial state is too far in energy from the correct solution, the success probability of reverse annealing is always close to zero, as evident from the curves for $ m_0 = 0 $ and $ m_0 = -1 $ in Fig.~\ref{fig:unitary-tf-100}. 
	
The maximum success probability decreases rapidly as a function of $ m_0 $. This is clearly seen in Fig.~\ref{fig:unitary-scaling}, where we report the maximum attainable success probability as a function of $ m_0 $, for annealing times $ \tf = \text{\SIlist{100;1000}{\nano\second}} $. 
%The maximum success probability is also affected by the total annealing time. In fact, 
Increasing the annealing time reduces non-adiabaticity and results in a lower success probability, compared with that at the end of a faster reverse anneal. As shown in Fig.~\ref{fig:unitary-scaling}, which zooms in on the region $ m_0 \in \rng{-1}{0} $, this decrease can be of several orders of magnitude for poorly chosen trial solutions.  The influence of the annealing time is less pronounced close to $ m_0 = 1 $, and more evident for intermediate and lower values of $ m_0 $. This is consistent with the adiabatic theorem, since a longer anneal time guarantees that the system will have a higher probability of remaining close to the initial eigenstate it has the largest overlap with (not necessarily the ground state)~\cite{Jansen:07}. 

Adopting a conventional quantum annealing procedure, the success probability in the case of $ \tf = \SI{100}{\nano\second} $ would be $ P_0 = 0.96 $. This value is larger than any $ P_0 $ achievable using reverse annealing. However, this argument cannot be used to discredit reverse annealing for two main reasons. First, it is clear that, in the analyzed case, we are very close to adiabaticity, where conventional annealing is efficient. Second, as clarified in the next Sections, the role of dissipation may strongly affect this scenario.
	
The results of this Section are in agreement with those reported in Ref.~\cite{nishimori:reverse-pspin-2}. Namely, as is clear from Fig.~\ref{fig:unitary-scaling}, upon iteration the IRA protocol will only decrease the success probability under unitary, closed system dynamics, unless the initial state was already chosen as the solution of the optimization problem. 
	
\begin{figure*}[t]
	\subfigure[]{\includegraphics[width = \columnwidth]{ra1/dissipative-tf-100}\label{fig:dissipative-tf-100}}
	\subfigure[]{\includegraphics[width = \columnwidth]{ra1/dissipative-tf-500}\label{fig:dissipative-tf-500}}
	\caption{Success probability in reverse annealing as a function of the inversion point $ \sinv $, for several values of the magnetization of the initial state. The $ p $-spin system is coupled to a collective dephasing bosonic environment as in Eq.~\eqref{eq:system-bath-collective}, and the coupling strength is $ \eta = \num{1e-3} $. The dashed vertical line denotes the time $ \sgap $ of the avoided crossing between the ground state and the first excited state. In (a) the annealing time is $ \tf = \SI{100}{\nano\second} $, in (b) $ \tf = \SI{500}{\nano\second} $. We sampled the interval $ \sinv \in \rngopen{0}{1} $ using a step $ \Delta s = 0.02 $. All other parameters are given in the main text.}
	\label{fig:dissipative}
\end{figure*}		
	

\section{Open system dynamics subject to dephasing-induced relaxation}\label{sec:dissipative}
	
Physical quantum processors always interact with the surrounding environment, which induces decoherence and thermal excitation/relaxation, which in turn impacts the performance of quantum annealing~\cite{childs:robustness,amin_decoherence_2009,albash:decoherence}. We 
%use a description of the bath in terms of harmonic oscillators, and we 
assume weak coupling between the qubit system and the environment. 
%We formulate the dynamics of the reduced system in terms of a quantum dynamical semigroup. 
It can then be shown that the reduced system density matrix evolves according to a quantum master equation in time-dependent Lindblad form~\cite{zanardi:master-equations}, known as the adiabatic master equation:
\begin{equation}\label{eq:lindblad}
	\frac{d\rho(t)}{dt} = \iu \bigl[\rho(t), \ham(t) + \ham\ped{LS}(t)\bigr] + \diss\bigl[\rho(t)\bigr].
\end{equation} 
In Eq.~\eqref{eq:lindblad}, $ \ham\ped{LS}(t) $ is a Lamb shift term and $ \diss $ is the dissipator superoperator, which makes the dynamics non-unitary and irreversible. They are expressed in terms of Lindblad operators, inducing dephasing or quantum jumps (pumps and decays) between pairs of adiabatic energy eigenstates~\cite{yip:mcwf}:
\begin{gather}\label{eq:hls-diss}
	\ham\ped{LS} = \sum_{ab} L_{ab}^\dagger(t) L_{ab}(t) S_{ab}(\omega_{ab});\\
	\begin{align}
	\diss[\rho(t)] &= \sum_{ab} \gamma_{ab} \biggl( L_{ab}(t) \rho(t) L_{ab}^\dagger(t) \notag\\
	&\quad- \frac{1}{2} \left\lbrace L_{ab}^\dagger(t) L_{ab}(t), \rho(t) \right\rbrace \biggr).
	\end{align}
\end{gather}
The Lindblad operators are determined by the instantaneous eigenbasis of the system Hamiltonian $H(t)$ and the system-bath interaction Hamiltonian $ \hamsysbath $. In general, this coupling Hamiltonian involves local operators
%, \ie, ``position'' degrees of freedom both for the qubits in real space (\eg, $ \sigma^z_i $), and for the harmonic oscillators in  momentum space (\eg, $ a_{k, i} + a_{k, i}^\dagger $). This generic form, however, 
that break the spin symmetry of the $ p $-spin model, as each qubit is then coupled to its own bath. We study both this independent decoherence model and the collective decoherence model, wherein  %Therefore, we will adopt a specific form for the interaction potential, where 
all the qubits are coupled to a collective bath with the same coupling energy $ g $, in order to preserve the spin symmetry. More specifically, we first consider collective dephasing, for which the system-bath coupling Hamiltonian is
\begin{equation}\label{eq:system-bath-collective}
	\hamsysbath\api{col} = g S_z 
	%\sum_k (a_k + a_k^\dagger),
	\otimes B ,
\end{equation}
where $B$ is a bath operator [e.g., $B = \sum_k (a_k + a_k^\dagger)$ for an oscillator bath with annihilation operators $a_k$ for the $k$th bosonic mode].
The Lindblad operators are represented in the instantaneous energy eigenbasis of $H(t)$ as~\cite{zanardi:master-equations}:
\begin{equation}\label{eq:Lab(t)}
	L_{ab}(t) = \braket{E_a(t)| S_z |E_b(t)} \ket{E_a(t)}\bra{E_b(t)}.
\end{equation}
This represents collective dephasing in the energy eigenbasis, wherein the dephasing process randomizes the relative phase between eigenstates of the system Hamiltonian. Thus, this model does not support phase coherence between energy eigenstates.\footnote{It is worth pointing out a caveat. Namely, the collective dephasing model in general supports decoherence free subspaces (DFSs), \ie, subspaces that evolve unitarily despite the coupling to the bath~\cite{Zanardi:97c,Lidar:1998fk}. For instance, the $ S = 0 $ subspace (for even $ \nspin $) is a DFS of the $ p $-spin model. However, the $p$-spin model is unsuitable for performing quantum annealing inside a DFS, since its Hamiltonian consists of operators that preserve the DFS, so that no dynamics would take place if we were to try to encode a computation using states inside the DFS. Instead, to obtain meaningful dynamics (performing a computation) subject to the collective dephasing model, we would need to add Heisenberg exchange terms to the system Hamiltonian~\cite{Kempe:2001uq}.} As a consequence, thermal relaxation tends to equilibrate the system towards its Gibbs state, with a characteristic timescale set by the inverse of the bath spectral density at the gap frequency~\cite{albash:decoherence}.
	
If instead the qubit system is coupled to independent, identical baths, the system-bath coupling operator becomes
\begin{equation}\label{eq:system-bath-independent}
	\hamsysbath\api{ind} = g \sum_{i} \sigma_i^z \otimes B_i, 
\end{equation}
where, e.g., in the bosonic case $B_i = \sum_k (a_{k, i} + a_{k, i}^\dagger)$. Thermal relaxation effects occur here similarly to the collective dephasing case.
However, simulations in this case are more demanding due to the fact that the spin symmetry is broken and that we have $\nspin$ times as many Lindblad operators, \ie,
\begin{equation}
	L_{ab, i}(t) = \braket{E_a(t)| \sigma_i^z |E_b(t)} \ket{E_a(t)}\bra{E_b(t)}.
\end{equation}
Therefore, in this case we will only investigate reverse annealing starting from the first excited state in the symmetric subspace with maximum spin, \ie, $ \ket{w = 1} $, for $ \nspin \in \{3,\dots,8\}$. Moreover, for the particular cases of $ \nspin = 7 $ and $ \nspin = 8 $, we truncate our system to the lowest $ 29 $ and $ 37 $ eigenstates, respectively, to speed up the numerics. This choice is made since the first three levels of the maximum spin subspace at $ s = 1 $ are spanned by $ \sum_{i=0}^2 \binom{7}{i} = 29 $ (for $ \nspin = 7 $) and $ \sum_{i=0}^{2} \binom{8}{i} = 37 $ (for $ \nspin = 8 $) energy eigenstates. We confirm that this is a good approximation by checking that the total population among these levels is close to $1$ during the reverse annealing when additional levels are included in the simulation.
	
\begin{figure}[t]
	\centering
	\includegraphics[width = \linewidth]{ra1/individual-vs-collective-nopausing.pdf}
	\caption{Success probability in reverse annealing as a function of the inversion point $ \sinv $, for $\nspin \in \{3,\dots,8\}$. The initial state is the first excited state of the maximum spin subspace ($ m_0 = 1 - 2/\nspin $). The dashed vertical line denotes the time $ \sgap $ of the avoided crossing between the ground state and the first excited state. The annealing time is $ \tf = \SI{100}{\nano\second} $. We sampled the interval $ \sinv \in (0, 1) $ using a step size of $ \Delta s = 0.005 $.}
	\label{fig:withoutpausing}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{ra1/peak-fidelity.pdf}
	\caption{Maximum success probability achievable with reverse annealing as a function of the number of qubits $ \nspin $, using the collective and the independent dephasing models of Eqs.~\eqref{eq:system-bath-collective} and~\eqref{eq:system-bath-independent}, respectively. The annealing time is $ \tf = \SI{100}{\nano\second} $.}
	\label{fig:fiddependenceonn}
\end{figure}

\begin{figure*}[tb]
	\subfigure[]{\includegraphics[width = \columnwidth]{ra1/dissipative-tf-100-pause-100}	\label{fig:dissipative-tf-100-pause-100}}
	\subfigure[]{\includegraphics[width = \columnwidth]{ra1/dissipative-tf-100-pause-400}\label{fig:dissipative-tf-100-pause-400}}
	\caption{Success probability in paused reverse annealing for the collective dephasing model, as a function of the inversion point $ \sinv $, for several values of the magnetization of the initial state. The coupling strength is $ \eta = \num{1e-3} $. The annealing time is $ \tf = \SI{100}{\nano\second} $. In (a) a pause of duration $ \lpause = \SI{100}{\nano\second} $ is inserted at the inversion point, while in (b) $ \lpause = \SI{400}{\nano\second} $. All other parameters are given in the main text. Dotted lines with empty symbols refer to open system reverse annealing of time $ \tf = \SI{100}{\nano\second} $ and no pauses. The dashed vertical line denotes $ \sinv = \sgap $. The interval $ \sinv \in \rngopen{0}{1} $ is sampled using a step size $ \Delta s = 0.02 $.}
	\label{fig:dissipative-tf-100-pause}
\end{figure*}		

\begin{figure}[tb]
	\includegraphics[width = \linewidth]{ra1/individual-vs-collective-pausing}
	\caption{Comparison of the success probability in reverse annealing for the collective and independent dephasing models, as a function of the inversion point $ \sinv $, for $\nspin \in\{3,\dots,8\}$. The initial state is the first excited state of the maximum spin subspace ($m_0 = 1 - 2/\nspin$). The dashed vertical line denotes the time $\sgap$ of the avoided crossing between the ground state and the first excited state. The annealing time is $\tf = \SI{100}{\nano\second}$, and a pause of duration $ \lpause = \SI{100}{\nano\second}$ is inserted at the inversion point.}
	\label{fig:withpausing}
\end{figure}

The adiabatic master equation in Eq.~\eqref{eq:lindblad} is unraveled using a time-dependent Monte Carlo wavefunction (MCWF) approach~\cite{yip:mcwf}. The advantage of MCWF is that it allows to work with wavefunctions rather than density matrices, thus saving quadratically in the dimension of the objects we need to store for numerical calculations. The tradeoff is that to recover the statistical properties of the density operator we need to average over a large number $ K $ of independent trajectories. For the collective system-bath coupling of Eq.~\eqref{eq:system-bath-collective}, the time evolution operator of each trajectory is generated by the effective non-Hermitian Hamiltonian
\begin{align}\label{eq:non-hermitian-hamiltonian}
	\ham\ped{eff}(t) &= \ham(t) + \ham\ped{LS}(t) - \frac{\iu}{2} \sum_{a \ne b} \gamma_{ab} L_{ab}^\dagger(t) L_{ab}(t) \notag \\ & \quad-\gamma_0 \frac{\iu}{2} \sum_{ab}  L_{aa}^\dagger(t) L_{bb}(t),
\end{align}
where $ \gamma_{ab} $ and $ \gamma_0 $ are the rates for jumps and dephasing, respectively. They are related to the temperature and to the spectral density of the bosonic bath,
\begin{equation}\label{eq:spectral-density}
	J(\omega) = g^2 \sum_k \delta(\omega -  \omega_k) = 2\pi \eta \omega e^{-\omega / \omegac},
\end{equation}
where $ \omega_k $ are the bath eigenfrequencies, $ \omegac $ is a high-frequency cutoff and $ \eta $ is the dimensionless coupling strength. We fix $ \omegac = \SI{1}{\tera\hertz} $ and $ \eta = \num{1e-3} $. The working temperature is chosen to be $ T = \SI{12.1}{\milli\kelvin} = \SI{1.57}{\giga\hertz} $, as in experimental quantum annealing systems~\cite{dwave-site}. Eq.~\eqref{eq:non-hermitian-hamiltonian} is easily extended to the independent dephasing case by including a summation over $ i $ for the Lindblad operators and in the Lamb shift term.
	
The time evolution operator generated by the non-Hermitian Hamiltonian of Eq.~\eqref{eq:non-hermitian-hamiltonian} is not unitary. Therefore, the norm of the wavefunction decays in time. Whenever the squared norm decreases below a randomly extracted threshold $ r \in \rng{0}{1} $, a quantum jump occurs, projecting the wavefunction on one of the eigenstates of the Hamiltonian $ \ham(t) $.
The adiabatic master equation dynamics is found after averaging over all stochastic trajectories. In this work, we fix $ K = 5000 $ trajectories and consequently find relative Monte Carlo errors $ \delta\ev{O} / \ev{O} $ of the order of $ \SI{1.5}{\percent} $ over all observables $ O $.
	
We repeat the simulations we reported in Sec.~\ref{sec:unitary} for $ \nspin = 20 $, $ p = 3 $ and $ \tf = \SI{100}{\nano\second} $, but now include the role of the environment. We consider both the collective and independent dephasing models. 
	
In Fig.~\ref{fig:dissipative-tf-100}, we show the success probability as a function of the inversion time $ \sinv $, for the four initial magnetizations $ m_0 = \text{\numlist{0.9;0.8;0;-1}} $. Monte Carlo errors are of the order of the point size in all cases and are invisible. 
	
As in the unitary case, if the inversion occurs too early (\ie, for $ \tinv \ll \tgap $, or, equivalently, $ \sinv \gg \sgap $), the reverse annealing protocol fails to find the ferromagnetic ground state. In fact, thermal excitations are suppressed, as well as Landau-Zener transitions, due to the large level spacing, compared with the temperature and the inverse of the annealing time. For $ \tinv \approx \tgap $ ($ \sinv \approx \sgap $), however, the scenario is drastically different from the unitary case of Fig.~\ref{fig:unitary-tf-100}. 

	
The first difference is that the success probability can be nonzero even if the inversion occurs for $ \sinv \gtrsim \sgap $, especially for $ m_0 = 0.9 $, where the tail of the curve extends to $ \sinv \approx 0.75 $. When the instantaneous gap is of the same order of magnitude as the temperature, thermal processes influence reverse annealing even before crossing the minimal gap. Second, for all $ m_0 $ we observe a sudden increase in the success probability around $ \sinv \approx \sgap $, that eventually brings all curves to an almost flat region at $ \sinv < \sgap $, where the success probability reaches the large value $ \pgs \approx 0.957 $. The value of the maximum success probability at the plateau is $ m_0 $-independent within Monte Carlo errors. The time at which the success probability starts to increase with respect to the baseline depends on $ m_0 $. Moreover, the flat region is wider for larger $ m_0 $, although it has a finite width for all $ m_0 $.
	
These results show that even trial solutions far in Hamming distance from the ferromagnetic ground state can result in a large success probability at the end of a reverse anneal. Moreover, the time window in which inverting the annealing favors the ferromagnetic ordering is relatively large. 
	
We also studied a longer annealing time, $ \tf = \SI{500}{\nano\second} $, as shown in Fig.~\ref{fig:dissipative-tf-500}.
%, where we show the success probability $ \pgs $ as a function of the inversion time, for $ m_0 = \text{\numlist{0.9;0.8;0;-1}} $. 
Here, we note that the onset of the success probability plateau shifts towards longer values of $ \sinv $, compared with the $ \tf = \SI{100}{\nano\second} $ case. Therefore, the plateau is wider, and the maximum success probability at the plateau is $ \pgs \approx 1 $ within Monte Carlo errors for all $ m_0 $ we considered. This is in contrast with the unitary case of Fig.~\ref{fig:unitary-scaling}, where increasing the annealing time had detrimental effects on the algorithm. This evidence supports the notion that the success probability enhancement is due to thermal effects, rather than due to purely unitary quantum dynamics~\cite{passarelli:pspin}. Moreover, the adiabatic theorem for open quantum system guarantees convergence to the steady state of the superoperator generator of the dynamics in the large $\tf$ limit~\cite{Venuti:2015kq,Venuti:2018aa}. This too helps to explain our observations: the steady state of the Davies-Lindblad generator of the open system dynamics we considered here is the Gibbs distribution of the final Hamiltonian, which at sufficiently low temperature relative to the gap is the ferromagnetic ground state. Recall that in our case $ \mingap \approx \SI{2.45}{\giga\hertz} $ (at $ \sgap \approx 0.309 $) and $ T = \SI{1.57}{\giga\hertz} $.

Comparing these results with conventional forward annealing in the presence of dissipation, we note that the success probability at the plateau is similar to that of standard quantum annealing for $ \eta = \num{1e-3} $ ($ P_0 = 0.98 $). The reason is that collective dephasing favors the ferromagnetic ordering in the $p$-spin model and its induced relaxation increases the success probability compared to the isolated case, in agreement with previous findings~\cite{passarelli:pspin}. We also observe that when the annealing is far from adiabaticity (e.g. $\tf = \SI{1}{\nano\second}$), reverse annealing becomes a more favorable approach to forward annealing for the $p$-spin model.
				
We also compare the collective and independent dephasing models of Eqs.~\eqref{eq:system-bath-collective} and~\eqref{eq:system-bath-independent}.
Fig.~\ref{fig:withoutpausing} shows the simulation results for the two models using the adiabatic master equation of Eq.~\eqref{eq:lindblad} for $ \nspin \in \{3,\dots,8\} $. As shown in the figure, simulations using the collective dephasing model have larger success probabilities for almost every $ \sinv$. This is because, in the independent dephasing model, other states not in the subspace of maximum spin become accessible by thermal excitation or diabatic transition during the reverse anneal. For all of the system sizes we simulated, we had to reverse anneal to a smaller inversion point $ \sinv $ for the independent dephasing model to achieve the same success probability as the collective dephasing model. Moreover, the maximum success probability achievable is always smaller for the independent dephasing model. The success probabilities from both models, however, are very similar as $ \sinv \to 0 $, \ie, in the quench limit of the direct part of the evolution. 
	

Figure~\ref{fig:fiddependenceonn} shows how the maximum success probability (over $ \sinv $) of both bath models depends on the number of qubits. As $ \nspin $ increases, the maximum success probability of the independent dephasing model decreases more rapidly than that of the collective dephasing model. While we can infer that if we modeled independent dephasing for $ \nspin = 20 $ we would not observe as large success probabilities as in Fig.~\ref{fig:dissipative}, we stress that  reverse annealing in the independent dephasing model still yields a significantly larger success probability  (for the same $\nspin$ values) than the unitary dynamics case described in Section~\ref{sec:unitary}.
	
	

\section{Open system dynamics with a pause}\label{sec:pausing}
	

Quantum annealing in the presence of a low temperature bath can benefit from pauses inserted at certain times during the dynamics~\cite{marshall, passarelli:pausing}. During a pause, $ s(t) = \text{constant} $, and the system evolves with a time independent Hamiltonian, subject to dephasing. When a pause is inserted some time after $ \sgap $, the environment favors a redistribution of the repopulation according to the Gibbs state at the pause point; at sufficiently low temperature (relative to the gap at this point), this can result in a repopulation of the instantaneous ground state. In this section, we show that pauses at the inversion point can further improve the performance of reverse annealing of the $ p $-spin model.
	
	
We repeat the simulations for $ \nspin = 20 $, $ p = 3 $ and $ \tf = \SI{100}{\nano\second} $, using the collective dephasing model. A pause of duration $ \lpause = \tf $ is inserted at $ t = \tinv $, so that the total annealing time, including the pause, is $ \tf' = \tf + \lpause = \SI{200}{\nano\second} $. 
	
In Fig.~\ref{fig:dissipative-tf-100-pause-100}, we report the success probability as a function of the inversion point, for starting magnetizations $ m_0 = \text{\numlist{0.9;0.8;0;-1}} $. We compare the paused case with the unpaused case, for which $ \tf = \SI{100}{\nano\second} $. 
As can be seen in the figure, if the dynamics is reversed too early ($ \sinv \gg \sgap $), the success probability at the end of the anneal vanishes. The level spacing is large compared with the temperature. The relaxation rate is small and the pause is too short to have impact on the dynamics. 
	
However, the presence of a pause significantly changes the outcome of the annealing around $ \sinv \approx \sgap $.  In fact, when a pause is inserted at $ \sinv \gtrsim \sgap $, the success probability reaches $ \pgs \approx 1 $ for a wide range of inversion points and for all $ m_0 $, within Monte Carlo errors. Here, the ground state is completely repopulated by thermal relaxation. This is in contrast with conventional quantum annealing, where the success probability exhibits a peak as a function of the pausing time, when the pause is inserted about $ \SI{20}{\percent} $ later than $ \sgap $, and then rapidly returns to its baseline value~\cite{marshall, passarelli:pausing}.
In contrast, for $ \sinv < \sgap $, the effect of the pause is negligible; the solid (with pause) and dotted (no pause) lines in Fig.~\ref{fig:dissipative-tf-100-pause-100} overlap in this region.

We repeated our analysis for a pause duration $ \lpause = \SI{400}{\nano\second} $, with total annealing time $ \tf' = \SI{500}{\nano\second} $. As shown in Fig.~\ref{fig:dissipative-tf-100-pause-400}, the longer pause duration affects the results only marginally. Comparing with Fig.~\ref{fig:dissipative-tf-100-pause-100}, we note that the qualitative behavior of the curves is the same in the two cases. The pause duration affects mostly the region $ \sinv \gtrsim \sgap $. A longer pause enhances thermal relaxation, thus the success probability starts to increase from its baseline earlier than for shorter $ \lpause $. This results in a wider plateau where the success probability is large, compared with Fig.~\ref{fig:dissipative-tf-100-pause-100}.
	
Finally, we compare the collective and independent dephasing models while including pausing,
%of Eqs.~\eqref{eq:system-bath-collective} and~\eqref{eq:system-bath-independent}, 
starting from the first excited state of the maximal spin sector.
%, for $ \nspin = \text{\numlist{3;4;5;6;7;8}} $. 
The results are shown in Fig.~\ref{fig:withpausing}, for a pause of duration $ \lpause = \SI{100}{\nano\second} $ inserted at the inversion point. The collective dephasing model continues to exhibit higher success probabilities than the independent dephasing model, as in the case discussed in the previous section, but the results of the two models coincide when $ \sinv < \sgap $. 
%Interestingly, with pausing the maximum success probabilities of the independent dephasing model can be restored to be as large as those of the collective dephasing model. 
Thus, relaxation to the ground state during the pause improves performance for both dephasing models. 
%The dependence of the maximum success probabilities on the number of qubits of both models with pausing is shown in Table~\ref{tab:numericaltable}. From the Table we also note 
Note that, as $ \nspin $ increases, the maximum success probability of the collective dephasing model is achieved at $ \sinv > \sgap $, while it is achieved at $ \sinv < \sgap $ in the independent dephasing model. This is in agreement with the $ \nspin = 20 $ result shown in Fig.~\ref{fig:dissipative-tf-100}.

	
%\begin{table*}[tb]
%	\footnotesize
%	\centering
%	\caption{Maximum success probability and gap size as a function of the number of qubits ($n$). The parentheses indicate at which $s_{\text{inv}}$ the maximum success probability is achieved.}
%	\begin{tabular}{c c c c c c c c}
%		\toprule
%		\multicolumn{2}{c}{$n$}  & $3$      &$4$ &$5$ &$6$ &$7$&$8$\\ \midrule
%		\multirow{2}[4]{*}{\specialcellc{No pausing: \\ Maximum success probability }}  & Individual bath&\makecell{$0.9335$ \\ $(s_{\text{inv}}=0.040)$} & \makecell{$0.9156$ \\ $(s_{\text{inv}}=0.055)$}  & \makecell{$0.8978$ \\ $(s_{\text{inv}}=0.065)$} & \makecell{$0.8749$ \\ $(s_{\text{inv}}=0.075)$} & \makecell{$0.8487$ \\ $(s_{\text{inv}}=0.085)$} & \makecell{$0.8198$ \\ $(s_{\text{inv}}=0.105)$}\\ \cmidrule{2-8}
%			& Collective bath &  \makecell{$0.9984$ \\ $(s_{\text{inv}}=0.065)$}& \makecell{$0.9976$ \\ $(s_{\text{inv}}=0.095)$} & \makecell{$0.9959$ \\ $(s=0.120)$}& \makecell{$0.9932$ \\ $(s_{\text{inv}}=0.145)$} & \makecell{$0.9882$ \\ $(s_{\text{inv}}=0.160)$} & \makecell{$0.9840$ \\ $(s_{\text{inv}}=0.195)$}\\ \midrule  
%		\multirow{2}[4]{*}{\specialcellc{With pausing: \\ Maximum success probability }}  & Individual bath&\makecell{$0.9994$ \\ $(s_{\text{inv}}=0.085)$}  & \makecell{$0.9990$ \\ $(s_{\text{inv}}=0.100)$} & \makecell{$0.9983$ \\ $(s_{\text{inv}}=0.120)$} & \makecell{$0.9973$ \\ $(s_{\text{inv}}=0.150)$} & \makecell{$0.9941$ \\ $(s_{\text{inv}}=0.180)$} & \makecell{$0.9917$ \\ $(s_{\text{inv}}=0.190)$}\\\cmidrule{2-8}
%			&Collective bath&\makecell{$0.9991$ \\ $(s_{\text{inv}}=0.085)$}  & \makecell{$0.9979$ \\ $(s_{\text{inv}}=0.100)$} & \makecell{$0.9960$ \\ $(s_{\text{inv}}=0.120)$} & \makecell{$0.9963$ \\ $(s_{\text{inv}}=0.370)$} & \makecell{$0.9966$ \\ $(s_{\text{inv}}=0.370)$} & \makecell{$0.9972$ \\ $(s_{\text{inv}}=0.370)$}\\ \midrule
%		\multirow{2}[4]{*}{}  & $\Delta$ (GHz) & $7.7551$  & $6.9451$ & $6.3062$ & $5.7842$ & $5.3451$ & $4.9672$\\ \cmidrule{2-8}
%			& $s_{\Delta}$  & $0.3302$   & $0.3210$    & $0.3163$ & $0.3137$ &$0.3120$ &$0.3109$\\  \bottomrule
%	\end{tabular}
%	\label{tab:numericaltable}
%\end{table*}

	
%\vspace{1.5cm}
\section{Conclusions}
\label{sec:conclusions}

Earlier work revealed an intriguing tension between experimental results demonstrating a substantial enhancement in success probabilities for random spin glass instances under reverse annealing compared to standard (forward) annealing~\cite{marshall}, and theoretical results finding that reverse annealing adversely affects performance for the $p$-spin model, in a closed system setting~\cite{nishimori:reverse-pspin-2}. In this work we resolved this tension by performing a numerical study of reverse annealing of the $p$-spin model in an open system setting, where we included dephasing in the instantaneous energy eigenbasis. We found that the associated thermal relaxation results in significant increase in the success probabilities, as long as the inversion point of the reverse annealing protocol is chosen to be close to the avoided crossing point, or before it. Pausing at the inversion point further improves performance. 

Since closed-system, unitary dynamics predicts that reverse annealing fails, yet its open system analogue succeeds, it follows that thermal relaxation is the mechanism responsible for the success. Reverse annealing is thus an example of a family of protocols that strictly benefit from thermal effects~\cite{verstraete2009quantum,Venuti:2017aa}.
It may be worth noting that quantum effects are likely to play an important role in thermal relaxation because the success probability is very small for $s_{\rm inv}$ close to $1$, i.e. when the Hamiltonian stays classical during the anneal, even with a pause.
Whether this can lead to any quantum speedups is an interesting problem worthy of future investigations.


\chapter{Experimental iterative reverse annealing}
\label{chap: IRA_exp}
Reverse annealing is a variant of quantum annealing, in which the system is prepared in a trial solution state, annealed reversely to an inversion point, and then annealed forwardly. It may also be iterated with the last output state as the input of the next iteration.
We perform experiments of reverse annealing on the D-Wave 2000Q device, with a focus on the $p$-spin problem with $p=2$. We examine the dependence of the performance on parameters such as problem size, anneal time and inversion points, as well as on D-Wave’s functionalities like pausing, and the number of iterations. The performance is evaluated in terms of total and partial success probabilities, the latter being the probabilities for two degenerate ground states. To explain the experimental results, we perform open-system simulations with decoherence in the instantaneous energy eigenbasis. The experimental total success probabilities well match the simulation data. We find a difference between independent and collective system-bath coupling models, which is explained by non-conservation of spin symmetry of classical inputs. Simulations show iterated reverse annealing fails in a closed system, suggesting the importance of thermal relaxation in the convergence to the correct solution. We also perform semi-classical simulations of spin-vector Monte Carlo to supplement  our understanding of the experimental data.

We next perform closed and open-systems simulations and compare the results with the data presented in the previous section. We choose relatively small system sizes $N=4$ and $8$ to facilitate numerical computations and also because experimental data do not show strong size dependence as discussed in the previous section.
For the purpose of clarify, we focus on reverse annealing without pausing (i.e. $t_p=0$) in this section. We expect in general applying pausing will lead to an overall enhancement to the results of open-system simulation.

\subsection{Closed system}
The time evolution of reverse annealing in a closed system is as follows.

In a closed system, the state after a single iteration (cycle) is
\begin{equation}
\ket{\psi(2t_{\text{inv}})} = U(2t_{\text{inv}},0)\ket{\psi(0)}\,,
\end{equation}
where $\ket{\psi(0)}$ is the initial state and
\begin{equation}
    U(2t_{\text{inv}}, 0) = {\cal T}\exp\left[-i\int_0^{2t_{\text{inv}}}H(t')dt'\right]
\end{equation}
is the unitary time-evolution operator and ${\cal T}$ denotes the forward time ordering. At the end of $r$ cycles, the final state $\ket{\psi(2rt_{\text{inv}})}$ can be expressed as:
\begin{equation}
\ket{\psi(2rt_{\text{inv}})} = U(2rt_{\text{inv}}, 0)\ket{\psi(0)}\,,
\end{equation}
with
\begin{equation}
    U(2rt_{\text{inv}}, 0) = \prod_{i=0}^{r-1}U(2(i+1)t_{\text{inv}}, 2it_{\text{inv}}) \,.
\end{equation}
Here, the final state of the $r$th cycle is the initial state of the next cycle. This condition is shared by the experiments in the previous section. The solution states are doubly degenerate, and the total success probability at the end of $r$ cycles is
\begin{equation}
|\langle\psi(2rt_{\text{inv}})|\uparrow\rangle^{\otimes N}|^2 + |\langle\psi(2rt_{\text{inv}})|\downarrow\rangle^{\otimes N}|^2 \,.
\end{equation}

For more efficient numerical simulations without loss of accuracy, we rotate the state vector into the instantaneous energy eigenbasis representation at each time step. 
\subsubsection{Dependence on the system size and computation time}

We initialize the state to have a single spin down, i.e. $\ket{0001}$ ($\ket{0} \equiv \ket{\uparrow}$, $\ket{1} \equiv \ket{\downarrow}~(m_0=0.5)$) for $N=4$ and $\ket{0000001}~(m_0=6/8=0.75)$ for $N=8$, respectively.
(But note that they are not the eigenstates of $H(1)$, due to a small residue transverse field at $s=1$.).
Note that the computational basis states such as $\ket{0001}$ and $\ket{0000001}$ are not simultaneous eigenstates of $\bold{S}^2 = \sum_{\alpha\in\{x,y,z\}}(S^{\alpha})^2$ and $S^z=\frac{1}{2}\sum_{i=1}^{N}\sigma_i^z$ (or $H_p$). Therefore the computational basis states do not lie in the subspace of any value of $S$, where $S$ represents the total spin quantum number of $N$ qubits.
In the situation where the initial state $\ket{\psi(0)}$ of reverse annealing is a computational basis state, there is also a natural upper bound on the success probability achievable in closed system reverse annealing because a computational state has only part of the basis state of the maximum spin subspace of $S_{\text{max}}=N/2$ (see Appendix.~\ref{append:successbound}). This upper bound explains why the following closed system results generally have low success probabilities.

We plot in Fig.~\ref{fig:close0001_r1} the simulation results for the total success probability  with various $\tau$. We see that the success probability after a single cycle is non-negligible only when $\tau$ is small enough ($\tau < 1$ [ns]), in which case diabatic transitions to states with lower energies take place.

\begin{figure}[h!]
\subfigure[]{\includegraphics[width=0.49\columnwidth]{ra2/4qubitsunitary_0001_new_largefont.pdf}\label{fig:4qubitsunitary}}
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/8qubitsunitary_00000001_new_largefont.pdf}\label{fig:8qubitsunitary}}
\caption{Total success probability for closed system with $r=1$ (single cycle) and a single-spin down as the initial state. (a) $N=4$, (b) $N=8$.}
\label{fig:close0001_r1}
\end{figure}


\subsubsection{Dependence on the initial state and number of iterations}
\label{sec:closed2}
We next choose the initial state $\ket{\psi(0)}$ with two spins down $\ket{0011}~(m_0=0)$ for $N=4$ and  $\ket{00000011}~(m_0=0.5)$ for $N=8$, respectively, the second excited states of $H_{0}$ of respective system sizes.

\begin{figure}[h!]
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/4qubitsunitary_0011_new_largefont.pdf}\label{fig:4qubitsunitary2}}
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/8qubitsunitary_00000011_new_largefont.pdf}\label{fig:8qubitsunitary2}}
\caption{Total success probability for $r=1$ with two spin down as the initial state. (a) $N=4$, (b) $N=8$.}
\label{fig:close0011_r1}
\end{figure}
Figure~\ref{fig:close0011_r1} shows that, for $N=4$ and $r=1$, the success probability is a little lower than the case when the initial state has a single spin down, Fig.~\ref{fig:close0001_r1}. Nevertheless, for very diabatic reverse annealing (very small $\tau$), the maximum success probability is around the same. For $N=8$, the success probability is negligible, no matter how diabatic the process is.

We plot in Fig.~\ref{fig:close0011_r2} the results for $r=2$ cycles, where we see that the success probability decreases compared to the $r=1$ case. This is consistent with the conclusion of Ref.~\cite{Yamashiro2019}.
\begin{figure}[h!]
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/4qubitsunitary_0011_r2_new_largefont.pdf}\label{fig:4qubitsunitary3}}
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/8qubitsunitary_00000011_r2_new_largefont.pdf}\label{fig:8qubitsunitary3}}
\caption{Total success probability for $r=2$ with two spin down as the initial state. (a) $N=4$, (b) $N=8$.}
\label{fig:close0011_r2}
\end{figure}

We may therefore safely conclude that the closed-system picture is far from the experimental reality in the D-Wave device.

\subsection{Open system}
For an open system, the state after the first cycle is
\begin{equation}
\rho(2t_{\text{inv}}) = V(2t_{\text{inv}},0)\rho(0) \,,
\end{equation}
where 
\begin{equation}
    V(2t_{\text{inv}},0) = {\cal T}\exp\left[\int_0^{2t_{\text{inv}}}\mathcal{L}(t')dt'\right] \,.
\label{eq:vpropagator}    
\end{equation}
$\mathcal{L}(t)$ is the time-dependent Liouville superoperator. We use the adiabatic master equation~\cite{Albash2012}, where $\mathcal{L}(t)$  at time $t$ satisfies
\begin{align}
	\frac{d\rho(t)}{dt} 
	&= \mathcal{L}(t)\rho(t)\\
	&= i \bigl[\rho(t), H(t) + H_\text{LS}(t)\bigr] + \mathcal{D}\bigl[\rho(t)\bigr] \,.
\end{align} 
Here, $ H_\text{LS}(t) $ is the Lamb shift term and $ \mathcal{D} $ is the dissipator superoperator. Again, the time dependence of the integrand in Eq.~(\ref{eq:vpropagator}) depends on $s(t)$.

In the weak coupling limit, the dissipator superoperator $ \mathcal{D} $ can be expressed in a diagonal form with Lindblad operators $L_{i,\omega}(t)$:

\begin{eqnarray}
\label{eq:dissdiag}
{\mathcal{D}}_{}  [\rho(t)]  & = &\sum_{i}\sum_{\omega}\gamma_i(\omega)\left(
L_{i,\omega}(t) \rho(t) L^\dagger_{i,\omega}(t)\phantom{\frac{1}{2}} \right. \notag \\
&& \hspace{-0.5cm} \left. \qquad\qquad - \frac{1}{2} \left\{ L_{i,\omega}^{\dagger}(t) L_{i,\omega}(t) , \rho(t) \right\} \right) \,,
\end{eqnarray}
where the summation runs over the Bohr frequency $\omega$ and qubit index $i$. 

At the end of $r$ cyles, the final state $\rho(2rt_{\text{inv}})$ is expressed as:
\begin{equation}
\rho(2rt_{\text{inv}}) = V(2rt_{\text{inv}}, 0)\rho(0)\,,
\end{equation}
with
\begin{equation}
    V(2rt_{\text{inv}}, 0) = \prod_{i=0}^{r-1}V(2(i+1)t_{\text{inv}}, 2it_{\text{inv}}) \,.
\end{equation}

To elaborate our methods further, we first assume that the qubit system is coupled to independent, identical bosonic baths, with the bath and interaction Hamiltonians being 
%
\begin{subequations}
\begin{align}
\label{eq:SBm}
H_B &= \sum_{i=1}^N \sum_{k=1}^\infty \omega_k b_{k,i}^\dagger b_{k,i} \ ,  \\
H_{SB}^{\text{ind}} &= g \sum_{i=1}^N
\sigma_i^z \otimes \sum_k \left(b_{k,i}^\dagger + b_{k,i} \right) \ ,
\end{align}
\end{subequations}
where $b_{k,i}^\dagger$ and $b_{k,i}$ are, respectively, the raising and lowering operators for the $k$th oscillator mode with natural frequency $\omega_k$.  The bath correlation functions appearing in Eq.~\eqref{eq:dissdiag} are given by
%
\begin{equation}
\gamma_{i}(\omega) = 2\pi \eta g^2\frac{\omega e^{-|\omega|/\omega_c}}{1-e^{-\beta\omega}}  \ ,
\end{equation}
%
arising from an Ohmic spectral density, and satisfy the Kubo-Martin Schwinger condition~\cite{kubo1957statistical, martin1959theory} ($\gamma_{i}(- \omega) = e^{-\beta\omega} \gamma_{i}(\omega)$, $\beta = 1/T$ being the inverse temperature).  We use $\eta g^2 = 1e^{-3}$, the cutoff frequency $\omega_c = 1$ [THz], and operating temperature of D-Wave chips $T= 12.1 \text{ [mK]} = 1.57$ [GHz]. With this assumption, we have the Lindblad operators as
\begin{equation}
   L_{i,\omega}(t) = \sum_{\epsilon_b-\epsilon_a = \omega} | \varepsilon_a(t) \rangle \langle \varepsilon_a(t) | \sigma^z_{i} | \varepsilon_b(t) \rangle \langle \varepsilon_b(t) | \,,
\end{equation}
corresponding to dephasing in the instantaneous eigenbasis $|\varepsilon_b(t) \rangle$ of $H(t)$. For more efficient numerical simulations we rotate the density matrix and Lindblad operators into the instantaneous energy eigenbasis at each time step, to keep the matrices sparse and without loss of accuracy. For system size $N = 8$, we truncate the system size to the lowest $n=18$ levels (out of $256$ levels).


We also consider the collective system-bath coupling model, where all the qubits are coupled to a collective bath with the same coupling strength $g$, which preserves the spin symmetry. In this case, the interaction Hamiltonian becomes
\begin{align}
    H_{SB}^{\text{col}} = g S^z \otimes B,
\end{align}
where
\begin{align}
    S^z = \sum_{i} \sigma_i^z, B = \sum_k \left(b_{k}^\dagger + b_{k} \right).
\end{align}
With this assumption, we can group together the Lindblad operators corresponding to different qubit $i$ into a single one:
\begin{equation}
   L_{\omega}(t) = \sum_{\epsilon_b-\epsilon_a = \omega} | \varepsilon_a(t) \rangle \langle \varepsilon_a(t) | S^z | \varepsilon_b(t) \rangle \langle \varepsilon_b(t) | \,.
\end{equation}
The resulting number of Lindblad operators is a factor of $N$ smaller than that of the independent system-bath coupling model.

The total success probability at the end of the $r$ cycles is
\begin{equation}
^{\otimes N}\langle\,\uparrow|\rho(2rt_{\text{inv}})|\uparrow\,\rangle^{\otimes N} + ^{\otimes N}\langle\,\downarrow|\rho(2rt_{\text{inv}})|\downarrow\,\rangle^{\otimes N} \,.
\end{equation}

Any relaxation during reverse anneal dynamics to the global instantaneous ground state or the instantaneous first excited state of $H(t)$ (Eq.~\ref{eq:H}, see spectrum at Appendix.~\ref{append:spectrum}) is beneficial. It is because they converge to the degenerate ground states $\{|\uparrow\,\rangle^{\otimes N},|\downarrow\,\rangle^{\otimes N}\}$ of $H_0$ at the end of the reverse anneal. 

\subsubsection{Dependence on computation time}
Figure~\ref{fig:4open_0001_r1} shows the simulation results for success probability as a function of $s_{\rm inv}$ with $N=4$, various $\tau$, and the initial state of $\ket{0001}~(m_0=0.5)$, using the independent and collective system-bath coupling models.
\begin{figure}[h!]
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/4qubitopen_0001_new_largefont.pdf}\label{fig:4qubitopena}}
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/4qubitopen_0001_collective_new_largefont.pdf}\label{fig:4qubitopenb}}
\caption{Success probability as a function of $s_{\rm inv}$ with (a) independent and (b) collective system-bath couplings. Initial state: $\ket{0001}~(m_0=0.5)$ and $r=1$, a single cycle.}
\label{fig:4open_0001_r1}
\end{figure}
%
For the initial state of $\ket{0001}$ and $r=1$, the independent system-bath model leads to a maximum success probability of $1$ for large $\tau$ and small $s_{\rm inv}$. However, the collective system-bath model leads to a maximum success probability of $1/4$. The reason is the same as in closed system simulations. For the computational initial state of $\ket{0001}$, only $1/4$ of its population is in the subspace of maximum quantum spin number. %
However, the global (instantaneous) ground state and the first excited state of the annealing Hamiltonian $H(s)$ both belong to the maximum spin subspace. Since the collective system-bath coupling model preserves the spin symmetry and the dynamics is restricted to each subspace, at most $1/4$ of the initial population can be relaxed to the instantaneous ground state and the first excited state, and reach the correct solutions at the end of the reverse anneal. For more information, we refer the reader to Appendix.~\ref{append:successbound}.

Comparing the simulation results in Fig.~\ref{fig:4open_0001_r1} and the experimental results in Sec.~\ref{sec:exp}, we see some common features. For example, the larger $\tau$ is, the higher the success probability is. For larger $\tau$, the maximum success probability can be achieved with a larger inversion point $s_{\text{inv}}$. 
Note that the experimental results in Sec.~\ref{sec:exp} have the maximum success probability as high as $1$, while closed system simulation and open-system simulations with the collective system-bath model have success probabilities upper bounded by some constants as already discussed. The high total success probability observed in experiments is evidence that the dynamics in the D-Wave device do not preserve the spin symmetry as naturally expected. Only open-system simulations with independent system-bath model can explain the experimental results.


\subsubsection{Dependence on the initial condition and the number of cycles}
% \begin{figure}[h!]
% \subfigure[]{\includegraphics[width=0.4939\columnwidth]{4qubitopen_0011_new.pdf}\label{fig:4qubitsunitarya}}
% \subfigure[]{\includegraphics[width=0.4939\columnwidth]{4qubitopen_0011_collecive_new.pdf}\label{fig:8qubitsunitary}}
% \caption{Open-system reverse annealing results, with different $\tau$. (a) Independent bath, (b) Collective bath. Initial state: $\ket{0011}$, $r=1$.}
% \label{fig:4open_0011_r1}
% \end{figure}
\begin{figure}[h!]
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/4qubitopen_0011_new_largefont.pdf}}
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/4qubitopen_0011_r2_new_largefont.pdf}}
\caption{Success probability with different $\tau$. Initial state: $\ket{0011}~(m_0=0)$. (a) $r=1$, (b) $r=2$.}
\label{fig:4open_0011_r1}
\end{figure}

For the initial state of $\ket{0011}~(m_0=0)$ and $r=1$, the independent system-bath model still gives a maximum success probability of $1$ as seen in Fig.~\ref{fig:4open_0011_r1}. Note that the collective system-bath model (not shown) has a maximum success probability of $1/6$, since the initial state has $1/{{4}\choose{2}} = 1/6$ of its population in the maximum spin subspace.

The dependence of success probability on $s_{\text{inv}}$ is very similar to that of initial state $\ket{0001}$. The only exception is for $\tau = 1$ [ns], where reverse annealing is too fast for the system to experience the open-system effect. Compared to the case of closed systems, the results depend much less on the initial condition. 

In Fig.~\ref{fig:4open_0011_r1}, we look further into the dependence on the number of cycles $r$, using the independent system-bath model. For $r=2$, we see that the results are similar to those of a single cycle. However, we do see a slight improvement, which was not observed in the closed system discussed in Sec.~\ref{sec:closed2}.

\subsubsection{Dependence on the type of coupling and the size}
\begin{figure}[h!]
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/8qubitsopen_1us_largefont.pdf}\label{fig:8open}}
\subfigure[]{\includegraphics[width=0.4939\columnwidth]{ra2/4qubitsvs8qubitsopen_1us_largefont.pdf}\label{fig:4vs8open}}
\caption{Success probability as a function of $s_{\rm inv}$. (a) Two types of system-bath coupling for $N=8$. (b) Two system sizes $N=4$ and $8$. The initial state has a single spin flipped. $\tau$ is $1 [\mu$s].}
\end{figure}

Fig.~\ref{fig:8open} shows the success probability for two system-bath coupling models with $N=8$. The initial state is  $\ket{00000001}~(m_0=6/8=0.75)$. In this case, the maximum success probability of collective system-bath couplings is  $1/8$, which is the population of the initial state in the maximal spin subspace. This observation is different from~\cite{Passarelli2019}, where the initial state (a superposition of computational basis state) lies completely inside the maximal spin subspace, and thus in~\cite{Passarelli2019} even collective system-bath couplings model can also produce the maximum success probability of $1$. 

In Fig.~\ref{fig:4vs8open}, we show the dependence of the success probability on the system size $N$. The initial state has a single spin down ($\ket{0001}~(m_0=1/2)$ for $N=4$ and $\ket{0000001}~(m_0=6/8=0.75)$ for $N=8$). We observe that results do not depend much on the system size, with the total success probabilities only slightly larger for $N=4$. This is in line with the experimental results ($N=4$ and 8 in Fig.~\ref{fig:RA_20_size}(b)).


\subsubsection{Partial success probability}
While the total success probabilities of open-system simulations with independent system-bath coupling model are generally consistent with those in experiments, open-system simulations always produce symmetric partial success probabilities as shown in Fig.~\ref{fig:8openep}. However, this is not the case in experiments (e.g. Fig.~\ref{fig:RA_20_diff_tau}). 
The reason is that the adiabatic master equation assumes decoherence (or jumping) between the instantaneous eigenstates of $H(s)$. Any relaxation during reverse anneal (at any $s$) to either the global instantaneous ground state $\ket{\epsilon_0(s)}$ or the instantaneous first excited state $\ket{\epsilon_1(s)}$ of $H(s)$ is beneficial, since they converge to the degenerate solution (ground) states of $H_0$ at $s=1$. However, $\ket{\epsilon_0(s)}$ and $\ket{\epsilon_1(s)}$ at $s=1$ expressed in terms of the solution states are: $\ket{\epsilon_0(s=1)} = \frac{\ket{\uparrow}^{\otimes N} + \ket{\downarrow}^{\otimes N}}{\sqrt{2}}$ and $\ket{\epsilon_1(s=1)} = \frac{\ket{\uparrow}^{\otimes N} - 
\ket{\downarrow}^{\otimes N}}{\sqrt{2}}$, which have an evenly-shared populations of all-up and all-down states. Similar observations are also found in~\cite{albash2015consistency}, and the semi-classical simulations such as spin-vector Monte Carlo (SVMC)~\cite{shin2014quantum}, which describes classical thermal hopping mechanisms, are expected to produce different results as we see in the next section.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{ra2/8qubitsegplot_open_individual_largefont.pdf}
    \caption{Success probability with partial probabilities in the inset for $N=8$  with independent system-bath coupling. The initial state is $\ket{00000001}~(m_0=6/8=0.75)$.}
    \label{fig:8openep}
\end{figure}

\section{Semi-classical simulations}\label{sec:classical}
In an effort to understand the asymmetric partial success probability in experiments, we performed semi-classical simulations of spin-vector Monte Carlo (SVMC)~\cite{shin2014quantum} and a new variant of SVMC-TF~\cite{Albash2020ComparingRM}. For the $p$-spin problem, we replace the Hamiltonian of Eq.~(\ref{eq:H}) by a classical Hamiltonian:
\begin{equation}
\mathcal{H}(s) = -\frac{A(s)}{2} \left(\sum_{i}^{N} \sin \theta_i\right) - \frac{B(s) N}{2}\left(\frac{1}{N}\sum_{i}^{N} \cos \theta_i\right)^{p}\,.
\label{eq:Hising}
\end{equation}
Each qubit $i$ is replaced by a classical O($2$) spin $\vec{M}_i=(\sin\theta_i,0,\cos\theta_i)$, $\theta_i \in [0, \pi]$. For the purpose of reverse annealing, we again need to specify the $t$ dependence of $s(t)$. The concept of time $t$ is here replaced by the number of Monte Carlo sweeps. Total annealing time is $2\tau(1-s_{\text{inv}})$. We will replace $\tau$ by a specified number of total sweeps.

To simulate the effect of thermal hopping through this semi-classical landscape with the inverse temperature $\beta$, we perform at each time step a spin update according to the Metropolis rule. In SVMC, a random angle $\theta_i^{'} \in [0, \pi]$ is picked for each spin $i$. Updates of the spin angles $\theta_i$ to $\theta_i^{'}$ are accepted according to standard Metropolis rule associated with the change in energy ($\Delta E$) of the classical Hamiltonian. In SVMC-TF, the random angle $\theta_i^{'} =\theta_i + \epsilon_i(s)$ is picked in a restricted range
\begin{align}
    \epsilon_i(s) \in \left[-\min \left(1,\frac{A(s)}{B(s)}\right) \pi, \min \left(1,\frac{A(s)}{B(s)}\right) \pi\right]. 
\end{align}
The goal of SVMC-TF is to restrict the angle update for $A(S) < B(s)$, and imitate the freeze-out effect observed in D-Wave device \cite{Amin2015}. The full SVMC and SVMC-TF algorithms for reverse annealing are summarized in Appendix.~\ref{append:svmc}.


We report the SVMC and SVMC-TF results for the case of $N=4$ and $8$ to be compared with the data in the previous sections. 
% The classical Hamiltonian is:
% \begin{equation}
% \mathcal{H}(s) = -\frac{A(s)}{2} \left(\sum_{i=1}^{4}\sin \theta_i\right) - \frac{B(s)}{8}\left(\sum_{i=1}^{4} \cos \theta_i\right)^{2}\,.
% \label{eq:Hising_4}
% \end{equation}
For $p$-spin problem, the corresponding energy change $\Delta E$ cannot be expressed in a simple form as in case of the Ising problem Hamiltonian~\cite{shin2014quantum}. The expression of $\Delta E$ is given in Appendix.~\ref{append:svmc}.
% For example, the update of qubit $2$ to a new angle results in a change in energy, denoted by $\Delta E_2$, as:
%{\small
%\begin{align*}
%\phantom{=}&\Delta E_2 \\
%= 
%&\left(-\frac{A(s)}{2} \left(\sum_{\substack{i=1\\i \ne 2}}^{4}\sin \theta_i + \sin \theta^{'}_2\right) - \frac{B(s)}{8}\left(\sum_{\substack{i=1\\i \ne 2}}^{4} \cos \theta_i + \cos \theta^{'}_2\right)^{2} \right) \\
%- &\left(-\frac{A(s)}{2} \left(\sum_{i=1}^{4}\sin \theta_i\right) - \frac{B(s)}{8}\left(\sum_{i=1}^{4} \cos \theta_i\right)^{2} \right) \,.
%\end{align*}
%}

\subsection*{Total success probability}
We choose the initial condition with a single spin down. In terms of angles, the initial angles are $\{0,0,0,\pi\}$. We again use the temperature $T=12.1$ [mK]. The classical analogue of the annealing time is chosen to be $\tau = 10^3$ and $10^4$ sweeps. The total number of sweeps with the inversion point $s_{\text{inv}}$ is then $2\tau(1-s_{\text{inv}})$. 

In Fig.~\ref{fig:comparealltotal} we report the simulation results of total success probability using SVMC and SVMC-TF, with $\tau = 10^3$ and $10^4$, respectively. The number of samples is $10^4$.
\begin{figure}[h!]
% \subfigure[]{\includegraphics[width = 0.4939\columnwidth]{svmcplot_100sweeps.pdf}\label{fig:4qubitsunitarya}}
\subfigure[]{\includegraphics[width = 0.4939\columnwidth]{ra2/svmcplot_1000sweeps_largefont.pdf}}
\subfigure[]{\includegraphics[width = 0.4939\columnwidth]{ra2/svmcplot_10000sweeps_largefont.pdf}}
\caption{Total success probability for SVMC and SVMC-TF. (a) $\tau = 10^3$ sweeps, (b) $\tau = 10^4$ sweeps. Error bars are 2$\sigma$ over $10^4$ samples.}
\label{fig:comparealltotal}
\end{figure}
SVMC gives high total success probabilities even with large inversion points $s_{\text{inv}}$. A large inversion point $s_{\text{inv}}$ means that during the whole reverse annealing process the ratio of $A(s)/B(s)$ is small. In the D-Wave device, it is expected that for small $A(s)/B(s)$ the dynamics freezes and it is difficult to reach the correct solutions. With the number of sweeps increased from $\tau=10^3$ to $10^4$, we observe that even for very large inversion points $s_{\text{inv}}$ the total success probability of SVMC can be as high as $1$. This is because the angle updates in SVMC are completely random and thus with a sufficient number of sweeps, it is possible for the state to flip to the correct solution.

However, in SVMC-TF, the range of angle update is restricted for $A(s)/B(s) < 1$. The restricted angle updates (freeze-out effect) prevent the state to flip to the correct solutions. Therefore the total success probability for large inversion points $s_{\text{inv}}$ is basically zero in SVMC-TF, regardless of the number of sweeps. This is also what we observe in the experimental data.

\subsection*{Partial success probability}
We compare the partial success probability obtained from SVMC and SVMC-TF in Fig.~\ref{fig:compareallpartial} for $N=4$ and $\tau = 10^3$.  Comparing the experimental data in Fig.~\ref{fig:RA_20_size} and Fig.~\ref{fig:compareallpartial}, we see that the data of SVMC-TF matches satisfactorily with the experimental result. SVMC-TF gives the correct trend for the uneven up and down partial success probabilities. Also, for a limited region of $s_{\text{inv}}$, the partial success probabilities of the all up states can be as high as $1$.
Classical SVMC-TF simulation also explains the D-Wave data of random systems in \cite{Albash2020ComparingRM}.
% This tendency that the classical SVMC-TF simulation also explains the D-Wave data has been observed in random systems \cite{Albash2020ComparingRM}.
% This may suggest that classical thermal effect is present in the D-Wave device \textcolor{red}{[HN: Really?]}.

The result for a larger system $N=8$ is plotted in Fig.~\ref{fig:8partial}. We observe a slight deviation from the experimental data in Fig.~\ref{fig:RA_20_size}(a) for $s_{\text{inv}} \lesssim 0.3$, where there exists a small but clear difference in the probabilities of all-up and all-down states whereas the SVMC-TF data do not show such tendency. %It is unclear where this difference comes from.  An additional discussion is provided in Sec. \ref{section:Conc}. 
Essentially similar data of larger system sizes of $N=16$ and $32$ are shown in Appendix.~\ref{append:svmctflarge}. These results may imply limitations of a semi-classical description by SVMC and SVMC-TF for the mechanism of relaxation in the real device.
\begin{figure}[h!]
% \subfigure[]{\includegraphics[width = 0.4939\columnwidth]{svmcplot_100sweeps_ge.pdf}\label{fig:4qubitsunitarya}}
\subfigure[]{\includegraphics[width = 0.4939\columnwidth]{ra2/svmcplot_1000sweeps_ge_largefont.pdf}}
\subfigure[]{\includegraphics[width = 0.4939\columnwidth]{ra2/svmctfplot_1000sweeps_n4_ge_largefont.pdf}}
\caption{Partial success probability by (a) SVMC and (b) SVMC-TF. $\tau = 10^3$ sweeps. Error bars are 2$\sigma$ over $10^4$ samples.}
\label{fig:compareallpartial}
\end{figure}

% \begin{figure}[h!]
% % \subfigure[]{\includegraphics[width = 0.4939\columnwidth]{svmctfplot_100sweeps_ge.pdf}\label{fig:4qubitsunitarya}}
% \subfigure[]{\includegraphics[width = 0.4939\columnwidth]{svmctfplot_1000sweeps_ge.pdf}\label{fig:8qubitsunitary}}
% \caption{Partial success probabilities. SVMC-TF. $N=8$.}
% \label{fig:compareallsweeps}
% \end{figure}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{ra2/svmctfplot_1000sweeps_n8_ge_largefont.pdf}
    \caption{Partial success probabilities. SVMC-TF. $N=8$. $\tau = 10^3$ sweeps. Error bars are 2$\sigma$ over $10^4$ samples.}
    \label{fig:8partial}
\end{figure}


\chapter{Adiabatic reverse annealing}
\label{chap:ara}
The annealing Hamiltonian for adiabatic reverse annealing (ARA) is~\cite{yamashiro2019dynamics, crosson2020prospects}: 
\begin{equation}
\label{eq:H}
  H(s, \lambda) = sH_{0} + (1-s)(1- \lambda)H_{\text{init}} + \Gamma (1-s)\lambda V_{\text{TF}} \,.
\end{equation}

The time-dependent parameters $s(t)$ and $\lambda(t)$ both
change from $0$ to $1$ as time $t$ proceeds from $0$ to $\tau$, where
$\tau$ is the total anneal time. We focus on the case of a linear function $s(t) = t/\tau$.

The notation of Eq.~\ref{eq:H} is as follows. $H_{0} = -N\left(\frac{1}{N}\sum_{i=1}^{N} \sigma^{z}_i\right)^{p}$ is the target problem Hamiltonian, with $p=3$ and
$N$ the number of qubits. $H_{\text{init}} = -\sum_{i=1}^{N}\epsilon_i \sigma^{z}_i$ is the initial Hamiltonian, $\epsilon_i = \pm 1$. $V_{\text{TF}} = -\sum_{i=1}^{N} \sigma^{x}_i$ is the transverse field Hamiltonian. \\
% $A(s)$ and $B(s)$ depends on the specific machine. The D-Wave 2000Q NASA processor annealing schedules of $A(s)$ and $B(s)$ are shown in Fig.~\ref{fig: DWavenasaschedule}.
We want to perform (adiabatic) reverse annealing with various initial states $\ket{\psi(s=0)} = \ket{\epsilon_1, \epsilon_2, \dots, \epsilon_N}$ (the ground state of $H_{\text{init}}$). 

\subsubsection{$\lambda(t) = s(t)$}
% \subsection{Staying in the maximum spin subspace}
% \begin{align}
%   H(s, \lambda) &= sH_{0} + (1-s)(1- \lambda)H_{\text{init}} + \Gamma (1-s)\lambda V_{\text{TF}} &\\
%     &= sH_{0} + (1-s)(1- s)H_{\text{init}} + \Gamma (1-s)s V_{\text{TF}}  \,.
% \end{align}
We further assume that $\lambda = s$. With this assumption, Eq.~\ref{eq:H} is simplified as:
\begin{equation}
\label{eq:H_simp}
  H(s) = sH_{0} + (1-s)^2 H_{\text{init}} + \Gamma (1-s)s V_{\text{TF}}  \,.
\end{equation}

\subsubsection{$\lambda(t) = 1$}
In this cases, Eq.~\ref{eq:H} is the quantum annealing (QA)  Hamiltonian.
% \subsection{Schedule}
\section{
Preliminary I: Adiabatic reverse annealing (ARA) Hamiltonian spectrum}
In this section, we want to explore how the spectrum changes by tuning certain parameters of Eq.~\ref{eq:H_simp}. This is important in the calculations of diabatic transition rates, excitation and relaxation rates, and thus the understanding of open-system behavior of adiabatic reverse annealing (ARA).
For the particular problem of $N=10$, the solution state of the $p$-spin problem is $\ket{\uparrow}^{\otimes 10}$. Consider the initial state with the number of spin-downs $N_\downarrow = 2$.
% first spin down, i.e. $\epsilon_1=-1$, $\epsilon_i=+1$ for $i \neq 1$. 
We plot the spectrum in Fig.~\ref{fig: ARAspectrum}.

\begin{figure}[h!]
\includegraphics[width=0.6\linewidth]{ra3/pspin_ARA_spectrum_10.pdf}
\caption{The $16$ lowest lying energies of $10$ qubits, with $H_{\text{init}}$ having $N_\downarrow = 2$.
%such that $\epsilon_1=-1$, $\epsilon_i=+1$ for $i \neq 1$.
}
\label{fig: ARAspectrum}
\end{figure}


\subsection{Controlling the parameters: $\Gamma$}
The energy gap between instantaneous eigenenergies $\epsilon_{i}(s)$ and $\epsilon_{j}(s)$ is $\Delta_{ij}(s) = \epsilon_{i}(s) - \epsilon_{j}(s)$. The corresponding minimum energy gap is $\Delta_{ij} = \min_{s} \Delta_{ij}(s)$.

In adiabatic reverse annealing, we are interested in the minimum energy gap between the ground state $\epsilon_{0}(s)$ and the $1$st excited state $\epsilon_{1}(s)$. It is denoted by $\Delta$ ($=\Delta_{\min})$.  
\begin{equation}
    \Delta = \Delta_{10} = \min_{s} \Delta_{10}(s) = \min_{s} \epsilon_{1}(s) - \epsilon_{0}(s) \,.
\end{equation}

Let $N=8$, the solution state of the $p$-spin problem is $\ket{\uparrow\,}^{\otimes 8}$. Consider again the initial state with $N_{\uparrow}=1$. We want to explore how the gap properties change with $\Gamma$ in Eq.~\ref{eq:H_simp}.
We calculate and plot in Fig.~\ref{fig: gammaplot} the value of $\Delta_{10}(s)$, for $N=8$ and $\Gamma = \{1, \cdots, 5\}$. In the inset we plot the dependence of $\Delta$ on $\Gamma$. In general $\Delta$ decreases as $\Gamma$ decreases. Also the shape of the gap is also sharper with smaller $\Gamma$. This allows diabatic transition.


\begin{figure}[h!]
\includegraphics[width=0.6\linewidth]{ra3/gamma_plot.pdf}
\caption{$\Delta(s)$ for $\Gamma = \{1, \cdots, 5\}$. In unit where $h=1$.}
\label{fig: gammaplot}
\end{figure}



\subsection{Controlling the parameters: Initial states $\epsilon_i$ or ($H_{\text{init}}$)}

We want to investigate how the gap properties change with different initial states. In this case we focus on $\Gamma = 1$.
\begin{figure}[h!]
\includegraphics[width=0.6\linewidth]{ra3/pspin_p2_spectrum_4_Hinit.pdf}
\caption{$\Delta(s)$ for different $\epsilon_i$. $\Gamma = 1$. In unit where $h=1$.}
\label{fig: gammaplot}
\end{figure}

From Fig.~\ref{fig: gammaplot}, we see that in general $\Delta$ decreases as the Hamming distance between the initial state and the target state increases.  




\subsection{Controlling the parameters: $N$}
We want to investigate how the minimum gap changes with system size $N$. In this case we focus on the initial state of 
%$\epsilon_1=-1$, $\epsilon_i=+1$ for $i \neq 1$,
$N_{\downarrow}=1$ and $\Gamma = 1$. The value of $\Delta$ for each $N$ is plotted in Fig.~\ref{fig: nplot}.

We also note down the $s$ where the minimum gap is found, i.e.
\begin{equation}
    s_{\mathrm{min}} = \mathrm{argmin} \Delta_{10}(s) \,.
\end{equation}
 This is important for the calculation of relaxation rates for reverse annealing.


\begin{figure}[h!]
\includegraphics[width=0.6\linewidth]{ra3/gaprevealplot.pdf}
\caption{$\Delta$ for $N = \{3, \cdots, 20\}$. In unit where $h=1$. Inset: the value of $s_{\mathrm{min}}$ for each $N$.}
\label{fig: nplot}
\end{figure}


%
\section{Preliminary II: Time evolution}
Let $\ket{\psi(s=0)}$ ($\ket{\psi(t=0)}$) denote the initial state. The anneal time is $\tau$. The final state at the end of the adiabatic reverse annealing (ARA) and the success probability can be expressed as follows.

\subsection{Closed system}
The state after the ARA in a closed system is
\begin{equation}
\ket{\psi(\tau)} = U(\tau,0)\ket{\psi(0)}\,,
\end{equation}
where 
\begin{equation}
    U(\tau, 0) = {\cal T}\exp\left[-i\int_0^{\tau}H(t')dt'\right]
\end{equation}
is the unitary operator and ${\cal T}$ denotes the forward time-ordering. The time-dependence of the Hamiltonian (in the integrand) is given by the $s(t)$ function.


% At the end of $r$ rounds, the final state $\ket{\psi(2rt_{\text{inv}})}$ can be expressed as:
% \begin{equation}
% \ket{\psi(2rt_{\text{inv}})} = U(2rt_{\text{inv}}, 0)\ket{\psi(0)}\,,
% \end{equation}
% with
% \begin{equation}
%     U(2rt_{\text{inv}}, 0) = \prod_{i=0}^{r-1}U(2(i+1)t_{\text{inv}}, 2it_{\text{inv}}) \,.
% \end{equation}



\subsection{Open system: Lindbladian dynamics}
For open system, the state after the ARA is
\begin{equation}
\rho(\tau) = V(\tau,0)\rho(0) \,,
\end{equation}
where 
\begin{equation}
    V(\tau,0) = {\cal T}\exp\left[\int_0^{\tau}\mathcal{L}(t')dt'\right] \,.
\label{eq:vpropagator}    
\end{equation}
$\mathcal{L}(t)$ is the time-dependent Liouville superoperator. For example, in adiabatic master equation, $\mathcal{L}(t)$  at time $t$ takes the form of
\begin{align}
\label{eq:ame}
	\frac{d\rho(t)}{dt} 
	&= \mathcal{L}(t)\rho(t)\\
	&= \iu \bigl[\rho(t), \ham(t) + \ham\ped{LS}(t)\bigr] + \diss\bigl[\rho(t)\bigr] \,.
\end{align} 
$ \ham\ped{LS}(t) $ is a Lamb shift term and $ \diss $ is the dissipator superoperator. Again, the time-dependence of the integrand in Eq.~\ref{eq:vpropagator} depends on the $s(t)$ function.

% At the end of $r$ rounds, the final state $\rho(2rt_{\text{inv}})$ can be expressed as:
% \begin{equation}
% \rho(2rt_{\text{inv}}) = V(2rt_{\text{inv}}, 0)\rho(0)\,,
% \end{equation}
% with
% \begin{equation}
%     V(2rt_{\text{inv}}, 0) = \prod_{i=0}^{r-1}V(2(i+1)t_{\text{inv}}, 2it_{\text{inv}}) \,.
% \end{equation}


\section{Preliminary III: Success metrics and classes or problems}
We use two success metrics for ARA: success probability and time to solution (TTS).
\subsection{Success probability}
The success probability refers to the probability of the final state being the target solution state. For the example of $p$-spin ($p=3$) model, the success probability at the end of ARA can be expressed as:

% \begin{equation}
%     \mathsf{Success\,probability} =
%     \begin{cases}
% |\langle\uparrow\uparrow\uparrow\uparrow|\psi(\tau)\rangle|^2, \text{\quad\quad in a closed system.}\\
% \langle\uparrow\uparrow\uparrow\uparrow|\rho(\tau)|\uparrow\uparrow\uparrow\uparrow\rangle , \text{\quad in an open system.}
% \end{cases}
% \end{equation}
\begin{equation}
    \mathsf{Success\,probability\,\,} p_g(\tau) =
    \begin{cases}
|^{\otimes N}\langle \,\uparrow|\psi(\tau)\rangle|^2, \text{\quad\quad in a closed system.}\\
^{\otimes N}\langle\,\uparrow|\rho(\tau)|\uparrow\,\rangle ^{\otimes N} , \text{\quad in an open system.}
\end{cases}
\end{equation}


\subsection{Time to solution (TTS)}
The time to solution (TTS) is defined as:

\begin{equation}
    \mathsf{TTS}(\tau, p_d) = \tau \frac{\log (1-p_d)}{\log p_e(\tau)} \,.
\end{equation}

$p_d$ is the threshold probability and $p_e(\tau) = 1 - p_g(\tau)$.


\subsection{Classes of problems}
We want to explore four general classes of problems: 1. Adiabatic reverse annealing in an open system 
($\mathsf{ARA_\text{Open}}$), 2. Adiabatic reverse annealing in a closed system ($\mathsf{ARA_\text{Closed}}$), 3. Standard quantum annealing in an open system ($\mathsf{QA_\text{Open}}$), and 4. Standard quantum annealing in a closed system ($\mathsf{QA_\text{Closed}}$). The comparison between $\mathsf{ARA_\text{Closed}}$ and $\mathsf{QA_\text{Closed}}$ has been made in~\cite{yamashiro2019dynamics} and it was shown that $\mathsf{ARA_\text{Closed}}$ can have an advantage over $\mathsf{QA_\text{Closed}}$. Since there are many studies (e.g.~\cite{passarelli2018dissipative} and~\cite{PhysRevA.101.022331}) showing dissipation can give quantum enhancement, we want to investigate further if and under what conditions $\mathsf{ARA_\text{Open}}$ performs better than  $\mathsf{ARA_\text{Closed}}$. On an equal setting, we want also to compare if $\mathsf{ARA_\text{Open}}$ has any computational advantage over $\mathsf{QA_\text{Open}}$, in order to support the use of the formal protocol in a realistic experimental setting. Any advantage/enhancement is defined according to the two success metrics mentioned before.

We already studied how the spectrum depends on $\Gamma$, $H_\text{init}$ and $N$. We want to evaluate how the performance of $\mathsf{ARA}$ and $\mathsf{QA}$ depends on these parameters. For each set of such parameters, we performed simulations in a range of anneal times $\tau$. 

As noted in~\cite{crosson2020prospects}, diabatic transition to higher excited states may be a shortcut of the route to the final solution. Therefore, we include in our studies anneal times $\tau$ shorter than the one set by adiabatic condition~\cite{albash2018adiabatic}. We also explore the cases with small $\Gamma$ and large Hamming distance between the initial state and the target state, which result in a very small and sharp gap and thus diabatic transitions to higher excited states.


\section{Illustrative examples}
We performed numerical experiments for both closed and open system. We use the full Hamiltonian without sector decomposition. The coupling is $\eta = 1e^{-3}$ and the cutoff frequency is  $\omega_c = 1$THz. We use independent bath of dephasing $\hamsysbath\api{ind} = g \sum_{i} \sigma_i^z \otimes B_i$ and collective bath of dephasing $\hamsysbath\api{col} = g \sum_{i} \sigma_i^z \otimes B$ and perform simulations of adiabatic master equation of Eq.~\ref{eq:ame}. We begin by studying three examples in the following subsections (Sec.~\ref{subsectiona}-~\ref{subsectionc}) and illustrate the dynamics of ground state population during the anneal.

%\subsection{Introductory examples}
\subsubsection{Results of $8$-qubit simulation: $\tau = 40$ns. $\Gamma = 1$.}
\label{subsectiona}
 We simulated the closed and open-system evolution with different initial states. In this example we have $N=8$, $\tau = 40$ns. $\Gamma = 1$. The results are plotted in Fig.~\ref{fig:8ame_727}. The solid lines are open-system simulation results while the dotted lines are closed-system simulation results.
\begin{figure}[h!]
\includegraphics[width = 12cm]{ra3/ame_plot_2_727.pdf}\label{fig:8qubitsame}
\caption{Open-system and close-system adiabatic reverse annealing (ARA) simulation results. $\tau = 40$ns. $\Gamma = 1$.}
\label{fig:8ame_727}
\end{figure}
%

\textit{Conclusion: }
From Fig.~\ref{fig:8ame_727}, we see that open-system effect (thermal excitation) is detrimental in this case, i.e. for all initial states specified, the solid lines are below the dotted lines along the evolution and at the end of the evolution.



\subsubsection{Results of $4$-qubit simulation: $\tau = 4$ns. $\Gamma = 1$.}
In this example we have $N=4$, $\tau = 4$ns, and $\Gamma = 1$. The results are plotted in Fig.~\ref{fig:4ame_723}. The solid lines are open-system simulation results while the dotted lines are closed-system simulation results.

\begin{figure}[h!]
\includegraphics[width = 12cm]{ra3/ame_plot_2_723.pdf}\label{fig:8qubitsame}
\caption{Open-system and close-system adiabatic reverse annealing (ARA) simulation results. $\tau = 4$ns. $\Gamma = 1$.}
\label{fig:4ame_723}
\end{figure}



\textit{Conclusion: }
From Fig.~\ref{fig:4ame_723}, we see that open-system effect makes no difference, i.e. for all initial states specified, the solid lines almost overlap with the dotted lines along the evolution and at the end of the evolution. The total anneal time $\tau = 4$ns is too short for environment (bath) to come into effect. The environment causes little difference to the success probabilities. This short anneal time also leads to observable diabatic transition to higher excited states.





\subsubsection{Results of $4$-qubit simulation: $\tau = 400$ns. $\Gamma = 0.3$.}
\label{subsectionc}
In this example we have $N=4$, $\tau = 400$ns. $\Gamma = 0.3$. The results are plotted in Fig.~\ref{fig:4ame_724_2}. 

\begin{figure}[h!]
\includegraphics[width = 12cm]{ra3/ame_plot_2_724_2.pdf}\label{fig:8qubitsame}
\caption{Open-system and close-system adiabatic reverse annealing (ARA) simulation results. $\tau = 400$ns. $\Gamma = 0.3$.}
\label{fig:4ame_724_2}
\end{figure}
\textit{Conclusion: }
From Fig.~\ref{fig:4ame_724_2}, we observe sudden diabatic transitions, since $\Gamma = 0.3$ results in very small gaps for most of the $H_{\text{init}}$. Meanwhile, a relatively long anneal time of $\tau = 400$ns allows open-system relaxation mechanism to increase the (instantaneous and final success probability) ground state population for some of the initial states. 
% \begin{figure}[h!]
% \subfigure[]{\includegraphics[width = 8cm]{ame_plot_2_724_2.pdf}\label{fig:4qubitsunitarya}}
% \subfigure[]{\includegraphics[width = 8cm]{ame_plot_2_724_2.pdf}\label{fig:8qubitsunitary}}
% \caption{Open-system and close-system adiabatic reverse annealing (ARA) simulation results. $\tau = 400$ns. $\Gamma = 0.3$.}
% \label{fig:compareall}
% \end{figure}
% \subsubsection{Results of $4$-qubit simulation: $\tau = 400$ns. $\Gamma = 5$.}

\section{ARA: Random initial state $c=0.5$.}
As in previous studies, the success of ARA depends on whether our initial state is close to the correct solution or not. In this section, we study the most general case where the initial state is a random guess ($c=0.5$, where $c=N_{\uparrow}/N$) and want to see if $\mathsf{ARA_\text{Open}}$ can give an enhancement over $\mathsf{ARA_\text{Closed}}$. Instead of looking at ground state population along the anneal, we now focus only on the results of ARA at the end of anneal. A summary of the results as a function of $N$ and $\tau$ is shown in Fig.~\ref{fig:compareall}.

\begin{figure}[h!]
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_closed_randomguess.pdf}\label{fig:4qubitsunitarya}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_open_randomguess.pdf}\label{fig:8qubitsunitary}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_col_randomguess.pdf}\label{fig:8qubitsunitary}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_qa_randomguess_TTS_compare_10.pdf}}
\caption{ARA performance for (a) closed system, (b) open system with independent system-bath coupling, (c) open system with collective system-bath coupling, (d) comparison of the 3 situations in terms of TTS ($N=10$).}
\label{fig:compareall}
\end{figure}

First of all, we observe that success probabilities go up monotonically with anneal time $\tau$ for the case of $\mathsf{ARA_\text{Closed}}$. As expected, the longer the anneal time $\tau$, the more adiabatic the evolution and the higher the success probability.
For $\mathsf{ARA_\text{Open}}$, however, we observe that there can exist an intermediate anneal time $\tau$ that gives a locally maximal success probability, and this is true for both SB coupling models. Such non-monotonic dependence of success probabilities in terms of anneal times $\tau$ is due to the environmental induced relaxation after diabatic transitions to higher excited states.

Secondly, at long anneal times, for the case of $\mathsf{ARA_\text{Closed}}$ the ground state is reached with with certainty (success probability $= 1$); while for the case of $\mathsf{ARA_\text{Open}}$, the Gibbs state is reached. Therefore, in all situations $\mathsf{ARA_\text{Closed}}$ always outperforms $\mathsf{ARA_\text{Open}}$ for long enough anneal times $\tau$. However, as shown in later section~\ref{sec:modelcompare}, the steady state reached by the two different system bath coupling model is different. 

To see if relaxation can provide any quantum enhancement, we do observe that for some $N$ $\mathsf{ARA_\text{Open}}$ performs better than $\mathsf{ARA_\text{Closed}}$ in the cases of intermediate anneal times $\tau$. We plot in Fig.~\ref{fig:compareall}\textcolor{blue}{(d)} for the case of $N=10$ that $\mathsf{ARA}$ performs better in an open system settings in terms of shorter $\mathsf{TTS}$. For both  $\mathsf{ARA_\text{Closed}}$ and $\mathsf{ARA_\text{Open}}$ we observe optimal TTS. To avoid the misinterpretation of TTS, we avoid the calculation of $\mathsf{TTS}(\tau)$ where the success probability $p_g(\tau)$ is very close to $0$ and $1$. Lastly, we can see that in general the performance of both $\mathsf{ARA_\text{Closed}}$ and  $\mathsf{ARA_\text{Open}}$ worsens as $N$ increases. 

% We draw several conclusions:
% 1. $\mathsf{ARA_\text{Open}}$ has optimal stopping times. But $\mathsf{ARA_\text{Closed}}$ does not.
% 2. Whether $\mathsf{ARA_\text{Open}}$ can beat $\mathsf{ARA_\text{Closed}}$ is case by case scenario
% Attached plot where it beats
% 3. 
% The conclusion of optimal stopping times is clearer when we look at the TTS.
% We made the conclusion that instead of 

\subsection{QA}
\begin{figure}[h!]
% \subfigure[]{\includegraphics[width = 8cm]{annealsuccessprob_qa_closed_randomguess.pdf}\label{fig:4qubitsunitarya}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_qa_open_randomguess.pdf}\label{fig:8qubitsunitary}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_qa_col_randomguess.pdf}\label{fig:8qubitsunitary}}
\caption{Standard QA in an open system with two different system-bath coupling model.}
\label{fig:qaopen}
\end{figure}

 We show in Fig.~\ref{fig:qaopen} the case of quantum annealing in open system $\mathsf{ARA_\text{Open}}$. Note that the initial state of QA is the equal superposition  $\ket{+}^{\otimes N}$. Comparing Fig.~\ref{fig:qaopen} with Fig.~\ref{fig:compareall}, we can see easily that $\mathsf{QA_\text{Open}}$ achieves higher success probabilities for all $N$ and $\tau$. Therefore, for random initial states $c=0.5$,  $\mathsf{ARA_\text{Open}}$ cannot outperform $\mathsf{QA_\text{Open}}$. 


\section{ARA performance in terms of $\Gamma$ and $H_{\mathrm{init}}$}
We now want to study the dependence of ARA performance in terms of $H_{\mathrm{init}}$ and $\Gamma$. For this purpose, we fix the number of qubits $N$ in our studies in this section.
\subsection{Min. Gap vs $H_{\mathrm{init}}$ vs $\Gamma$. $N=4$.}
\begin{figure}[h!]
\includegraphics[width=0.8\textwidth]{ra3/pspin_ARA_spectrum_3d.pdf}
\caption{The value of minimum gap as a function of $H_{\mathrm{init}}$ and $\Gamma$. $N=4$.}
\label{fig:spectrum_3d}
\end{figure}

We first plot in Fig.~\ref{fig:spectrum_3d} the value of minimum gap of ARA ($N=4$) as a function of initial state $H_{\mathrm{init}}$ and $\Gamma$. Except for initial states that are close to the correct solutions, in general the larger the transverse field $\Gamma$ the larger the minimum gap $\Delta_{\text{min}}$.


\subsection{Different Anneal times + Different $\Gamma = \{1,2,5\}$. $N=4$. $\mathsf{ARA_\text{Open}}$.}
% \begin{figure}[h!]
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=3.33in]{annealsuccessprob_89_trial.pdf}
% \caption{}
% \label{fig:sub1}
% \end{subfigure}
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=3.33in]{annealsuccessprob_825_trial.pdf}
% \caption{}
% \label{fig:sub3}
% \end{subfigure}
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=3.33in]{annealsuccessprob_810_trial.pdf}
% \caption{}
% \label{fig:sub3}
% \end{subfigure}
% \caption[]{}
% \label{fig: 3atoms}
% \end{figure}
\begin{figure}[h!]
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_89_trial.pdf}\label{fig:4qubitsunitarya}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_825_trial.pdf}\label{fig:8qubitsunitary}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_810_trial.pdf}\label{fig:8qubitsunitary}}
\caption{$\mathsf{ARA_{\text{open}}}$ results (a) $\Gamma=1$, (b) $\Gamma=2$, (c) $\Gamma=5$. Independent system-bath coupling.}
\label{fig:ARAopen4qubits}
\end{figure}

We studied and plot in Fig.~\ref{fig:ARAopen4qubits} the performance of $\mathsf{ARA_\text{Open}}$ as a function of initial state $H_{\mathrm{init}}$ and $\Gamma$. We focus on the assumption of Independent system-bath coupling. In general the closer the initial state to the correct solution, the higher the success probabilities of $\mathsf{ARA_\text{Open}}$. Except for initial states that are close to the correct solutions, in general we want to increase the transverse field $\Gamma$ to enhance ARA performance because it results in a larger gap, in agreement with the observation in Fig.~\ref{fig:spectrum_3d}. We also plot this dependence on $\Gamma$ in Fig.~\ref{fig:ARAopen4qubitsuudd} in terms of success probability and $\mathsf{TTS}$. $\mathsf{TTS}$ is also shorter for larger $\Gamma$ and we observe optimal $\mathsf{TTS}$ for all three values of $\Gamma$. 
% \subsection{Different Anneal times + $\Gamma = 1$. $4$ qubits. Closed vs Open.}
% We want to explore different anneal times $\tau$. One observation about the TTS is that

% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{success_duuu_close_open.pdf}\label{fig:4qubitscloseame}
% \label{fig:4ame_724_2}
% \caption{Black: open, Blue: closed.}
% \end{figure}


\begin{figure}[h!]
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_89_810_825.pdf}\label{fig:4qubitsunitarya}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/TTS_89_810_825.pdf}\label{fig:8qubitsunitary}}
\caption{$\mathsf{ARA_{\text{open}}}$ results, with initial state being $\ket{\downarrow\downarrow\uparrow\uparrow}$. (a) success probability, (b) $\mathsf{TTS}$. Independent system-bath coupling.}
\label{fig:ARAopen4qubitsuudd}
\end{figure}


% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{annealsuccessprob_89_810_825.pdf}\label{fig:8qubitsame}
% \label{fig:4ame_724_2}
% \end{figure}
\subsection{Different Anneal times + Different  $\Gamma<1$. $N=4$. $\mathsf{ARA_\text{Closed}}$ and $\mathsf{ARA_\text{Open}}$.}
We studied the case of $\Gamma<1$, which would results in a smaller gap (Fig.~\ref{fig:spectrum_3d}) except for the case where the initial state is equal to the correct solution. We studied and plot in Fig.~\ref{fig:gammasmaller1_closed} and Fig.~\ref{fig:gammasmaller1_open} the performance of $\mathsf{ARA_\text{Closed}}$ and $\mathsf{ARA_\text{Open}}$ respectively as a function of initial state $H_{\mathrm{init}}$ and $\Gamma$. Again we focus on the assumption of independent system-bath coupling. 

\begin{figure}[h!]
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_82_Gamma01}\label{fig:4qubitsunitarya}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_82_Gamma05}\label{fig:8qubitsunitary}}
\caption{$\mathsf{ARA_\text{Closed}}$  (a) $\Gamma = 0.1$, (b) $\Gamma = 0.5$. $N=4$.}
\label{fig:gammasmaller1_closed}
\end{figure}

\begin{figure}[h!]
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_82_open_Gamma01}\label{fig:4qubitsunitarya}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealsuccessprob_82_open_Gamma05}\label{fig:8qubitsunitary}}
\caption{$\mathsf{ARA_\text{Open}}$. (a) $\Gamma = 0.1$, (b) $\Gamma = 0.5$. $N=4$. Independent system-bath coupling.}
\label{fig:gammasmaller1_open}
\end{figure}

Comparing the results of $\mathsf{ARA_\text{Closed}}$ (Fig.~\ref{fig:gammasmaller1_closed}) and $\mathsf{ARA_\text{Open}}$ (Fig.~\ref{fig:gammasmaller1_open}), we again observe the non-monotonic dependence of success probabilities in terms of anneal times $\tau$ exclusively for $\mathsf{ARA_\text{Open}}$. We also see noticeable improvements of success probabilities due to open-system effect at intermediate anneal times $\tau$, especially if the initial states are far away from the correct solution. For both $\mathsf{ARA_\text{Closed}}$ and $\mathsf{ARA_\text{Open}}$, the larger $\Gamma$ the higher the success probabilities, except for the case where the initial state is equal to the correct solution.
% \clearpage
% \subsection{Different Anneal times + $\Gamma = 0.5$. $4$ qubits. Closed vs Open}
% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{annealsuccessprob_82_Gamma05_dddd_openvsclose.pdf}\label{fig:4qubitscloseame}
% \label{fig:4ame_724_2}
% \caption{Black: open, Blue: closed.}
% \end{figure}


% \clearpage
% \section{Pausing}
% \subsection{Different Anneal times + $\Gamma = 1$. $4$ qubits. Pausing for a duration $\tau$ at $s=0.3$. Closed vs Open}
% Closed:
% \begin{figure}[h!]
% \includegraphics[width=0.65\textwidth]{annealsuccessprob_Gamma1_pausing}\label{fig:4qubitscloseame}
% \label{fig:4ame_724_2}
% \caption{}
% \end{figure}

% \clearpage
% \subsection{Different Anneal times + $\Gamma = 1$. $4$ qubits. Pausing for a duration $\tau$ at $s=0.3$. Closed vs Open}
% Open:
% \begin{figure}[h!]
% \includegraphics[width=0.65\textwidth]{annealsuccessprob_open_Gamma1_pausing}\label{fig:4qubitscloseame}
% \label{fig:4ame_724_2}
% \caption{}
% \end{figure}

% \clearpage
% \subsection{Different Anneal times + $\Gamma = 1$. $4$ qubits. Pausing for a duration $\tau$ at $s=0.3$. Closed vs Open}
% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{annealsuccessprob_Gamma1_dddd_openvsclose_pausing}\label{fig:4qubitscloseame}
% \label{fig:4ame_724_2}
% \caption{Black: open, Blue: closed.}
% \end{figure}


% \clearpage
% \section{$8$, $10$-qubit example}
% \subsection{Different Anneal times. $8$ qubits. Two spins down. $\Gamma = 1$.}
% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{annealsuccessprob_dduuuuuu.pdf}\label{fig:8qubitsame}
% \caption{Black: open, Blue: closed.}
% \label{fig:4ame_724_2}
% \end{figure}

% \clearpage
% \subsection{Different Anneal times. $8$ qubits. Two spins down. $\Gamma = 1$.}
% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{TTS_dduuuuuu.pdf}\label{fig:8qubitsame}
% \caption{Black: open, Blue: closed.}
% \label{fig:4ame_724_2}
% \end{figure}

% \clearpage
% \subsection{Different Anneal times. $10$ qubits. Two spins down. $\Gamma = 1$.}
% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{annealsuccessprob_dduuuuuuuu.pdf}\label{fig:8qubitsame}
% \caption{Black: open, Blue: closed.}
% \label{fig:4ame_724_2}
% \end{figure}


% \clearpage
% \subsection{Different Anneal times. $10$ qubits. Two spins down. $\Gamma = 1$.}
% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{annealTTS_dduuuuuuuu.pdf}\label{fig:8qubitsame}
% \caption{Black: open, Blue: closed.}
% \label{fig:4ame_724_2}
% \end{figure}


% \clearpage
% \subsection{Different Anneal times. $8$ qubits. Two spins down. $\Gamma = 0.1$.}
% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{annealsuccessprob_dduuuuuu_2.pdf}\label{fig:8qubitsame}
% \caption{Black: open, Blue: closed.}
% \label{fig:4ame_724_2}
% \end{figure}


% \clearpage
% \subsection{Different Anneal times. $8$ qubits. Two spins down. $\Gamma = 0.1$.}
% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{annealTTS_dduuuuuu_2.pdf}\label{fig:8qubitsame}
% \caption{Black: open, Blue: closed.}
% \label{fig:4ame_724_2}
% \end{figure}

% \clearpage
% \subsection{Different Anneal times. $10$ qubits. Two spins down. $\Gamma = 0.1$.}
% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{annealsuccessprob_dduuuuuuuu_2.pdf}\label{fig:8qubitsame}
% \caption{Black: open, Blue: closed.}
% \label{fig:4ame_724_2}
% \end{figure}

\clearpage
\subsection{Different Anneal times. $\Gamma = 0.1$, $N_{\downarrow}=2$. $N=\{8,10\}$. $\mathsf{ARA_\text{Open}}$.}
We studied the extreme case of $\Gamma = 0.1$ for larger $N$. Note that for such small $\Gamma = 0.1$, the transverse field is very weak and the Hamiltonian is dominated by the problem Hamiltonian $H_0$ and $H_{\text{init}}$. The resulting gap is very small and sharp and there is a large degree of diabatic transition to higher excited states. 

We plot in Fig.~\ref{fig:8_10_gamma01} the $\mathsf{TTS}$ dependence of anneal times $\tau$, for $N=\{8,10\}$ both with $N_{\downarrow}=2$. Due to the significant diabatic transition to higher excited states, $\mathsf{ARA_\text{Open}}$ tends to perform better than $\mathsf{ARA_\text{Closed}}$ because of the relaxation to the ground state.
\begin{figure}[h!]
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealTTS_dduuuuuu_2.pdf}\label{fig:4qubitsunitarya}}
\subfigure[]{\includegraphics[width = 8cm]{ra3/annealTTS_dduuuuuuuu_2.pdf}\label{fig:8qubitsunitary}}
\caption{(a) $N=8$, (b) $N=10$. $\Gamma = 0.1$ and $N_{\downarrow}=2$. Independent system-bath coupling.}
\label{fig:8_10_gamma01}
\end{figure}



\section{Independent vs collective SB coupling}
\label{sec:modelcompare}
We investigated the difference between the  independent and collective system-bath coupling assumption.

\subsection{Long anneal times $\tau$}
As observed in Fig.~\ref{fig:compareall}, for long anneal times $\tau$ the success probabilities given by simulation with the collective SB coupling assumption are higher than those given by independent SB coupling.
In fact, the steady state solution $\rho(s = 1,\tau \rightarrow \infty)$ of the Lindbladian master equation in the weak coupling limit is the Gibbs state set by the problem Hamiltonian. 
\begin{equation}
\rho(s = 1,\tau \rightarrow \infty) = \frac{e^{- \beta H_S(1)}}{\mathcal{Z}} = \frac{e^{- \beta H_0}}{\mathcal{Z}}\ .
\label{eq:rhoS0}
\end{equation}
where $\mathcal{Z} = \textrm{Tr}\left(\exp\left(- \beta H_0 \right)\right)$.

Recall that the permutation symmetry allows us to write the Hamiltonian in terms of only a set of total spin operators of two subsystems,
\begin{equation}
 \hat S^{x,z}_1 \equiv \frac{1}{2}\sum_{i=1}^{|N_{\uparrow}|}\hat\sigma^{x,z}_i,\quad
 \hat S^{x,z}_2 \equiv \frac{1}{2}\sum_{i=|N_{\uparrow}|+1}^{N}\hat\sigma^{x,z}_i \,.
\label{ra:eq:s1s2}
\end{equation}
% as
% \begin{align}
%  \hat H_0 &= -N(\frac{2}{N}(\hat S^z_1 + \hat S^z_2))^p \\
%  \hat H_{\text{init}} &= -2(\hat S^z_1 - \hat S^z_2),
%  \hat V_{\text{TF}}=-(\hat S^x_1 + \hat S^x_2).
%  \label{eq:H_blocked}
% \end{align}

% Since \((\hat{\bf{S}}_1)^2\) and \((\hat{\bf{S}}_2)^2\) commute with the total Hamiltonian, the system stays in the subspace with the largest values of \((\hat{\bf{S}}_1)^2\) and \((\hat{\bf{S}}_2)^2\) because the initial state lies in this subspace.

For collective SB coupling model, the dynamics occurs entirely in the two subspaces with maximum eigenvalues
of $S_1^2$ and $S^2_2$. The Lindbladian is defined according to the projection of $H(s)$ to such  subspaces.
% therefore we can restrict numerical simulations to the subspace
% given by their tensor product, having dimension $D = (\lfloor Nc \rfloor + 1)(N - \lfloor Nc\rfloor +
% 1)$, quadratic rather than exponential in $N$. In the two subspaces, suitable
% bases are given by the simultaneous eigenstates of $\{ S_j^2, S_j^z \}$, denoted $\left|j; w\right>$ and
% such that $S_j^z \left|j; w\right> = (S^z_{j,\text{max}} - w)\left|j; w\right>$, with $S^z_{1,\text{max}} = \lfloor Nc \rfloor /2$ and $S^z_{2,\text{max}} = 
% (N - \lfloor Nc \rfloor)/2$. In this representation, the initial state is 
% $\left|\psi(0)\right> = \left|1;0 \right> \otimes \left|2;N - \lfloor Nc \rfloor\right>$.
For collective SB coupling model, the steady state is given by:
\begin{equation}
\rho'(s = 1,\tau \rightarrow \infty) = \frac{e^{- \beta H_0'}}{\mathcal{Z'}} 
\label{eq:rhoS0}
\end{equation}
where $\mathcal{Z'} = \textrm{Tr}\left(\exp\left(- \beta H_0' \right)\right)$ and $H_0' = PH_0P$. $P = \sum_{\alpha} \ket{\psi_{\alpha}}\bra{\psi_{\alpha}}$ and $\ket{\psi_{\alpha}} = \left|1;w_1\right> \otimes \left|2;w_2\right>$ is the basis that has the maximum eigenvalues of $S_1^2$ and $S_2^2$.

A simple proof below shows that for long anneal times the success probability given by collective SB coupling model is always higher than the one given by independent SB coupling model.
\begin{proof}
Since $H_0'$ is the projection of $H_0$ in the subspace with the largest values of \((\hat{\bf{S}}_1)^2\) and \((\hat{\bf{S}}_2)^2\), $\mathcal{Z'}<\mathcal{Z}$. The success (ground state) probability $\langle g | \rho'(s = 1, \tau \rightarrow \infty) | g \rangle = \frac{e^{- \beta e_g}}{\mathcal{Z'}} > \frac{e^{- \beta e_g}}{\mathcal{Z}} = \langle g | \rho(s = 1, \tau \rightarrow \infty) | g \rangle$, where $e_g$ is the ground state energy. 
\end{proof}




\subsection{Intermediate anneal times $\tau$}
In general, since the assumption of independent SB coupling allows decoherence to many more eigenstates of $H(s)$ outside the maximal spin subspaces, it gives a lower success probability than the independent SB model for almost all anneal times $\tau$. For the example of $c=0.5$ and $\tau = 10$ns, we see in Fig.~\ref{fig:indvscol_n} that the difference of the success probability set by the two models diverge as system size $N$ increases. It is expected since the dimension reduction due to the restriction to maximal spin subspaces also scale exponentially in $N$.
% \begin{figure}[h!]
% \includegraphics[width=0.8\textwidth]{annealsuccessprob_n.pdf}\label{fig:8qubitsame}
% \label{fig:4ame_724_2}
% \end{figure}
\begin{figure}[h!]
\includegraphics[width=0.8\textwidth]{ra3/annealsuccessprob_vscol.pdf}
\caption{Dependence of success probability as a function of $N$ due to the two different SB coupling model. $c=0.5$, $\Gamma=1$ and $\tau = 10$ns.}
\label{fig:indvscol_n}
\end{figure}







% \clearpage
% \subsection{Different $N$.}
% We want to explore different $N$.

% \textit{Conclusion: }
% From Fig.~\ref{fig:4ame_724_2}, we observe sudden diabatic transitions, since $\Gamma = 0.3$ results in very small gaps for most of the $H_{\text{init}}$. Meanwhile, a relatively long anneal time of $\tau = 400$ns allows open-system relaxation mechanism to increase the (instantaneous and final success probability) ground state population for some of the initial states. 

% \section{Conditions where open-system ARA is better than unitary evolution}
% In general, as $\Gamma$ is smaller, $c$ is smaller, and $N$ is larger, 
% \begin{enumerate}
%   \item .
%   \item Intermediate anneal times
% \end{enumerate}

\section{Conclusion}
We broadly study the performance of ARA as a function of transverse field $\Gamma$, initial state $H_{\text{init}}$ and system size $N$. In general, except for the cases where the initial state is equal to the correct solution, ARA performs better with larger $\Gamma$. 

We observe non-monotonic dependence of success probabilities in terms of anneal times $\tau$ for $\mathsf{ARA_\text{Open}}$. For long anneal times, $\mathsf{ARA_\text{Closed}}$ reach solution with certainty, while $\mathsf{ARA_\text{Open}}$ reaches the Gibbs state. For $\mathsf{ARA_\text{Open}}$, the difference due to independent system-bath coupling assumption and collective system-bath coupling assumption is studied for both long anneal times $\tau$ and intermediate anneal times $\tau$. In general, the former assumption always results in a lower success probability (or longer TTS).

$\mathsf{ARA_\text{Open}}$ tends for outperform $\mathsf{ARA_\text{Closed}}$ in the following conditions:
\begin{enumerate}
  \item Small $\Gamma$.
  \item Initial state far away from the correct solution.
  \item Large $N$.
  \item Intermediate anneal times $\tau$.
\end{enumerate}
The first three conditions result in a small and sharp gap for diabatic transitions for intermediate anneal times $\tau$. Because of the environmental induced relaxation back to the ground state after diabatic transitions to higher excited states, $\mathsf{ARA_\text{Open}}$ performs better than $\mathsf{ARA_\text{Closed}}$ with the above conditions, in agreement with the prospects of quantum enhancement for diabatic annealing~\cite{crosson2020prospects}.


==> dedication.tex <==
\topskip0pt
\vspace*{\fill}
\vspace*{-2in}
\begin{quote}
    \center
\end{quote}
\vspace*{\fill}

